Step-Video-T2V Technical Report: The Practice, Challenges, and Future of Video Foundation Model

We present Step-Video-T2V, a state-of-the-art text-to-video pre-trained model with 30B parameters and the ability to generate videos up to 204 frames in length. A deep compression Variational Autoencoder, Video-VAE, is designed for video generation tasks, achieving 16x16 spatial and 8x temporal compression ratios, while maintaining exceptional video reconstruction quality. User prompts are encoded using two bilingual text encoders to handle both English and Chinese. A DiT with 3D full attention is trained using Flow Matching and is employed to denoise input noise into latent frames. A video-based DPO approach, Video-DPO, is applied to reduce artifacts and improve the visual quality of the generated videos. We also detail our training strategies and share key observations and insights. Step-Video-T2V's performance is evaluated on a novel video generation benchmark, Step-Video-T2V-Eval, demonstrating its state-of-the-art text-to-video quality when compared with both open-source and commercial engines. Additionally, we discuss the limitations of current diffusion-based model paradigm and outline future directions for video foundation models. We make both Step-Video-T2V and Step-Video-T2V-Eval available at https://github.com/stepfun-ai/Step-Video-T2V. The online version can be accessed from https://yuewen.cn/videos as well. Our goal is to accelerate the innovation of video foundation models and empower video content creators.

==> sec/ack.tex <==



==> table/ckpt_ppl_and_select_ratio.tex <==
\begin{table}[t]
\begin{minipage}{0.49\linewidth}
  \centering
  \includegraphics[width=1.0\textwidth]{figure/ckpt_ppl.pdf}
  \captionsetup{type=figure}
  \captionof{figure}{\textbf{The PPL of tokens selected by different checkpoint.} We test the PPL of the tokens selected at 2B, 5B, 8B, 11B, and 14B.
  }
  % \vspace{-1.5em}
  \label{fig:ckpt_ppl}
\end{minipage}
\hfill
\begin{minipage}{0.48\linewidth}
  \centering
  \includegraphics[width=1.0\textwidth]{figure/acc_vs_select_ratio.pdf}
  \captionsetup{type=figure}
  \captionof{figure}{\textbf{Effect of token select ratio.} We train 1B LM with SLM objective on 5B tokens.}
  % \vspace{-1.5em}
  \label{fig:acc_vs_select_ratio}
\end{minipage}
\hfill

\end{table}

% \begin{wrapfigure}{r}{0.5\textwidth}
%   \includegraphics[width=0.48\textwidth]{figure/totckpt_ppl.png}
% \caption{Select tokens using 2k, 5k, 8k, 11k, and 14k checkpoints(CKPT), and test the PPL of the corresponding selected tokens(ST) on all CKPT. The training data differs by 1B every 1k CKPT.}
% \label{fig:totckpt_ppl}
% \end{wrapfigure} 
% \begin{figure}[htbp]
% \centering
% \includegraphics[width=0.4\textwidth]{figure/acc_vs_select_ratio.pdf}
% \caption{Effect of token select ratio. We train 1B LM with SLM objective on 5B tokens.}
% \label{fig:acc_vs_select_ratio}
% \end{figure}

==> table/hhll_case.tex <==
\begin{table*}[t]
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}p{16cm}@{}}
\toprule
\multicolumn{1}{c}{\textbf{\textit{Examples of Four Categories of Tokens}}} \\
\midrule
\textcolor[RGB]{30,144,255}{GM}\textcolor[RGB]{34,139,34}{AT} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{250,128,114}{1}\textcolor[RGB]{30,144,255}{:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{6}\textcolor[RGB]{250,128,114}{7}\textcolor[RGB]{34,139,34}{0} \textcolor[RGB]{34,139,34}{ Q}\textcolor[RGB]{250,128,114}{4}\textcolor[RGB]{30,144,255}{9} \textcolor[RGB]{34,139,34}{ V}\textcolor[RGB]{34,139,34}{3}\textcolor[RGB]{250,128,114}{1} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{GM}\textcolor[RGB]{34,139,34}{AT} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{250,128,114}{7}\textcolor[RGB]{30,144,255}{1}\textcolor[RGB]{34,139,34}{0} \textcolor[RGB]{34,139,34}{ Q}\textcolor[RGB]{34,139,34}{5}\textcolor[RGB]{34,139,34}{0} \textcolor[RGB]{34,139,34}{ V}\textcolor[RGB]{34,139,34}{3}\textcolor[RGB]{30,144,255}{5} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{F}\textcolor[RGB]{34,139,34}{ollow}\textcolor[RGB]{34,139,34}{ers}\textcolor[RGB]{30,144,255}{:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{250,128,114}{7}\textcolor[RGB]{250,170,0}{5} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{K}\textcolor[RGB]{34,139,34}{ud}\textcolor[RGB]{34,139,34}{os} \textcolor[RGB]{34,139,34}{ {[}}\textcolor[RGB]{34,139,34}{?}\textcolor[RGB]{34,139,34}{{]}:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{30,144,255}{8}\textcolor[RGB]{250,170,0}{9}\textcolor[RGB]{250,170,0}{0} \textcolor[RGB]{34,139,34}{ {[}}\textcolor[RGB]{30,144,255}{0}\textcolor[RGB]{34,139,34}{{]},} \textcolor[RGB]{34,139,34}{ given}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{30,144,255}{2}\textcolor[RGB]{30,144,255}{3}\textcolor[RGB]{30,144,255}{5} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Re}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{250,128,114}{ Mr}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{30,144,255}{ and} \textcolor[RGB]{34,139,34}{ Mrs} \textcolor[RGB]{30,144,255}{ W}\textcolor[RGB]{30,144,255}{iley}\textcolor[RGB]{250,170,0}{,} \textcolor[RGB]{250,128,114}{ V}\textcolor[RGB]{30,144,255}{IC}\textcolor[RGB]{30,144,255}{ }\textcolor[RGB]{34,139,34}{{[}}\textcolor[RGB]{34,139,34}{\#}\textcolor[RGB]{34,139,34}{per}\textcolor[RGB]{34,139,34}{mal}\textcolor[RGB]{34,139,34}{ink}\textcolor[RGB]{34,139,34}{{]}} \textcolor[RGB]{34,139,34}{  }\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{250,170,0}{3} \textcolor[RGB]{250,170,0}{ Feb} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{30,144,255}{1}\textcolor[RGB]{250,128,114}{0}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{250,170,0}{1}\textcolor[RGB]{34,139,34}{:}\textcolor[RGB]{250,170,0}{0}\textcolor[RGB]{250,170,0}{3} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{250,170,0}{A}\textcolor[RGB]{250,170,0}{ns} \textcolor[RGB]{250,128,114}{ A} \textcolor[RGB]{250,128,114}{ \textbackslash n } \textcolor[RGB]{250,128,114}{ \textbackslash n }\textcolor[RGB]{30,144,255}{the}\textcolor[RGB]{250,128,114}{ir} \textcolor[RGB]{30,144,255}{ first} \textcolor[RGB]{34,139,34}{ child} \textcolor[RGB]{250,128,114}{ was} \textcolor[RGB]{250,128,114}{ born} \textcolor[RGB]{30,144,255}{ after} \textcolor[RGB]{30,144,255}{ J} \textcolor[RGB]{250,128,114}{ years}\textcolor[RGB]{250,170,0}{...} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{250,170,0}{th}\textcolor[RGB]{34,139,34}{us} \textcolor[RGB]{30,144,255}{ }\textcolor[RGB]{34,139,34}{1} \textcolor[RGB]{30,144,255}{ child} \textcolor[RGB]{30,144,255}{ ---}\textcolor[RGB]{34,139,34}{>} \textcolor[RGB]{250,170,0}{ j} \textcolor[RGB]{30,144,255}{ years} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{250,170,0}{=>} \textcolor[RGB]{250,170,0}{ thus} \textcolor[RGB]{30,144,255}{ after} \textcolor[RGB]{30,144,255}{ another} \textcolor[RGB]{250,128,114}{ J} \textcolor[RGB]{34,139,34}{ years} \textcolor[RGB]{250,128,114}{ his} \textcolor[RGB]{250,128,114}{ age} \textcolor[RGB]{30,144,255}{ =} \textcolor[RGB]{250,170,0}{ J} \textcolor[RGB]{250,170,0}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{th}\textcolor[RGB]{34,139,34}{us} \textcolor[RGB]{30,144,255}{ his} \textcolor[RGB]{34,139,34}{ age} \textcolor[RGB]{250,170,0}{ is} \textcolor[RGB]{250,128,114}{ J} \textcolor[RGB]{30,144,255}{ -->} \textcolor[RGB]{30,144,255}{ after} \textcolor[RGB]{30,144,255}{ }\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{30,144,255}{J} \textcolor[RGB]{30,144,255}{ years} \textcolor[RGB]{30,144,255}{ and} \textcolor[RGB]{250,128,114}{ }\textcolor[RGB]{30,144,255}{2}\textcolor[RGB]{30,144,255}{j} \textcolor[RGB]{30,144,255}{ after} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{30,144,255}{3}\textcolor[RGB]{30,144,255}{j} \textcolor[RGB]{30,144,255}{ years} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{250,128,114}{his} \textcolor[RGB]{30,144,255}{ present} \textcolor[RGB]{34,139,34}{ age} \textcolor[RGB]{250,128,114}{ is} \textcolor[RGB]{30,144,255}{ T} \textcolor[RGB]{250,170,0}{ which} \textcolor[RGB]{34,139,34}{ is} \textcolor[RGB]{250,128,114}{ after} \textcolor[RGB]{250,170,0}{ T} \textcolor[RGB]{250,128,114}{ years}\textcolor[RGB]{250,170,0}{.} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{th}\textcolor[RGB]{34,139,34}{us} \textcolor[RGB]{250,128,114}{ total} \textcolor[RGB]{30,144,255}{ time} \textcolor[RGB]{250,170,0}{ after} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{30,144,255}{2}\textcolor[RGB]{250,128,114}{year}\textcolor[RGB]{34,139,34}{s} \textcolor[RGB]{30,144,255}{ will} \textcolor[RGB]{34,139,34}{ be} \textcolor[RGB]{34,139,34}{ T}\textcolor[RGB]{30,144,255}{+}\textcolor[RGB]{34,139,34}{2} \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor[RGB]{250,170,0}{since} \textcolor[RGB]{250,170,0}{ after} \textcolor[RGB]{30,144,255}{ every} \textcolor[RGB]{30,144,255}{ J} \textcolor[RGB]{250,170,0}{ year} \textcolor[RGB]{30,144,255}{ they} \textcolor[RGB]{30,144,255}{ have} \textcolor[RGB]{30,144,255}{ a} \textcolor[RGB]{34,139,34}{ child} \textcolor[RGB]{30,144,255}{ after} \textcolor[RGB]{30,144,255}{ T}\textcolor[RGB]{250,128,114}{+}\textcolor[RGB]{34,139,34}{2} \textcolor[RGB]{30,144,255}{ they} \textcolor[RGB]{34,139,34}{ will} \textcolor[RGB]{30,144,255}{ have} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{30,144,255}{\{(}\textcolor[RGB]{34,139,34}{T}\textcolor[RGB]{34,139,34}{+}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{250,128,114}{)\}\{}\textcolor[RGB]{30,144,255}{J}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{30,144,255}{ +} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1} \textcolor[RGB]{30,144,255}{ (} \textcolor[RGB]{30,144,255}{ +}\textcolor[RGB]{30,144,255}{1} \textcolor[RGB]{250,170,0}{ is} \textcolor[RGB]{30,144,255}{ for} \textcolor[RGB]{34,139,34}{ the} \textcolor[RGB]{30,144,255}{ oldest}\textcolor[RGB]{30,144,255}{)} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{th}\textcolor[RGB]{34,139,34}{us} \textcolor[RGB]{250,170,0}{ A} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_}\textcolor[RGB]{34,139,34}{\_} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{250,170,0}{F}\textcolor[RGB]{30,144,255}{ight} \textcolor[RGB]{30,144,255}{ for} \textcolor[RGB]{34,139,34}{ your} \textcolor[RGB]{34,139,34}{ dream}\textcolor[RGB]{34,139,34}{s} \textcolor[RGB]{34,139,34}{ :}\textcolor[RGB]{34,139,34}{For} \textcolor[RGB]{34,139,34}{ all} \textcolor[RGB]{34,139,34}{ those} \textcolor[RGB]{34,139,34}{ who} \textcolor[RGB]{34,139,34}{ fear} \textcolor[RGB]{34,139,34}{ from} \textcolor[RGB]{34,139,34}{ Ver}\textcolor[RGB]{34,139,34}{bal}\textcolor[RGB]{34,139,34}{-} \textcolor[RGB]{34,139,34}{ lets} \textcolor[RGB]{34,139,34}{ give} \textcolor[RGB]{34,139,34}{ it} \textcolor[RGB]{34,139,34}{ a} \textcolor[RGB]{34,139,34}{ fight} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{M}\textcolor[RGB]{34,139,34}{oney} \textcolor[RGB]{34,139,34}{ Sav}\textcolor[RGB]{34,139,34}{ed} \textcolor[RGB]{34,139,34}{ is} \textcolor[RGB]{34,139,34}{ the} \textcolor[RGB]{34,139,34}{ M}\textcolor[RGB]{34,139,34}{oney} \textcolor[RGB]{34,139,34}{ E}\textcolor[RGB]{34,139,34}{arn}\textcolor[RGB]{34,139,34}{ed} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Jo} \textcolor[RGB]{34,139,34}{ B}\textcolor[RGB]{34,139,34}{ole} \textcolor[RGB]{34,139,34}{ So} \textcolor[RGB]{34,139,34}{ Ni}\textcolor[RGB]{34,139,34}{ha}\textcolor[RGB]{34,139,34}{al} \textcolor[RGB]{34,139,34}{ ,} \textcolor[RGB]{34,139,34}{ Sat} \textcolor[RGB]{34,139,34}{ Sh}\textcolor[RGB]{34,139,34}{ri} \textcolor[RGB]{34,139,34}{ A}\textcolor[RGB]{34,139,34}{ka}\textcolor[RGB]{34,139,34}{al} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{G}\textcolor[RGB]{30,144,255}{mat} \textcolor[RGB]{30,144,255}{ test} \textcolor[RGB]{30,144,255}{ review} \textcolor[RGB]{34,139,34}{ :} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{6}\textcolor[RGB]{30,144,255}{7}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{30,144,255}{-}\textcolor[RGB]{30,144,255}{to}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{30,144,255}{7}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{a}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{long}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{j}\textcolor[RGB]{34,139,34}{our}\textcolor[RGB]{34,139,34}{ney}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{without}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{destination}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{st}\textcolor[RGB]{34,139,34}{ill}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{h}\textcolor[RGB]{34,139,34}{appy}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{30,144,255}{4}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{6}\textcolor[RGB]{34,139,34}{4}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{.}\textcolor[RGB]{34,139,34}{html} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{Intern} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Jo}\textcolor[RGB]{34,139,34}{ined}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{250,170,0}{6} \textcolor[RGB]{250,128,114}{ A}\textcolor[RGB]{34,139,34}{pr} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{250,128,114}{1}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Post}\textcolor[RGB]{34,139,34}{s}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{250,128,114}{8} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{F}\textcolor[RGB]{34,139,34}{ollow}\textcolor[RGB]{34,139,34}{ers}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{0} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{K}\textcolor[RGB]{34,139,34}{ud}\textcolor[RGB]{34,139,34}{os} \textcolor[RGB]{34,139,34}{ {[}}\textcolor[RGB]{34,139,34}{?}\textcolor[RGB]{34,139,34}{{]}:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{250,128,114}{4} \textcolor[RGB]{34,139,34}{ {[}}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{{]},} \textcolor[RGB]{34,139,34}{ given}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{250,170,0}{3}\textcolor[RGB]{250,170,0}{7} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Re}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ Mr}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{34,139,34}{ and} \textcolor[RGB]{34,139,34}{ Mrs} \textcolor[RGB]{34,139,34}{ W}\textcolor[RGB]{34,139,34}{iley}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ V}\textcolor[RGB]{34,139,34}{IC}\textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{{[}}\textcolor[RGB]{34,139,34}{\#}\textcolor[RGB]{34,139,34}{per}\textcolor[RGB]{34,139,34}{mal}\textcolor[RGB]{34,139,34}{ink}\textcolor[RGB]{34,139,34}{{]}} \textcolor[RGB]{34,139,34}{  }\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{250,170,0}{1} \textcolor[RGB]{250,128,114}{ Nov} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{250,170,0}{7}\textcolor[RGB]{34,139,34}{:}\textcolor[RGB]{250,170,0}{4}\textcolor[RGB]{250,170,0}{6} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{je}\textcolor[RGB]{30,144,255}{etes}\textcolor[RGB]{34,139,34}{h}\textcolor[RGB]{34,139,34}{sing}\textcolor[RGB]{34,139,34}{h} \textcolor[RGB]{34,139,34}{ wrote}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{250,128,114}{Ne}\textcolor[RGB]{30,144,255}{ed} \textcolor[RGB]{30,144,255}{ the} \textcolor[RGB]{30,144,255}{ solution} \textcolor[RGB]{30,144,255}{ using} \textcolor[RGB]{30,144,255}{ Al}\textcolor[RGB]{34,139,34}{gebra}\textcolor[RGB]{250,170,0}{....} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{Mr}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{30,144,255}{ \&} \textcolor[RGB]{34,139,34}{ Mrs} \textcolor[RGB]{34,139,34}{ W}\textcolor[RGB]{34,139,34}{iley} \textcolor[RGB]{30,144,255}{ have} \textcolor[RGB]{34,139,34}{ a} \textcolor[RGB]{30,144,255}{ child} \textcolor[RGB]{30,144,255}{ every} \textcolor[RGB]{30,144,255}{ J} \textcolor[RGB]{34,139,34}{ years}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{30,144,255}{ Their} \textcolor[RGB]{30,144,255}{ oldest} \textcolor[RGB]{34,139,34}{ child} \textcolor[RGB]{30,144,255}{ is} \textcolor[RGB]{30,144,255}{ now} \textcolor[RGB]{30,144,255}{ T} \textcolor[RGB]{34,139,34}{ years} \textcolor[RGB]{34,139,34}{ old}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{30,144,255}{ If} \textcolor[RGB]{30,144,255}{ they} \textcolor[RGB]{34,139,34}{ have} \textcolor[RGB]{30,144,255}{ a} \textcolor[RGB]{30,144,255}{ child} \textcolor[RGB]{30,144,255}{ }\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ years} \textcolor[RGB]{34,139,34}{ from} \textcolor[RGB]{34,139,34}{ now}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{30,144,255}{ how} \textcolor[RGB]{250,128,114}{ many} \textcolor[RGB]{250,128,114}{ children} \textcolor[RGB]{30,144,255}{ will} \textcolor[RGB]{34,139,34}{ they} \textcolor[RGB]{34,139,34}{ have} \textcolor[RGB]{30,144,255}{ in} \textcolor[RGB]{30,144,255}{ total}\textcolor[RGB]{34,139,34}{?} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{(}\textcolor[RGB]{30,144,255}{A}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{250,128,114}{\{}\textcolor[RGB]{30,144,255}{T}\textcolor[RGB]{30,144,255}{+}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{J}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ +} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor[RGB]{34,139,34}{(}\textcolor[RGB]{34,139,34}{B}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{250,128,114}{ J}\textcolor[RGB]{30,144,255}{T} \textcolor[RGB]{34,139,34}{ +} \textcolor[RGB]{250,128,114}{ }\textcolor[RGB]{30,144,255}{1} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{(}\textcolor[RGB]{34,139,34}{C}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{J}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{30,144,255}{T}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ +} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{30,144,255}{T}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{(}\textcolor[RGB]{34,139,34}{D}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{250,128,114}{ T}\textcolor[RGB]{30,144,255}{J} \textcolor[RGB]{250,170,0}{ -} \textcolor[RGB]{30,144,255}{ }\textcolor[RGB]{34,139,34}{1} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{(}\textcolor[RGB]{34,139,34}{E}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{T}\textcolor[RGB]{250,128,114}{+}\textcolor[RGB]{30,144,255}{J}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{J}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{{[}}\textcolor[RGB]{34,139,34}{Re}\textcolor[RGB]{34,139,34}{ve}\textcolor[RGB]{34,139,34}{al}\textcolor[RGB]{34,139,34}{{]}} \textcolor[RGB]{34,139,34}{ Spo}\textcolor[RGB]{34,139,34}{iler}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{250,128,114}{ O}\textcolor[RGB]{34,139,34}{A}\textcolor[RGB]{30,144,255}{:} \textcolor[RGB]{250,170,0}{ \textbackslash n }\textcolor[RGB]{30,144,255}{(}\textcolor[RGB]{30,144,255}{A}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{Source}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{250,128,114}{ Manh}\textcolor[RGB]{34,139,34}{attan} \textcolor[RGB]{250,128,114}{ Guide} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{250,170,0}{B}\textcolor[RGB]{34,139,34}{un}\textcolor[RGB]{34,139,34}{uel} \textcolor[RGB]{30,144,255}{ -} \textcolor[RGB]{30,144,255}{ would} \textcolor[RGB]{30,144,255}{ really} \textcolor[RGB]{34,139,34}{ appreciate} \textcolor[RGB]{250,128,114}{ you} \textcolor[RGB]{250,170,0}{ providing} \textcolor[RGB]{30,144,255}{ your} \textcolor[RGB]{30,144,255}{ bit} \textcolor[RGB]{30,144,255}{ on} \textcolor[RGB]{250,128,114}{ solving} \textcolor[RGB]{250,170,0}{ the} \textcolor[RGB]{250,128,114}{ original} \textcolor[RGB]{250,128,114}{ problem} \textcolor[RGB]{30,144,255}{ above} \textcolor[RGB]{30,144,255}{ algebra}\textcolor[RGB]{34,139,34}{ically}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{30,144,255}{ The} \textcolor[RGB]{250,170,0}{ problem} \textcolor[RGB]{30,144,255}{ and} \textcolor[RGB]{30,144,255}{ various} \textcolor[RGB]{250,170,0}{ explan}\textcolor[RGB]{34,139,34}{ations} \textcolor[RGB]{250,128,114}{ remain} \textcolor[RGB]{30,144,255}{ confusing}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{250,170,0}{ Should} \textcolor[RGB]{250,170,0}{ we} \textcolor[RGB]{250,170,0}{ think} \textcolor[RGB]{34,139,34}{ of} \textcolor[RGB]{30,144,255}{ it} \textcolor[RGB]{34,139,34}{ as} \textcolor[RGB]{34,139,34}{ a} \textcolor[RGB]{30,144,255}{ pro}\textcolor[RGB]{34,139,34}{gression} \textcolor[RGB]{250,170,0}{ or} \textcolor[RGB]{30,144,255}{ some} \textcolor[RGB]{30,144,255}{ other} \textcolor[RGB]{250,170,0}{ way}\textcolor[RGB]{34,139,34}{?} \textcolor[RGB]{30,144,255}{ Please} \textcolor[RGB]{250,170,0}{ share} \textcolor[RGB]{34,139,34}{ your} \textcolor[RGB]{250,170,0}{ take}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{30,144,255}{ Thank} \textcolor[RGB]{34,139,34}{ you}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{Ver}\textcolor[RGB]{34,139,34}{itas} \textcolor[RGB]{34,139,34}{ P}\textcolor[RGB]{34,139,34}{rep} \textcolor[RGB]{34,139,34}{ G}\textcolor[RGB]{34,139,34}{M}\textcolor[RGB]{34,139,34}{AT} \textcolor[RGB]{34,139,34}{ Inst}\textcolor[RGB]{34,139,34}{ruct}\textcolor[RGB]{34,139,34}{or} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Jo}\textcolor[RGB]{34,139,34}{ined}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{6} \textcolor[RGB]{34,139,34}{ Oct} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{0} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Post}\textcolor[RGB]{34,139,34}{s}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{30,144,255}{4}\textcolor[RGB]{250,128,114}{5}\textcolor[RGB]{250,128,114}{6}\textcolor[RGB]{30,144,255}{6} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Location}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ P}\textcolor[RGB]{34,139,34}{une}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ India} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{F}\textcolor[RGB]{34,139,34}{ollow}\textcolor[RGB]{34,139,34}{ers}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{30,144,255}{1}\textcolor[RGB]{30,144,255}{0}\textcolor[RGB]{30,144,255}{2}\textcolor[RGB]{30,144,255}{9} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{K}\textcolor[RGB]{34,139,34}{ud}\textcolor[RGB]{34,139,34}{os} \textcolor[RGB]{34,139,34}{ {[}}\textcolor[RGB]{34,139,34}{?}\textcolor[RGB]{34,139,34}{{]}:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{30,144,255}{4}\textcolor[RGB]{30,144,255}{4}\textcolor[RGB]{250,170,0}{6}\textcolor[RGB]{250,170,0}{0} \textcolor[RGB]{34,139,34}{ {[}}\textcolor[RGB]{30,144,255}{1}\textcolor[RGB]{34,139,34}{{]}} \textcolor[RGB]{34,139,34}{ ,} \textcolor[RGB]{34,139,34}{ given}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{30,144,255}{6}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Re}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ Mr}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{34,139,34}{ and} \textcolor[RGB]{34,139,34}{ Mrs} \textcolor[RGB]{34,139,34}{ W}\textcolor[RGB]{34,139,34}{iley}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ V}\textcolor[RGB]{34,139,34}{IC}\textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{{[}}\textcolor[RGB]{34,139,34}{\#}\textcolor[RGB]{34,139,34}{per}\textcolor[RGB]{34,139,34}{mal}\textcolor[RGB]{34,139,34}{ink}\textcolor[RGB]{34,139,34}{{]}} \textcolor[RGB]{34,139,34}{  }\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{1} \textcolor[RGB]{34,139,34}{ Nov} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{9}\textcolor[RGB]{34,139,34}{:}\textcolor[RGB]{250,170,0}{4}\textcolor[RGB]{250,170,0}{5} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{1} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{K}\textcolor[RGB]{34,139,34}{UD}\textcolor[RGB]{34,139,34}{OS} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Ex}\textcolor[RGB]{34,139,34}{pert}\textcolor[RGB]{34,139,34}{'}\textcolor[RGB]{34,139,34}{s} \textcolor[RGB]{34,139,34}{ post} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{250,128,114}{je}\textcolor[RGB]{34,139,34}{etes}\textcolor[RGB]{34,139,34}{h}\textcolor[RGB]{34,139,34}{sing}\textcolor[RGB]{34,139,34}{h} \textcolor[RGB]{34,139,34}{ wrote}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{Ne}\textcolor[RGB]{34,139,34}{ed} \textcolor[RGB]{34,139,34}{ the} \textcolor[RGB]{34,139,34}{ solution} \textcolor[RGB]{34,139,34}{ using} \textcolor[RGB]{34,139,34}{ Al}\textcolor[RGB]{34,139,34}{gebra}\textcolor[RGB]{34,139,34}{....} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Mr}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{34,139,34}{ \&} \textcolor[RGB]{34,139,34}{ Mrs} \textcolor[RGB]{34,139,34}{ W}\textcolor[RGB]{34,139,34}{iley} \textcolor[RGB]{34,139,34}{ have} \textcolor[RGB]{34,139,34}{ a} \textcolor[RGB]{34,139,34}{ child} \textcolor[RGB]{34,139,34}{ every} \textcolor[RGB]{34,139,34}{ J} \textcolor[RGB]{34,139,34}{ years}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{34,139,34}{ Their} \textcolor[RGB]{34,139,34}{ oldest} \textcolor[RGB]{34,139,34}{ child} \textcolor[RGB]{34,139,34}{ is} \textcolor[RGB]{34,139,34}{ now} \textcolor[RGB]{34,139,34}{ T} \textcolor[RGB]{34,139,34}{ years} \textcolor[RGB]{34,139,34}{ old}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{34,139,34}{ If} \textcolor[RGB]{34,139,34}{ they} \textcolor[RGB]{34,139,34}{ have} \textcolor[RGB]{34,139,34}{ a} \textcolor[RGB]{34,139,34}{ child} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{2} \textcolor[RGB]{34,139,34}{ years} \textcolor[RGB]{34,139,34}{ from} \textcolor[RGB]{34,139,34}{ now}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ how} \textcolor[RGB]{34,139,34}{ many} \textcolor[RGB]{34,139,34}{ children} \textcolor[RGB]{34,139,34}{ will} \textcolor[RGB]{34,139,34}{ they} \textcolor[RGB]{34,139,34}{ have} \textcolor[RGB]{34,139,34}{ in} \textcolor[RGB]{34,139,34}{ total}\textcolor[RGB]{34,139,34}{?} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{(}\textcolor[RGB]{34,139,34}{A}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{T}\textcolor[RGB]{34,139,34}{+}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{J}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ +} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{(}\textcolor[RGB]{34,139,34}{B}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{34,139,34}{ J}\textcolor[RGB]{34,139,34}{T} \textcolor[RGB]{34,139,34}{ +} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{(}\textcolor[RGB]{34,139,34}{C}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{J}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{T}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ +} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{T}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{(}\textcolor[RGB]{34,139,34}{D}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{34,139,34}{ T}\textcolor[RGB]{34,139,34}{J} \textcolor[RGB]{34,139,34}{ -} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{(}\textcolor[RGB]{34,139,34}{E}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{T}\textcolor[RGB]{34,139,34}{+}\textcolor[RGB]{34,139,34}{J}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{J}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{{[}}\textcolor[RGB]{34,139,34}{Re}\textcolor[RGB]{34,139,34}{ve}\textcolor[RGB]{34,139,34}{al}\textcolor[RGB]{34,139,34}{{]}} \textcolor[RGB]{34,139,34}{ Spo}\textcolor[RGB]{34,139,34}{iler}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ O}\textcolor[RGB]{34,139,34}{A}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{(}\textcolor[RGB]{34,139,34}{A}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Source}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ Manh}\textcolor[RGB]{34,139,34}{attan} \textcolor[RGB]{34,139,34}{ Guide} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{250,170,0}{Th}\textcolor[RGB]{34,139,34}{ink} \textcolor[RGB]{34,139,34}{ of} \textcolor[RGB]{30,144,255}{ it} \textcolor[RGB]{30,144,255}{ as} \textcolor[RGB]{250,128,114}{ an} \textcolor[RGB]{30,144,255}{ Ar}\textcolor[RGB]{34,139,34}{ithmetic} \textcolor[RGB]{30,144,255}{ Pro}\textcolor[RGB]{34,139,34}{gression} \textcolor[RGB]{30,144,255}{ where} \textcolor[RGB]{250,170,0}{ every} \textcolor[RGB]{30,144,255}{ subsequent} \textcolor[RGB]{34,139,34}{ term} \textcolor[RGB]{250,170,0}{ (}\textcolor[RGB]{30,144,255}{child}\textcolor[RGB]{30,144,255}{)} \textcolor[RGB]{30,144,255}{ has} \textcolor[RGB]{30,144,255}{ a} \textcolor[RGB]{30,144,255}{ difference} \textcolor[RGB]{34,139,34}{ of} \textcolor[RGB]{30,144,255}{ J} \textcolor[RGB]{30,144,255}{ y}\textcolor[RGB]{34,139,34}{rs} \textcolor[RGB]{250,170,0}{ from} \textcolor[RGB]{34,139,34}{ the} \textcolor[RGB]{34,139,34}{ previous} \textcolor[RGB]{34,139,34}{ term} \textcolor[RGB]{34,139,34}{ (}\textcolor[RGB]{34,139,34}{child}\textcolor[RGB]{34,139,34}{).} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{250,128,114}{ \textbackslash n }\textcolor[RGB]{30,144,255}{1}\textcolor[RGB]{34,139,34}{st} \textcolor[RGB]{30,144,255}{ child}\textcolor[RGB]{250,170,0}{,} \textcolor[RGB]{30,144,255}{ }\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{nd} \textcolor[RGB]{34,139,34}{ child}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{3}\textcolor[RGB]{34,139,34}{rd} \textcolor[RGB]{34,139,34}{ child}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{250,170,0}{ ....}\textcolor[RGB]{30,144,255}{...} \textcolor[RGB]{30,144,255}{ n}\textcolor[RGB]{34,139,34}{th} \textcolor[RGB]{34,139,34}{ child} \textcolor[RGB]{30,144,255}{ (}\textcolor[RGB]{30,144,255}{to} \textcolor[RGB]{34,139,34}{ be} \textcolor[RGB]{250,128,114}{ born} \textcolor[RGB]{30,144,255}{ after} \textcolor[RGB]{30,144,255}{ }\textcolor[RGB]{34,139,34}{2} \textcolor[RGB]{30,144,255}{ y}\textcolor[RGB]{34,139,34}{rs}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{250,128,114}{ \textbackslash n }\textcolor[RGB]{250,170,0}{What} \textcolor[RGB]{34,139,34}{ is} \textcolor[RGB]{34,139,34}{ the} \textcolor[RGB]{34,139,34}{ difference} \textcolor[RGB]{34,139,34}{ between} \textcolor[RGB]{250,128,114}{ first} \textcolor[RGB]{34,139,34}{ and} \textcolor[RGB]{250,170,0}{ last} \textcolor[RGB]{250,128,114}{ terms} \textcolor[RGB]{250,128,114}{ (}\textcolor[RGB]{30,144,255}{children}\textcolor[RGB]{30,144,255}{)?} \textcolor[RGB]{30,144,255}{ (}\textcolor[RGB]{250,170,0}{T} \textcolor[RGB]{30,144,255}{ +} \textcolor[RGB]{30,144,255}{ }\textcolor[RGB]{30,144,255}{2}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{250,128,114}{ y}\textcolor[RGB]{34,139,34}{rs} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{250,128,114}{ \textbackslash n }\textcolor[RGB]{30,144,255}{What} \textcolor[RGB]{34,139,34}{ is} \textcolor[RGB]{34,139,34}{ the} \textcolor[RGB]{30,144,255}{ common} \textcolor[RGB]{34,139,34}{ difference} \textcolor[RGB]{250,128,114}{ (}\textcolor[RGB]{30,144,255}{age} \textcolor[RGB]{30,144,255}{ difference} \textcolor[RGB]{34,139,34}{ between} \textcolor[RGB]{30,144,255}{ two} \textcolor[RGB]{34,139,34}{ consecutive} \textcolor[RGB]{30,144,255}{ k}\textcolor[RGB]{30,144,255}{ids}\textcolor[RGB]{30,144,255}{)?} \textcolor[RGB]{30,144,255}{ J} \textcolor[RGB]{34,139,34}{ y}\textcolor[RGB]{34,139,34}{rs} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{What} \textcolor[RGB]{34,139,34}{ is} \textcolor[RGB]{34,139,34}{ the} \textcolor[RGB]{250,170,0}{ number} \textcolor[RGB]{34,139,34}{ of} \textcolor[RGB]{30,144,255}{ terms} \textcolor[RGB]{34,139,34}{ (}\textcolor[RGB]{30,144,255}{children}\textcolor[RGB]{30,144,255}{)?} \textcolor[RGB]{30,144,255}{ (}\textcolor[RGB]{34,139,34}{T} \textcolor[RGB]{34,139,34}{ +} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{30,144,255}{)/}\textcolor[RGB]{34,139,34}{J} \textcolor[RGB]{30,144,255}{ +} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{250,128,114}{(}\textcolor[RGB]{250,128,114}{Number} \textcolor[RGB]{34,139,34}{ of} \textcolor[RGB]{34,139,34}{ terms} \textcolor[RGB]{250,170,0}{ of} \textcolor[RGB]{30,144,255}{ an} \textcolor[RGB]{30,144,255}{ AP} \textcolor[RGB]{250,128,114}{ is} \textcolor[RGB]{30,144,255}{ n} \textcolor[RGB]{30,144,255}{ =} \textcolor[RGB]{30,144,255}{ (}\textcolor[RGB]{30,144,255}{Last} \textcolor[RGB]{34,139,34}{ term} \textcolor[RGB]{30,144,255}{ -} \textcolor[RGB]{34,139,34}{ First} \textcolor[RGB]{34,139,34}{ term}\textcolor[RGB]{30,144,255}{)/}\textcolor[RGB]{30,144,255}{Common} \textcolor[RGB]{30,144,255}{ D}\textcolor[RGB]{34,139,34}{ifference} \textcolor[RGB]{30,144,255}{ +} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{250,170,0}{.} \textcolor[RGB]{30,144,255}{ )} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_}\textcolor[RGB]{34,139,34}{\_} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Kar}\textcolor[RGB]{34,139,34}{ish}\textcolor[RGB]{34,139,34}{ma} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Ver}\textcolor[RGB]{34,139,34}{itas} \textcolor[RGB]{34,139,34}{ P}\textcolor[RGB]{34,139,34}{rep} \textcolor[RGB]{30,144,255}{ |} \textcolor[RGB]{34,139,34}{ G}\textcolor[RGB]{34,139,34}{M}\textcolor[RGB]{34,139,34}{AT} \textcolor[RGB]{34,139,34}{ Inst}\textcolor[RGB]{34,139,34}{ruct}\textcolor[RGB]{34,139,34}{or} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{My} \textcolor[RGB]{34,139,34}{ B}\textcolor[RGB]{34,139,34}{log} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{Save} \textcolor[RGB]{30,144,255}{ \$}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0} \textcolor[RGB]{34,139,34}{ on} \textcolor[RGB]{30,144,255}{ Ver}\textcolor[RGB]{34,139,34}{itas} \textcolor[RGB]{34,139,34}{ P}\textcolor[RGB]{34,139,34}{rep} \textcolor[RGB]{34,139,34}{ G}\textcolor[RGB]{34,139,34}{M}\textcolor[RGB]{34,139,34}{AT} \textcolor[RGB]{34,139,34}{ C}\textcolor[RGB]{34,139,34}{ourses} \textcolor[RGB]{34,139,34}{ And} \textcolor[RGB]{34,139,34}{ Ad}\textcolor[RGB]{34,139,34}{m}\textcolor[RGB]{34,139,34}{issions} \textcolor[RGB]{34,139,34}{ Cons}\textcolor[RGB]{34,139,34}{ult}\textcolor[RGB]{34,139,34}{ing} \textcolor[RGB]{34,139,34}{ En}\textcolor[RGB]{34,139,34}{roll} \textcolor[RGB]{30,144,255}{ now}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{34,139,34}{ Pay} \textcolor[RGB]{34,139,34}{ later}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{34,139,34}{ Take} \textcolor[RGB]{34,139,34}{ advantage} \textcolor[RGB]{34,139,34}{ of} \textcolor[RGB]{34,139,34}{ Ver}\textcolor[RGB]{34,139,34}{itas} \textcolor[RGB]{34,139,34}{ P}\textcolor[RGB]{34,139,34}{rep}\textcolor[RGB]{34,139,34}{'}\textcolor[RGB]{34,139,34}{s} \textcolor[RGB]{34,139,34}{ flexible} \textcolor[RGB]{34,139,34}{ payment} \textcolor[RGB]{34,139,34}{ plan} \textcolor[RGB]{34,139,34}{ options}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{34,139,34}{ Ver}\textcolor[RGB]{34,139,34}{itas} \textcolor[RGB]{34,139,34}{ P}\textcolor[RGB]{34,139,34}{rep} \textcolor[RGB]{34,139,34}{ Re}\textcolor[RGB]{34,139,34}{views} \textcolor[RGB]{30,144,255}{ Re}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ Mr}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{34,139,34}{ and} \textcolor[RGB]{34,139,34}{ Mrs} \textcolor[RGB]{34,139,34}{ W}\textcolor[RGB]{34,139,34}{iley}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ V}\textcolor[RGB]{34,139,34}{IC} \textcolor[RGB]{34,139,34}{ {[}}\textcolor[RGB]{34,139,34}{\#}\textcolor[RGB]{34,139,34}{per}\textcolor[RGB]{34,139,34}{mal}\textcolor[RGB]{34,139,34}{ink}\textcolor[RGB]{34,139,34}{{]}} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{1} \textcolor[RGB]{34,139,34}{ Nov} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{30,144,255}{0}\textcolor[RGB]{34,139,34}{9}\textcolor[RGB]{34,139,34}{:}\textcolor[RGB]{34,139,34}{4}\textcolor[RGB]{34,139,34}{5} \textcolor[RGB]{30,144,255}{ Similar} \textcolor[RGB]{34,139,34}{ topics} \textcolor[RGB]{34,139,34}{ Rep}\textcolor[RGB]{34,139,34}{lies} \textcolor[RGB]{34,139,34}{ Last} \textcolor[RGB]{34,139,34}{ post} \textcolor[RGB]{34,139,34}{ Similar} \textcolor[RGB]{34,139,34}{ Top}\textcolor[RGB]{34,139,34}{ics}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{30,144,255}{ }\textcolor[RGB]{250,128,114}{1} \textcolor[RGB]{250,128,114}{ Mr}\textcolor[RGB]{30,144,255}{.} \textcolor[RGB]{250,128,114}{ and} \textcolor[RGB]{34,139,34}{ Mrs}\textcolor[RGB]{30,144,255}{.} \textcolor[RGB]{30,144,255}{ O}\textcolor[RGB]{250,128,114}{’}\textcolor[RGB]{250,128,114}{Le}\textcolor[RGB]{34,139,34}{ary} \textcolor[RGB]{250,128,114}{ (}\textcolor[RGB]{30,144,255}{SC}\textcolor[RGB]{30,144,255}{)} \textcolor[RGB]{30,144,255}{ }\textcolor[RGB]{250,170,0}{5} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{250,170,0}{8} \textcolor[RGB]{30,144,255}{ Jul} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{250,128,114}{2}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{250,170,0}{7}\textcolor[RGB]{34,139,34}{:}\textcolor[RGB]{250,170,0}{1}\textcolor[RGB]{250,170,0}{5} \textcolor[RGB]{30,144,255}{ Mr}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{30,144,255}{ IN}\textcolor[RGB]{250,170,0}{VE}\textcolor[RGB]{34,139,34}{ST}\textcolor[RGB]{250,128,114}{OR} \textcolor[RGB]{30,144,255}{ inv}\textcolor[RGB]{34,139,34}{ested} \textcolor[RGB]{30,144,255}{ a} \textcolor[RGB]{250,128,114}{ total} \textcolor[RGB]{34,139,34}{ of}\textcolor[RGB]{30,144,255}{\$}\textcolor[RGB]{30,144,255}{1}\textcolor[RGB]{250,170,0}{2}\textcolor[RGB]{30,144,255}{,}\textcolor[RGB]{30,144,255}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0} \textcolor[RGB]{250,170,0}{ for} \textcolor[RGB]{250,170,0}{ a} \textcolor[RGB]{250,170,0}{ one}\textcolor[RGB]{30,144,255}{-}\textcolor[RGB]{34,139,34}{year} \textcolor[RGB]{30,144,255}{ }\textcolor[RGB]{30,144,255}{4} \textcolor[RGB]{30,144,255}{ }\textcolor[RGB]{30,144,255}{3}\textcolor[RGB]{34,139,34}{0} \textcolor[RGB]{250,170,0}{ Mar} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{30,144,255}{0}\textcolor[RGB]{30,144,255}{7}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{30,144,255}{9}\textcolor[RGB]{34,139,34}{:}\textcolor[RGB]{250,170,0}{2}\textcolor[RGB]{250,170,0}{4} \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor[RGB]{250,128,114}{2} \textcolor[RGB]{34,139,34}{ Mr}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{250,128,114}{ and} \textcolor[RGB]{34,139,34}{ Mrs}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{250,128,114}{ W}\textcolor[RGB]{34,139,34}{iley} \textcolor[RGB]{30,144,255}{ have} \textcolor[RGB]{34,139,34}{ a} \textcolor[RGB]{30,144,255}{ child} \textcolor[RGB]{34,139,34}{ every} \textcolor[RGB]{34,139,34}{ J} \textcolor[RGB]{34,139,34}{ years}\textcolor[RGB]{30,144,255}{.} \textcolor[RGB]{34,139,34}{ Their} \textcolor[RGB]{30,144,255}{ oldest} \textcolor[RGB]{30,144,255}{ }\textcolor[RGB]{30,144,255}{7} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{250,170,0}{9} \textcolor[RGB]{250,128,114}{ Feb} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{7}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{250,170,0}{1}\textcolor[RGB]{34,139,34}{:}\textcolor[RGB]{250,170,0}{4}\textcolor[RGB]{250,170,0}{0} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{Mr}\textcolor[RGB]{34,139,34}{.}\textcolor[RGB]{250,128,114}{ke}\textcolor[RGB]{30,144,255}{vin}\textcolor[RGB]{30,144,255}{can} \textcolor[RGB]{30,144,255}{ }\textcolor[RGB]{30,144,255}{6} \textcolor[RGB]{30,144,255}{ }\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{250,170,0}{6} \textcolor[RGB]{250,170,0}{ Aug} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{6}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{250,170,0}{2}\textcolor[RGB]{34,139,34}{:}\textcolor[RGB]{250,170,0}{2}\textcolor[RGB]{250,170,0}{6} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{PS}\textcolor[RGB]{30,144,255}{:} \textcolor[RGB]{34,139,34}{ Mr}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{30,144,255}{ \&} \textcolor[RGB]{34,139,34}{ Mrs}\textcolor[RGB]{30,144,255}{.} \textcolor[RGB]{30,144,255}{ Smith} \textcolor[RGB]{30,144,255}{ }\textcolor[RGB]{250,170,0}{2} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{250,170,0}{6} \textcolor[RGB]{250,170,0}{ Dec} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{30,144,255}{5}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{250,128,114}{0}\textcolor[RGB]{34,139,34}{:}\textcolor[RGB]{250,170,0}{0}\textcolor[RGB]{250,170,0}{3} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{Display} \textcolor[RGB]{34,139,34}{ posts} \textcolor[RGB]{34,139,34}{ from} \textcolor[RGB]{34,139,34}{ previous}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ Sort} \textcolor[RGB]{34,139,34}{ by} \textcolor[RGB]{30,144,255}{ Sci}\textcolor[RGB]{30,144,255}{enc}\textcolor[RGB]{34,139,34}{em}\textcolor[RGB]{34,139,34}{ad}\textcolor[RGB]{34,139,34}{ness} \textcolor[RGB]{34,139,34}{ Disc}\textcolor[RGB]{34,139,34}{uss}\textcolor[RGB]{34,139,34}{ion} \textcolor[RGB]{34,139,34}{ Board} \textcolor[RGB]{34,139,34}{ »} \textcolor[RGB]{34,139,34}{ Fund}\textcolor[RGB]{34,139,34}{ament}\textcolor[RGB]{34,139,34}{als} \textcolor[RGB]{34,139,34}{ »} \textcolor[RGB]{30,144,255}{ Re}\textcolor[RGB]{34,139,34}{ag}\textcolor[RGB]{34,139,34}{ents} \textcolor[RGB]{34,139,34}{ and} \textcolor[RGB]{34,139,34}{ Appar}\textcolor[RGB]{34,139,34}{atus} \textcolor[RGB]{30,144,255}{ Ac}\textcolor[RGB]{34,139,34}{quisition} \textcolor[RGB]{34,139,34}{ »} \textcolor[RGB]{250,170,0}{ Sul}\textcolor[RGB]{250,128,114}{ph}\textcolor[RGB]{34,139,34}{ur}\textcolor[RGB]{34,139,34}{ic} \textcolor[RGB]{30,144,255}{ Ac}\textcolor[RGB]{34,139,34}{id} \textcolor[RGB]{250,128,114}{ in} \textcolor[RGB]{30,144,255}{ Australia} \textcolor[RGB]{30,144,255}{ Select} \textcolor[RGB]{34,139,34}{ A} \textcolor[RGB]{34,139,34}{ Forum} \textcolor[RGB]{34,139,34}{ Fund}\textcolor[RGB]{34,139,34}{ament}\textcolor[RGB]{34,139,34}{als} \textcolor[RGB]{34,139,34}{  } \textcolor[RGB]{34,139,34}{ »} \textcolor[RGB]{34,139,34}{ Chem}\textcolor[RGB]{34,139,34}{istry} \textcolor[RGB]{34,139,34}{ in} \textcolor[RGB]{34,139,34}{ General} \textcolor[RGB]{34,139,34}{  } \textcolor[RGB]{34,139,34}{ »} \textcolor[RGB]{34,139,34}{ Organ}\textcolor[RGB]{34,139,34}{ic} \textcolor[RGB]{34,139,34}{ Chem}\textcolor[RGB]{34,139,34}{istry} \textcolor[RGB]{34,139,34}{  } \textcolor[RGB]{34,139,34}{ »} \textcolor[RGB]{34,139,34}{ Re}\textcolor[RGB]{34,139,34}{ag}\textcolor[RGB]{34,139,34}{ents} \textcolor[RGB]{34,139,34}{ and} \textcolor[RGB]{34,139,34}{ Appar}\textcolor[RGB]{34,139,34}{atus} \textcolor[RGB]{34,139,34}{ Ac}\textcolor[RGB]{34,139,34}{quisition} \textcolor[RGB]{34,139,34}{  } \textcolor[RGB]{34,139,34}{ »} \textcolor[RGB]{34,139,34}{ Begin}\textcolor[RGB]{34,139,34}{nings} \textcolor[RGB]{34,139,34}{  } \textcolor[RGB]{34,139,34}{ »} \textcolor[RGB]{34,139,34}{ Res}\textcolor[RGB]{34,139,34}{p}\textcolor[RGB]{34,139,34}{ons}\textcolor[RGB]{34,139,34}{ible} \textcolor[RGB]{34,139,34}{ Pract}\textcolor[RGB]{34,139,34}{ices} \textcolor[RGB]{34,139,34}{  } \textcolor[RGB]{34,139,34}{ »} \textcolor[RGB]{34,139,34}{ Mis}\textcolor[RGB]{34,139,34}{cell}\textcolor[RGB]{34,139,34}{aneous} \textcolor[RGB]{34,139,34}{  } \textcolor[RGB]{34,139,34}{ »} \textcolor[RGB]{34,139,34}{ The} \textcolor[RGB]{34,139,34}{ Wik}\textcolor[RGB]{34,139,34}{i} \textcolor[RGB]{34,139,34}{ Special} \textcolor[RGB]{34,139,34}{ topics} \textcolor[RGB]{34,139,34}{  } \textcolor[RGB]{34,139,34}{ »} \textcolor[RGB]{34,139,34}{ Te}\textcolor[RGB]{34,139,34}{ch}\textcolor[RGB]{34,139,34}{no}\textcolor[RGB]{34,139,34}{chem}\textcolor[RGB]{34,139,34}{istry} \textcolor[RGB]{34,139,34}{  } \textcolor[RGB]{34,139,34}{ »} \textcolor[RGB]{34,139,34}{ Ener}\textcolor[RGB]{34,139,34}{get}\textcolor[RGB]{34,139,34}{ic} \textcolor[RGB]{34,139,34}{ Material}\textcolor[RGB]{34,139,34}{s} \textcolor[RGB]{34,139,34}{  } \textcolor[RGB]{34,139,34}{ »} \textcolor[RGB]{34,139,34}{ Bio}\textcolor[RGB]{34,139,34}{chem}\textcolor[RGB]{34,139,34}{istry} \textcolor[RGB]{34,139,34}{  } \textcolor[RGB]{34,139,34}{ »} \textcolor[RGB]{34,139,34}{ Radio}\textcolor[RGB]{34,139,34}{chem}\textcolor[RGB]{34,139,34}{istry} \textcolor[RGB]{34,139,34}{  } \textcolor[RGB]{34,139,34}{ »} \textcolor[RGB]{34,139,34}{ Comput}\textcolor[RGB]{34,139,34}{ational} \textcolor[RGB]{34,139,34}{ Mod}\textcolor[RGB]{34,139,34}{els} \textcolor[RGB]{34,139,34}{ and} \textcolor[RGB]{34,139,34}{ Te}\textcolor[RGB]{34,139,34}{chni}\textcolor[RGB]{34,139,34}{ques} \textcolor[RGB]{34,139,34}{  } \textcolor[RGB]{34,139,34}{ »} \textcolor[RGB]{34,139,34}{ P}\textcolor[RGB]{34,139,34}{rep}\textcolor[RGB]{34,139,34}{ublic}\textcolor[RGB]{34,139,34}{ation} \textcolor[RGB]{34,139,34}{ Non}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{chem}\textcolor[RGB]{34,139,34}{istry} \textcolor[RGB]{34,139,34}{  } \textcolor[RGB]{34,139,34}{ »} \textcolor[RGB]{34,139,34}{ Forum} \textcolor[RGB]{34,139,34}{ Mat}\textcolor[RGB]{34,139,34}{ters} \textcolor[RGB]{34,139,34}{  } \textcolor[RGB]{34,139,34}{ »} \textcolor[RGB]{34,139,34}{ Leg}\textcolor[RGB]{34,139,34}{al} \textcolor[RGB]{34,139,34}{ and} \textcolor[RGB]{34,139,34}{ Soci}\textcolor[RGB]{34,139,34}{etal} \textcolor[RGB]{34,139,34}{ Iss}\textcolor[RGB]{34,139,34}{ues} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Pages}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{  }\textcolor[RGB]{34,139,34}{1} \textcolor[RGB]{30,144,255}{  }\textcolor[RGB]{250,128,114}{2} \textcolor[RGB]{250,128,114}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Author}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ Sub}\textcolor[RGB]{30,144,255}{ject}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ Sul}\textcolor[RGB]{34,139,34}{ph}\textcolor[RGB]{34,139,34}{ur}\textcolor[RGB]{34,139,34}{ic} \textcolor[RGB]{34,139,34}{ Ac}\textcolor[RGB]{34,139,34}{id} \textcolor[RGB]{34,139,34}{ in} \textcolor[RGB]{34,139,34}{ Australia} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{h}\textcolor[RGB]{30,144,255}{iss}\textcolor[RGB]{30,144,255}{ing}\textcolor[RGB]{34,139,34}{no}\textcolor[RGB]{34,139,34}{ise} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{Intern}\textcolor[RGB]{34,139,34}{ational} \textcolor[RGB]{34,139,34}{ Haz}\textcolor[RGB]{34,139,34}{ard} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Post}\textcolor[RGB]{34,139,34}{s}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{30,144,255}{3}\textcolor[RGB]{30,144,255}{9}\textcolor[RGB]{30,144,255}{3}\textcolor[RGB]{30,144,255}{9} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Register}\textcolor[RGB]{34,139,34}{ed}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{30,144,255}{2}\textcolor[RGB]{30,144,255}{6}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{30,144,255}{1}\textcolor[RGB]{30,144,255}{2}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{2} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{Member} \textcolor[RGB]{34,139,34}{ Is} \textcolor[RGB]{34,139,34}{ Off}\textcolor[RGB]{34,139,34}{line} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{M}\textcolor[RGB]{34,139,34}{ood}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{30,144,255}{ Pul}\textcolor[RGB]{34,139,34}{ver}\textcolor[RGB]{34,139,34}{ules}\textcolor[RGB]{34,139,34}{cent}\textcolor[RGB]{34,139,34}{!} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{250,170,0}{I}\textcolor[RGB]{30,144,255}{'}\textcolor[RGB]{34,139,34}{ve} \textcolor[RGB]{30,144,255}{ stated} \textcolor[RGB]{250,170,0}{ several} \textcolor[RGB]{34,139,34}{ times} \textcolor[RGB]{250,170,0}{ on} \textcolor[RGB]{30,144,255}{ various} \textcolor[RGB]{250,128,114}{ threads}\textcolor[RGB]{30,144,255}{,} \textcolor[RGB]{30,144,255}{ that} \textcolor[RGB]{30,144,255}{ SO}\textcolor[RGB]{250,128,114}{<}\textcolor[RGB]{34,139,34}{sub}\textcolor[RGB]{34,139,34}{>}\textcolor[RGB]{30,144,255}{3}\textcolor[RGB]{34,139,34}{</}\textcolor[RGB]{34,139,34}{sub}\textcolor[RGB]{34,139,34}{>} \textcolor[RGB]{30,144,255}{ produces} \textcolor[RGB]{30,144,255}{ a} \textcolor[RGB]{250,170,0}{ pract}\textcolor[RGB]{34,139,34}{ically} \textcolor[RGB]{250,128,114}{ in}\textcolor[RGB]{250,170,0}{cond}\textcolor[RGB]{30,144,255}{ens}\textcolor[RGB]{250,128,114}{able} \textcolor[RGB]{250,128,114}{ acid} \textcolor[RGB]{30,144,255}{ mist} \textcolor[RGB]{30,144,255}{ when} \textcolor[RGB]{250,128,114}{ led} \textcolor[RGB]{30,144,255}{ to} \textcolor[RGB]{30,144,255}{ water} \textcolor[RGB]{250,128,114}{ and}\textcolor[RGB]{30,144,255}{,} \textcolor[RGB]{30,144,255}{ BTW}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{250,170,0}{ at} \textcolor[RGB]{250,170,0}{ }\textcolor[RGB]{250,170,0}{7}\textcolor[RGB]{30,144,255}{0}\textcolor[RGB]{250,128,114}{0}\textcolor[RGB]{250,170,0}{°}\textcolor[RGB]{34,139,34}{C} \textcolor[RGB]{250,170,0}{ the} \textcolor[RGB]{250,170,0}{ decomposition} \textcolor[RGB]{250,128,114}{ rate} \textcolor[RGB]{250,170,0}{ of} \textcolor[RGB]{34,139,34}{ SO}\textcolor[RGB]{34,139,34}{<}\textcolor[RGB]{34,139,34}{sub}\textcolor[RGB]{34,139,34}{>}\textcolor[RGB]{34,139,34}{3}\textcolor[RGB]{34,139,34}{</}\textcolor[RGB]{34,139,34}{sub}\textcolor[RGB]{34,139,34}{>} \textcolor[RGB]{34,139,34}{ is} \textcolor[RGB]{250,170,0}{ \~{}}\textcolor[RGB]{250,170,0}{8}\textcolor[RGB]{250,170,0}{7}\textcolor[RGB]{34,139,34}{\%} \textcolor[RGB]{30,144,255}{ .} \textcolor[RGB]{30,144,255}{ .} \textcolor[RGB]{34,139,34}{ .} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{250,128,114}{C}\textcolor[RGB]{250,128,114}{rack}\textcolor[RGB]{30,144,255}{ing} \textcolor[RGB]{30,144,255}{ Na}\textcolor[RGB]{30,144,255}{<}\textcolor[RGB]{34,139,34}{sub}\textcolor[RGB]{34,139,34}{>}\textcolor[RGB]{30,144,255}{2}\textcolor[RGB]{34,139,34}{</}\textcolor[RGB]{34,139,34}{sub}\textcolor[RGB]{34,139,34}{>}\textcolor[RGB]{30,144,255}{S}\textcolor[RGB]{34,139,34}{<}\textcolor[RGB]{34,139,34}{sub}\textcolor[RGB]{34,139,34}{>}\textcolor[RGB]{250,128,114}{2}\textcolor[RGB]{34,139,34}{</}\textcolor[RGB]{34,139,34}{sub}\textcolor[RGB]{34,139,34}{>}\textcolor[RGB]{30,144,255}{O}\textcolor[RGB]{34,139,34}{<}\textcolor[RGB]{34,139,34}{sub}\textcolor[RGB]{34,139,34}{>}\textcolor[RGB]{30,144,255}{7}\textcolor[RGB]{34,139,34}{</}\textcolor[RGB]{34,139,34}{sub}\textcolor[RGB]{34,139,34}{>} \textcolor[RGB]{30,144,255}{ proceed}\textcolor[RGB]{34,139,34}{s} \textcolor[RGB]{250,128,114}{ at} \textcolor[RGB]{250,170,0}{ \~{}}\textcolor[RGB]{250,170,0}{4}\textcolor[RGB]{250,128,114}{6}\textcolor[RGB]{250,170,0}{6}\textcolor[RGB]{34,139,34}{°}\textcolor[RGB]{34,139,34}{C} \textcolor[RGB]{250,170,0}{ and} \textcolor[RGB]{250,170,0}{ the} \textcolor[RGB]{250,128,114}{ issu}\textcolor[RGB]{34,139,34}{ing} \textcolor[RGB]{30,144,255}{ g}\textcolor[RGB]{30,144,255}{ass}\textcolor[RGB]{34,139,34}{es} \textcolor[RGB]{34,139,34}{ are} \textcolor[RGB]{30,144,255}{ readily} \textcolor[RGB]{30,144,255}{ absor}\textcolor[RGB]{34,139,34}{bed} \textcolor[RGB]{30,144,255}{ by} \textcolor[RGB]{30,144,255}{ conc}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{34,139,34}{ H}\textcolor[RGB]{34,139,34}{<}\textcolor[RGB]{34,139,34}{sub}\textcolor[RGB]{34,139,34}{>}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{</}\textcolor[RGB]{34,139,34}{sub}\textcolor[RGB]{34,139,34}{>}\textcolor[RGB]{30,144,255}{SO}\textcolor[RGB]{34,139,34}{<}\textcolor[RGB]{34,139,34}{sub}\textcolor[RGB]{34,139,34}{>}\textcolor[RGB]{30,144,255}{4}\textcolor[RGB]{34,139,34}{</}\textcolor[RGB]{34,139,34}{sub}\textcolor[RGB]{34,139,34}{>} \textcolor[RGB]{250,128,114}{ to} \textcolor[RGB]{34,139,34}{ form} \textcolor[RGB]{30,144,255}{ o}\textcolor[RGB]{30,144,255}{le}\textcolor[RGB]{34,139,34}{um}\textcolor[RGB]{30,144,255}{!} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{30,144,255}{Ph}\textcolor[RGB]{250,128,114}{th}\textcolor[RGB]{34,139,34}{al}\textcolor[RGB]{30,144,255}{ic} \textcolor[RGB]{30,144,255}{ Ac}\textcolor[RGB]{34,139,34}{id} \textcolor[RGB]{250,128,114}{ \textbackslash n }\textcolor[RGB]{250,128,114}{Har}\textcolor[RGB]{34,139,34}{ml}\textcolor[RGB]{34,139,34}{ess} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Post}\textcolor[RGB]{34,139,34}{s}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{30,144,255}{1}\textcolor[RGB]{250,128,114}{9} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Register}\textcolor[RGB]{34,139,34}{ed}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{30,144,255}{7}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{250,170,0}{8}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{250,128,114}{1}\textcolor[RGB]{30,144,255}{1} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Location}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{30,144,255}{ Australia} \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Member} \textcolor[RGB]{34,139,34}{ Is} \textcolor[RGB]{34,139,34}{ Off}\textcolor[RGB]{34,139,34}{line} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{M}\textcolor[RGB]{34,139,34}{ood}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ No} \textcolor[RGB]{34,139,34}{ M}\textcolor[RGB]{34,139,34}{ood} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{250,128,114}{That}\textcolor[RGB]{34,139,34}{'}\textcolor[RGB]{34,139,34}{s} \textcolor[RGB]{250,128,114}{ a} \textcolor[RGB]{30,144,255}{ good} \textcolor[RGB]{30,144,255}{ idea} \textcolor[RGB]{30,144,255}{ Neil}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ I}\textcolor[RGB]{34,139,34}{'}\textcolor[RGB]{34,139,34}{ll} \textcolor[RGB]{250,170,0}{ be} \textcolor[RGB]{30,144,255}{ sure} \textcolor[RGB]{34,139,34}{ to} \textcolor[RGB]{250,128,114}{ try} \textcolor[RGB]{34,139,34}{ that} \textcolor[RGB]{250,128,114}{ next} \textcolor[RGB]{34,139,34}{ time} \textcolor[RGB]{250,128,114}{ (}\textcolor[RGB]{30,144,255}{pro}\textcolor[RGB]{34,139,34}{bably} \textcolor[RGB]{250,128,114}{ for} \textcolor[RGB]{250,128,114}{ H}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{250,128,114}{O}\textcolor[RGB]{30,144,255}{2}\textcolor[RGB]{250,170,0}{).} \textcolor[RGB]{30,144,255}{ Just} \textcolor[RGB]{250,170,0}{ went} \textcolor[RGB]{34,139,34}{ to} \textcolor[RGB]{250,128,114}{ Tr}\textcolor[RGB]{30,144,255}{adel}\textcolor[RGB]{250,128,114}{ink} \textcolor[RGB]{34,139,34}{ and} \textcolor[RGB]{250,128,114}{ asked} \textcolor[RGB]{250,170,0}{ if} \textcolor[RGB]{34,139,34}{ they} \textcolor[RGB]{250,170,0}{ sold} \textcolor[RGB]{250,170,0}{ M}\textcolor[RGB]{250,128,114}{of}\textcolor[RGB]{250,128,114}{lo} \textcolor[RGB]{250,128,114}{ d}\textcolor[RGB]{30,144,255}{rain} \textcolor[RGB]{34,139,34}{ cleaner}\textcolor[RGB]{250,128,114}{.} \textcolor[RGB]{30,144,255}{ The} \textcolor[RGB]{34,139,34}{ gu}\textcolor[RGB]{34,139,34}{y} \textcolor[RGB]{34,139,34}{ said} \textcolor[RGB]{30,144,255}{ yeah} \textcolor[RGB]{250,170,0}{ and} \textcolor[RGB]{250,128,114}{ I} \textcolor[RGB]{30,144,255}{ asked} \textcolor[RGB]{30,144,255}{ for} \textcolor[RGB]{250,128,114}{ a} \textcolor[RGB]{30,144,255}{ liter} \textcolor[RGB]{30,144,255}{ of} \textcolor[RGB]{34,139,34}{ it}\textcolor[RGB]{250,128,114}{.} \textcolor[RGB]{250,128,114}{ No} \textcolor[RGB]{30,144,255}{ problems} \textcolor[RGB]{250,128,114}{ what}\textcolor[RGB]{34,139,34}{so}\textcolor[RGB]{34,139,34}{ever}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{30,144,255}{ he} \textcolor[RGB]{250,170,0}{ just} \textcolor[RGB]{250,170,0}{ said} \textcolor[RGB]{250,170,0}{ ''}\textcolor[RGB]{250,170,0}{be} \textcolor[RGB]{250,128,114}{ careful} \textcolor[RGB]{250,128,114}{ with} \textcolor[RGB]{30,144,255}{ it}\textcolor[RGB]{250,170,0}{''.} \textcolor[RGB]{250,170,0}{ It} \textcolor[RGB]{250,170,0}{ was} \textcolor[RGB]{250,170,0}{ \$}\textcolor[RGB]{250,170,0}{4}\textcolor[RGB]{30,144,255}{5} \textcolor[RGB]{250,128,114}{ but} \textcolor[RGB]{250,170,0}{ a} \textcolor[RGB]{30,144,255}{ liter} \textcolor[RGB]{250,170,0}{ will} \textcolor[RGB]{34,139,34}{ last} \textcolor[RGB]{34,139,34}{ me} \textcolor[RGB]{34,139,34}{ a} \textcolor[RGB]{250,128,114}{ while} \textcolor[RGB]{30,144,255}{ and} \textcolor[RGB]{30,144,255}{ making} \textcolor[RGB]{30,144,255}{ it} \textcolor[RGB]{30,144,255}{ myself} \textcolor[RGB]{30,144,255}{ would}\textcolor[RGB]{250,128,114}{'}\textcolor[RGB]{34,139,34}{ve} \textcolor[RGB]{34,139,34}{ been} \textcolor[RGB]{250,170,0}{ vast}\textcolor[RGB]{34,139,34}{ly} \textcolor[RGB]{34,139,34}{ more} \textcolor[RGB]{34,139,34}{ expensive} \textcolor[RGB]{30,144,255}{ I} \textcolor[RGB]{30,144,255}{ imagine}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{250,128,114}{ Success}\textcolor[RGB]{34,139,34}{!} \textcolor[RGB]{250,128,114}{ Me}\textcolor[RGB]{30,144,255}{Syn}\textcolor[RGB]{250,128,114}{th} \textcolor[RGB]{30,144,255}{ Haz}\textcolor[RGB]{34,139,34}{ard} \textcolor[RGB]{30,144,255}{ to} \textcolor[RGB]{30,144,255}{ O}\textcolor[RGB]{34,139,34}{thers} \textcolor[RGB]{34,139,34}{ Post}\textcolor[RGB]{34,139,34}{s}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{30,144,255}{1}\textcolor[RGB]{250,128,114}{0}\textcolor[RGB]{250,170,0}{7} \textcolor[RGB]{34,139,34}{ Register}\textcolor[RGB]{34,139,34}{ed}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{250,170,0}{9}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{250,170,0}{7}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{1} \textcolor[RGB]{30,144,255}{ Member} \textcolor[RGB]{34,139,34}{ Is} \textcolor[RGB]{34,139,34}{ Off}\textcolor[RGB]{34,139,34}{line} \textcolor[RGB]{34,139,34}{ M}\textcolor[RGB]{34,139,34}{ood}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{30,144,255}{ http}\textcolor[RGB]{34,139,34}{://}\textcolor[RGB]{34,139,34}{www}\textcolor[RGB]{34,139,34}{.}\textcolor[RGB]{30,144,255}{youtube}\textcolor[RGB]{34,139,34}{.}\textcolor[RGB]{34,139,34}{com}\textcolor[RGB]{34,139,34}{/}\textcolor[RGB]{34,139,34}{watch}\textcolor[RGB]{34,139,34}{?}\textcolor[RGB]{34,139,34}{v}\textcolor[RGB]{34,139,34}{=}\textcolor[RGB]{250,128,114}{5}\textcolor[RGB]{30,144,255}{Z}\textcolor[RGB]{250,170,0}{lt}\textcolor[RGB]{250,170,0}{ql}\textcolor[RGB]{250,170,0}{V}\textcolor[RGB]{250,170,0}{u}\textcolor[RGB]{250,170,0}{DI}\textcolor[RGB]{30,144,255}{o} \textcolor[RGB]{250,170,0}{ Sul}\textcolor[RGB]{30,144,255}{fur}\textcolor[RGB]{34,139,34}{ic} \textcolor[RGB]{34,139,34}{ acid} \textcolor[RGB]{250,170,0}{ can} \textcolor[RGB]{34,139,34}{ be} \textcolor[RGB]{250,170,0}{ produced} \textcolor[RGB]{250,128,114}{ in} \textcolor[RGB]{250,170,0}{ the} \textcolor[RGB]{250,170,0}{ labor}\textcolor[RGB]{34,139,34}{atory} \textcolor[RGB]{30,144,255}{ by} \textcolor[RGB]{30,144,255}{ burning} \textcolor[RGB]{250,128,114}{ sul}\textcolor[RGB]{34,139,34}{fur} \textcolor[RGB]{30,144,255}{ in} \textcolor[RGB]{30,144,255}{ air} \textcolor[RGB]{250,128,114}{ and} \textcolor[RGB]{250,170,0}{ dissol}\textcolor[RGB]{34,139,34}{ving} \textcolor[RGB]{250,128,114}{ the} \textcolor[RGB]{250,170,0}{ gas} \textcolor[RGB]{250,170,0}{ produced} \textcolor[RGB]{34,139,34}{ in} \textcolor[RGB]{250,170,0}{ a} \textcolor[RGB]{30,144,255}{ hydro}\textcolor[RGB]{250,128,114}{gen} \textcolor[RGB]{30,144,255}{ per}\textcolor[RGB]{34,139,34}{ox}\textcolor[RGB]{34,139,34}{ide} \textcolor[RGB]{34,139,34}{ solution}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{30,144,255}{ SO}\textcolor[RGB]{34,139,34}{2} \textcolor[RGB]{34,139,34}{ +} \textcolor[RGB]{30,144,255}{ H}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{O}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ →} \textcolor[RGB]{34,139,34}{ H}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{SO}\textcolor[RGB]{250,128,114}{4} \textcolor[RGB]{30,144,255}{ this} \textcolor[RGB]{250,170,0}{ was} \textcolor[RGB]{250,128,114}{ found} \textcolor[RGB]{30,144,255}{ on} \textcolor[RGB]{250,170,0}{ w}\textcolor[RGB]{34,139,34}{ik}\textcolor[RGB]{34,139,34}{ipedia}\textcolor[RGB]{30,144,255}{...} \textcolor[RGB]{30,144,255}{ did} \textcolor[RGB]{34,139,34}{ you} \textcolor[RGB]{250,128,114}{ not} \textcolor[RGB]{30,144,255}{ look} \textcolor[RGB]{250,170,0}{ through} \textcolor[RGB]{250,128,114}{ the} \textcolor[RGB]{250,128,114}{ sull}\textcolor[RGB]{250,128,114}{fur}\textcolor[RGB]{30,144,255}{ic} \textcolor[RGB]{34,139,34}{ acid} \textcolor[RGB]{250,170,0}{ w}\textcolor[RGB]{34,139,34}{iki} \textcolor[RGB]{30,144,255}{ before} \textcolor[RGB]{30,144,255}{ bo}\textcolor[RGB]{30,144,255}{iling} \textcolor[RGB]{30,144,255}{ down} \textcolor[RGB]{30,144,255}{ bat}\textcolor[RGB]{30,144,255}{ery} \textcolor[RGB]{34,139,34}{ acid}\textcolor[RGB]{34,139,34}{?} \textcolor[RGB]{30,144,255}{ any}\textcolor[RGB]{30,144,255}{ways}\textcolor[RGB]{30,144,255}{...} \textcolor[RGB]{250,170,0}{ There} \textcolor[RGB]{34,139,34}{ are} \textcolor[RGB]{30,144,255}{ some} \textcolor[RGB]{250,128,114}{ good} \textcolor[RGB]{250,128,114}{ videos} \textcolor[RGB]{34,139,34}{ on} \textcolor[RGB]{34,139,34}{ you}\textcolor[RGB]{34,139,34}{t}\textcolor[RGB]{34,139,34}{ube} \textcolor[RGB]{250,128,114}{ that} \textcolor[RGB]{250,170,0}{ demonstrate} \textcolor[RGB]{250,170,0}{ how} \textcolor[RGB]{30,144,255}{ to} \textcolor[RGB]{250,128,114}{ synth}\textcolor[RGB]{34,139,34}{es}\textcolor[RGB]{34,139,34}{ize} \textcolor[RGB]{34,139,34}{ sul}\textcolor[RGB]{34,139,34}{fur}\textcolor[RGB]{34,139,34}{ic} \textcolor[RGB]{34,139,34}{ acid} \textcolor[RGB]{250,170,0}{ using} \textcolor[RGB]{250,128,114}{ different} \textcolor[RGB]{34,139,34}{ methods}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{250,170,0}{ The} \textcolor[RGB]{30,144,255}{ d}\textcolor[RGB]{30,144,255}{rain} \textcolor[RGB]{34,139,34}{ cleaner} \textcolor[RGB]{250,128,114}{ you} \textcolor[RGB]{250,170,0}{ get} \textcolor[RGB]{250,128,114}{ from} \textcolor[RGB]{250,128,114}{ the} \textcolor[RGB]{30,144,255}{ store} \textcolor[RGB]{250,128,114}{ will} \textcolor[RGB]{250,128,114}{ be} \textcolor[RGB]{30,144,255}{ imp}\textcolor[RGB]{34,139,34}{ure} \textcolor[RGB]{250,170,0}{ and} \textcolor[RGB]{250,128,114}{ may} \textcolor[RGB]{34,139,34}{ contain} \textcolor[RGB]{250,128,114}{ organ}\textcolor[RGB]{34,139,34}{ic} \textcolor[RGB]{30,144,255}{ matter} \textcolor[RGB]{250,170,0}{ that} \textcolor[RGB]{250,128,114}{ dis}\textcolor[RGB]{250,170,0}{colors} \textcolor[RGB]{34,139,34}{ the} \textcolor[RGB]{30,144,255}{ acid}\textcolor[RGB]{34,139,34}{.}
\\ \bottomrule
\end{tabular}
}
\caption{\textbf{Sample text containing four categories of tokens.} Among them, \textcolor[RGB]{30,144,255}{blue} represents tokens of categorie H→L, \textcolor[RGB]{34,139,34}{green} indicates tokens of categorie L→L, \textcolor[RGB]{250,170,0}{yellow} signifies tokens of categorie H→H, and \textcolor[RGB]{250,128,114}{red} denotes tokens of categorie L→H.}
\label{tab:hhll_case}
\end{table*}

==> table/lossyref_result.tex <==
\begin{table*}[t]
\centering
\small
% \setlength{\tabcolsep}{2pt}
\caption{The results of training TinyLLaMA using the Lossy Reference Model, with a total of 15B tokens trained.}
\label{tab:lossy_ref_result}
\begin{tabular}{l|ccccc|c}
\toprule
\textbf{Model} & \textbf{GSM8K} & \textbf{MATH} & \textbf{SVAMP} & \textbf{ASDiv} & \textbf{MAWPS} & \textbf{AVG} \\
\midrule
Tinyllama-CT & 6.4 & 2.4 & 21.7 & 36.7 & 47.7 & 23.0 \\
Tinyllama-CT w/LRM  & 12.1 & 10.6 & 36.9 & 51.0 & 68.7 & 35.9 \\
\bottomrule
\end{tabular}
\end{table*}

==> table/main_general_results.tex <==
\begin{table*}[t]
\center
\caption{The main results of the \model{} on benchmarks. \textbf{MMLU} and \textbf{BBH} are evaluated using 5-shot and 3-shot prompting, respectively.}
\label{tab:diversityresult}
\setlength\tabcolsep{3pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcc|ccccccccccc|c}
\toprule
{\textbf{Model}} & $|\boldsymbol{\theta}|$ & \textbf{Toks} & \textbf{MMLU} & \textbf{BBH} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}AGI\\ Eval\end{tabular}}} & \textbf{HS} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}ARC\\ Chlg\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}ARC\\ Easy\end{tabular}}} & \textbf{WG} & \textbf{Piqa} & \textbf{BQ} & \textbf{Obqa} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Tydi \\ QA\end{tabular}}} & \textbf{AVG} \\ \midrule
\multicolumn{15}{c}{\texttt{1-2B Base Models}}
\\ \midrule
\href{https://huggingface.co/TinyLlama/TinyLlama-1.1B-intermediate-step-1195k-token-2.5T}{TinyLLaMA} & 1.1B & - & 25.9 & 29.3 & 30.8 & 59.0 & 31.9 & 56.8  & 58.7 & 73.1 & 63.2 & 34.4 & 26.4 & 44.5 \\
% \href{https://huggingface.co/facebook/opt-1.3b}{Opt} & 1.3B & - & 25.0 & 22.6 & 31.7 & 53.7 & 29.4 & 51.0 & 59.4 & 72.4 & 57.7 & 33.2 & 7.5 & 40.3 \\
% \href{https://huggingface.co/bigscience/bloom-1b7}{Bloom} & 1.7B & - & 25.2 & 17.3 & 31.1 & 48.0 & 27.1 & 48.1 & 57.4 & 70.0 & 61.8 & 30.0 & 10.5 & 38.8 \\
% \href{https://huggingface.co/bigscience/bloom-1b1}{Bloom} & 1.1B & - & 24.1 & 18.5 & 31.3 & 43.0 & 25.5 & 45.4 & 55.3 & 67.1 & 59.1 & 29.4 & 10.2 & 37.2 \\
%\href{https://huggingface.co/microsoft/phi-1_5}{Phi-1.5} & 1.3B & - & 40.7 & 28.8 & 32.4 & 62.6 & 48.0 & 73.1 & 72.7 & 75.5 & 75.0 & 48.2 & 7.3 & \\
% \href{https://huggingface.co/EleutherAI/pythia-1.4b}{Pythia} & 1.4B & - & 24.4 & 25.1 & 30.9 & 52.0 & 28.6 & 53.9 & 57.1 & 71.1 & 63.5 & 33.2 & 12.9 & 41.2 \\
% \href{https://huggingface.co/EleutherAI/pythia-1b}{Pythia} & 1.0B & - & 23.3 & 25.1 & 30.3 & 47.1 & 27.0 & 49.0 & 53.7 & 69.3 & 60.8 & 31.4 & 6.3 & 38.5 \\
%\href{https://huggingface.co/google/gemma-2b}{Gemma} & 2.0B & - & 27.0 & 34.1 & 31.2 & 42.3 & 23.0 & 37.1 & 50.3 & 59.6 & 63.0 & 27.8 & \\
% \midrule
% \multicolumn{15}{c}{\texttt{Continue Pretraining on Tinyllama 1.1B}}
% \\ \midrule
TinyLLaMA-CT & 1.1B & 80B & 25.3 & 28.2 & 31.3 & 56.6 & 30.0 & 55.7 & 59.1 & 72.2 & 63.2 & 34.6 & 21.1 & 43.4 \\
\model{}-Base & 1.1B & 48B & \hl{36.6} & \hl{32.1} & \hl{32.4} & \hl{58.0} & \hl{35.0} & \hl{64.3} & \hl{59.3} & \hl{73.1} & \hl{74.5} & \hl{38.0} & \hl{30.0} & \hl{48.5} \\
% $\Delta$ & & \grey{-40\%} & \blue{+11.3} & \blue{+3.9} & \blue{+1.1} & \blue{+1.4} & \blue{+5.0} & \blue{+8.6} & \blue{+0.2} & \blue{+0.9} & \blue{+11.3} & \blue{+3.4} & \blue{+8.9} & \blue{\textbf{+5.1}} \\
% TrimLoss
\bottomrule
\end{tabular}
}
\end{table*}

\begin{table*}[t]
\center
\footnotesize
\setlength\tabcolsep{4pt}
\caption{The main results of the \model{}-1.1B on code and math.}
\label{tab:diversityresult}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcc|cccc|cc|c}
\toprule
{\textbf{Model}} & $|\boldsymbol{\theta}|$ & \textbf{Toks} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{HumanEval}\\ pass@1\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{HumanEval}\\ pass@10\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{MBPP}\\ pass@1\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{MBPP}\\ pass@10\end{tabular}} & \textbf{GSM8K} & \textbf{Math} & \textbf{AVG} \\ 
\midrule
\multicolumn{10}{c}{\texttt{1-2B Base Models}}
\\ \midrule
\href{https://huggingface.co/TinyLlama/TinyLlama-1.1B-intermediate-step-1195k-token-2.5T}{TinyLLaMA} & 1.1B & - & 8.7 & 10.3 & 14.4 & 21.6 & 2.9 & 3.0 & 10.2 \\
%\href{https://huggingface.co/facebook/opt-1.3b}{Opt} & 1.3B & - & 0.0 & 0.0 & - & - & 2.7 & 2.2 & \\
% \href{https://huggingface.co/bigscience/bloom-1b7}{Bloom} & 1.7B & - & 4.0 & 7.5 & 5.5 & 9.6 & 2.6 & 3.2 & 5.4 \\
% \href{https://huggingface.co/bigscience/bloom-1b1}{Bloom} & 1.1B & - & 2.5 & 5.9 & 2.8 & 4.8 & 2.7 & 2.6 & 3.6 \\
%\href{https://huggingface.co/microsoft/phi-1_5}{Phi-1.5} & 1.3B & - & 33.9 & 42.7 & - & - & 32.4 & 4.2 & \\
% \href{https://huggingface.co/EleutherAI/pythia-1.4b}{Pythia} & 1.4B & - & 4.1 & 6.1 & 3.7 & 8.0 & 1.7 & 2.6 & 4.4 \\
% \href{https://huggingface.co/EleutherAI/pythia-1b}{Pythia} & 1.0B & - & 5.9 & 6.7 & 3.0 & 5.6 & 2.3 & 3.0 & 4.4 \\
% \midrule
% \multicolumn{10}{c}{\texttt{Continue Pretraining on Tinyllama 1.1B}}
% \\ \midrule
TinyLLaMA-CT & 1.1B & 80B & 9.0 & 10.7 & 12.2 & 18.2 & 2.7 & 3.2 & 9.3 \\
\model{}-Base & 1.1B & 48B & \hl{15.9} & \hl{21.3} & \hl{18.7} & \hl{26.0} & \hl{30.9} & \hl{8.2} & \hl{20.2} \\
% $\Delta$ & & \grey{-40\%} & \blue{+6.9} & \blue{+10.6} & \blue{+6.5} & \blue{+7.8} & \blue{+28.2} & \blue{+5.0} & \blue{\textbf{+10.9}} \\
% TrimLoss
\bottomrule
\end{tabular}
}
\end{table*}

==> table/main_math_results.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{2pt}
\caption{
\textbf{Few-shot CoT reasoning results of math pretraining.} All models are tested with few-shot prompting. Previous best results are highlighted in \hlb{blue}, while our best results are in \hl{purple}. $^*$Only unique math-related tokens are calculated. For \model{}, we calculate only the selected tokens that are used for training. $^\dagger$We use OpenAI's MATH subset \citep{lightman2023let} for evaluation, since some original test samples have been used in public training sets such as PRM800k. $^\ddagger$The SAT only has 32 four-choice problems, so we average our results over the last three checkpoints, if available.
}
\label{tab:math-cot-result}
\resizebox{\linewidth}{!}{
\begin{tabular}{lrcrr|ccccccccc|c}
\toprule
\textbf{Model} & $|\boldsymbol{\theta}|$ & \textbf{Data} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Uniq.\\ Toks$^*$\end{tabular}}}& \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Train\\ Toks\end{tabular}}} & \textbf{GSM8K} & \textbf{MATH$^\dagger$} & \textbf{SVAMP} & \textbf{ASDiv} & \textbf{MAWPS} & \textbf{TAB}& \textbf{MQA} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}MMLU\\ STEM\end{tabular}}} & \textbf{SAT$^\ddagger$} & \textbf{AVG} \\
\midrule
\multicolumn{15}{c}{\texttt{1-2B Base Models}} \\
\midrule
\href{https://huggingface.co/Tinyllama/Tinyllama-1.1B-intermediate-step-1431k-3T}{Tinyllama}& 1.1B & - & - & - & 2.9 & 3.2 & 11.0 & 18.1 & 20.4 & 12.5 & 14.6 & 16.1 & 21.9 & 13.4 \\
\href{https://huggingface.co/microsoft/phi-1_5}{Phi-1.5} & 1.3B & - & - & - & 32.4 & 4.2 & 43.4 & 53.1 & 66.2 & 24.4 & 14.3 & 21.8 & 18.8 & 31.0 \\
\href{https://huggingface.co/Qwen/Qwen1.5-1.8B}{Qwen1.5} & 1.8B & - & - & - & \hlb{36.1} & 6.8 & \hlb{48.5} & \hlb{63.6} & \hlb{79.0} & 29.2 & 25.1 & 31.3 & 40.6 & \hlb{40.0} \\
\href{https://huggingface.co/google/gemma-2b}{Gemma} & 2.0B & - & - & - & 18.8 & 11.4 & 38.0 & 56.6 & 72.5 & \hlb{36.9} & \hlb{26.8} & \hlb{34.4} & 50.0 & 38.4 \\ 
% \href{https://huggingface.co/openbmb/MiniCPM-2B-sft-bf16}{MiniCPM} & 2.4B& - & - & - & 52.7 & 16.0 & 67.0 & 73.2 & 90.1 & 37.6 & 40.9 & 43.1 & 46.9 & 51.9 \\
% \href{https://huggingface.co/microsoft/phi-2}{Phi2} & 2.7B & - & - & - & 55.3 & 11.8 & 65.4 & 75.5 & 84.0 & 43.6 & 38.2 & 47.9 & 40.6 & 51.4 \\
DeepSeekLLM & 1.3B & OWM & 14B & 150B & 11.5 & 8.9 & - & - & - & -  & - & 29.6 & 31.3 & -\\
% DeepSeekLLM-1.3B & Proof-Pile-2 & 55B & 150B & 14.3 & 11.2 & - & - & - & - \\
DeepSeekMath & 1.3B & - & 120B & 150B & 23.8 & \hlb{13.6} & - & - & - & - & - & {33.1} & \hlb{56.3} & - \\
\midrule
\multicolumn{15}{c}{\texttt{Continual Pretraining on Tinyllama-1B}}
\\ \midrule
% Tinyllama-1B & Proof-Pile-2 & 55B & 100B & 8.9 & 6.0 & 25.6 & 42.1 & 53.6 & 27.2 \\
Tinyllama-CT & 1.1B & OWM & 14B & 15B & 6.4 & 2.4 & 21.7 & 36.7 & 47.7 & 17.9 & 13.9 & 23.0 & 25.0 & 21.6 \\
\model{}-Math & 1.1B & OWM & 14B & {9B} & 29.8 & 14.0 & 49.2 & 61.4 & 79.8 & 25.8 & 30.4 & \hl{24.7} & 28.1 & 38.1 \\
$\Delta$  & & & & \grey{-40\%} & \blue{+23.4} & \blue{+11.6} & \blue{+27.5} & \blue{+24.7} & \blue{+32.1} & \blue{+7.9} & \blue{+16.5} & \blue{+1.7} & \blue{+3.1} & \blue{\textbf{+16.5}} \\
% {\model{}-Math t4} & 1.1B & OWM & 14B & {9B} & 30.1 & 12.2 & 45.4 & 60.1 & 77.6 & 22.6 & 27.3 & \hl{24.1} & 24.0 & 35.9\\
% $\Delta$ T4 & & & & \grey{-6B} & \blue{+23.7} & \blue{+9.8} & \blue{+23.7} & \blue{+23.4} & \blue{+29.9} & \blue{+4.7} & \blue{+13.4} & \blue{+1.1} & \blue{-1.0} & \blue{\textbf{+14.3}}\\  
\midrule
\model{}-Math & 1.1B & OWM & 14B & {30B} & \hl{36.2} & \hl{15.6} & \hl{52.1} & \hl{67.0} & \hl{83.9} & \hl{29.0} & \hl{32.5} & {23.3} & \hl{28.1} & \hl{40.9} \\
\midrule
\multicolumn{15}{c}{\texttt{$\ge$ 7B Base Models}}
\\ \midrule
\href{https://huggingface.co/meta-llama/Llama-2-7b-hf}{LLaMA-2} & 7B & & - & - & 14.0 & 3.6 & 39.5 & 51.7 & 63.5 & 30.9 & 12.4 & 32.7 & 34.4 & 31.4 \\
% \href{https://huggingface.co/codellama/CodeLlama-7b-Python-hf}{CodeLlama} & 7B & & - & - & 12.4 & 7.0 & 44.5 & 49.0 & 64.9 & 25.5 & 17.2 & 24.1 & 34.4 & 31.0 \\ 
\href{https://huggingface.co/mistralai/Mistral-7B-v0.1}{Mistral} & 7B & & - & - & 41.2 & 11.6 & 64.7 & 68.5 & 87.5 & 52.9 & 33.0 & 49.5 & 59.4 & 52.0 \\
Minerva & 8B & - & 39B & 164B & 16.2 & 14.1 & -& -& -& -& -& 35.6 & - & - \\
Minerva & 62B & - & 39B & 109B & 52.4 & 27.6 & -& -& -& -& -& 53.9 & - & - \\
Minerva & 540B & - & 39B & 26B & 58.8 & {33.6} & -& -& -& -& -& \hlb{63.9} & - & - \\
\href{https://huggingface.co/EleutherAI/llemma_7b}{LLemma} & 7B & PPile & 55B & 200B & 38.8 & 17.2 & 56.1 & 69.1 & 82.4 & 48.7 & 41.0 & 45.4 & 59.4 & 50.9 \\
\href{https://huggingface.co/EleutherAI/llemma_34b}{LLemma} & 34B & PPile & 55B & 50B & 54.2 & 23.0 & 67.9 & {75.7} & 90.1 & 57.0 & 49.8 & 54.7 & 68.8 & 60.1 \\
\href{https://huggingface.co/internlm/internlm2-math-base-7b}{Intern-Math} & 7B & - & 31B & 125B & 41.8 & 14.4 & 61.6 & 66.8 & 83.7 & 50.0 & 57.3  & 24.8 & 37.5 & 48.7 \\
\href{https://huggingface.co/internlm/internlm2-math-base-20b}{Intern-Math} & 20B & - & 31B & 125B & \hlb{65.4} & 30.0 & \hlb{75.7} & 79.3 & \hlb{94.0} & 50.9 & 38.5 & 53.1 & 71.9 & 62.1\\
\href{https://huggingface.co/deepseek-ai/deepseek-math-7b-base}{DeepSeekMath} & 7B & - & 120B & 500B & {64.1} & \hlb{34.2} & {74.0} & \hlb{83.9} & {92.4} & \hlb{63.4} & \hlb{62.4} & 56.4 & \hlb{84.4} & \hlb{68.4} \\
\midrule
\multicolumn{15}{c}{\texttt{Continual Pretraining on Mistral-7B}} \\
\midrule
Mistral-CT & 7B & OWM & 14B & 15B & 42.9 & 22.2 & 68.6 & 71.0 & 86.1 & 45.1 & 47.7 & 52.6 & 65.6 & 55.8\\
\model{}-Math & 7B & OWM & 14B & {10.5B} & \hl{66.9} & \hl{31.0} & \hl{77.8} & \hl{79.0} & \hl{93.9} & \hl{49.9} & \hl{58.7} & \hl{54.6} & \hl{84.4} & \hl{66.2}\\
$\Delta$  & & & & \grey{-30\%} & \blue{+24.0} & \blue{+8.8} & \blue{+9.2} & \blue{+8.0} & \blue{+7.8} & \blue{+4.8} & \blue{+11.0} & \blue{+2.0} & \blue{+18.8} &  \blue{\textbf{+10.4}}\\  
\bottomrule
\end{tabular}
}
\end{table*}


==> table/maskratio_result.tex <==
\begin{table*}[t]
\centering
\small
% \setlength{\tabcolsep}{2pt}
\caption{Compare the results of directly selecting token training models based on the reference model under different mask ratios.}
\label{tab:lossy_ref_result}
\begin{tabular}{l|cccccc|c}
\toprule
\textbf{Model} & \textbf{} & \textbf{GSM8K} & \textbf{MATH} & \textbf{SVAMP} & \textbf{ASDiv} & \textbf{MAWPS} & \textbf{AVG} \\
\midrule
Tinyllama-CT & 6.4 & 3.6 & 21.0 & 34.4 & 48.2 & 22.7 \\
Lossy Reference Model & 12.3 & 5.4 & 25.2 & 35.8 & 43.8 & 24.5 \\
Tinyllama-CT w/LRM  & 12.1 & 5.6 & 29.6 & 43.3 & 53.2 & 28.8 \\
\bottomrule
\end{tabular}
\end{table*}

==> table/math_tora_results.tex <==
\begin{table}[t]
\caption{\textbf{Tool-integrated reasoning results of math pretraining.}}
\label{tab:math-tora}
\centering
\setlength{\tabcolsep}{5pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{lrcc|ccccccc|c}
\toprule
\textbf{Model} & \textbf{Size} & \textbf{Tools} & \textbf{SFT Data} & \textbf{GSM8k} & \textbf{MATH} 
 & \textbf{SVAMP} &  \textbf{ASDiv} & \multicolumn{1}{c}{\textbf{MAWPS}} & \textbf{TAB} & \textbf{GSM-H} & \multirow{2}{*}{\textbf{AVG}} \\
\cmidrule{1-11}
\multicolumn{4}{l|}{\textbf{Used for SFT?}} & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \\
\midrule
\multicolumn{12}{c}{\texttt{Previous Models}} \\
\midrule
GPT4-0314 & - & \xmark & - &  92.0 & 42.5 & 93.1  & 91.3 & 97.6  & 67.1 & 64.7 & 78.3\\
GPT4-0314 (PAL) & - & \cmark & - & 94.2 & 51.8 & 94.8  & 92.6 & 97.7  & 95.9 & 77.6 & 86.4\\
MAmmoTH & 70B & \cmark & MI-260k & 76.9 & 41.8 & 82.4 & - & - & - & - & - \\
ToRA & 7B & \cmark & ToRA-69k & {68.8} & {40.1} & {68.2}  & {73.9} & {88.8} & 42.4  & {54.6}& {62.4} \\
ToRA & 70B & \cmark & ToRA-69k & {{84.3}} & {{49.7}}  & {{82.7}}  & {{86.8}} & {{93.8}}  & {{74.0}} & {{67.2}}& {{76.9}} \\
DeepSeekMath & 7B & \cmark & ToRA-69k & 79.8 & 52.0 & 80.1 & 87.1 & 93.8 & 85.8 & 63.1 & 77.4  \\
\midrule
\multicolumn{12}{c}{\texttt{Our Pretrained Models}} \\
\midrule
TinyLlama-CT & 1B  &\cmark &  ToRA-69k & 51.4 & 38.4 & 53.4 & 66.7 & 81.7 & 20.5 & 42.8 & 50.7\\
\model{}-Math & 1B & \cmark & ToRA-69k & \hl{59.4} & \hl{40.6} & \hl{60.7} & \hl{74.2} & \hl{88.6} & \hl{26.7} & \hl{48.1} & \hl{56.9}
\\
$\Delta$ &  &  &  & \blue{+8.0} & \blue{+2.2} & \blue{+7.3} & \blue{+7.5} & \blue{+6.9} & \blue{+6.2} & \blue{+5.3} & \blue{\textbf{+6.2}} \\ 
\midrule
Mistral-CT & 7B & \cmark & ToRA-69k & 77.5 & 48.4 & 76.9 & 83.8 & 93.4 & 67.5 & 60.4 & 72.6\\
\model{}-Math & 7B & \cmark & ToRA-69k & \hl{81.3} & \hl{51.8} & \hl{80.8} & \hl{85.5} & \hl{94.5} & \hl{70.1} & \hl{63.1} & \hl{75.3} \\
$\Delta$ &  &  &  & \blue{+3.8} & \blue{+3.4} & \blue{+3.9} & \blue{+1.7} & \blue{+1.1} & \blue{+2.6} & \blue{+2.7} & \blue{\textbf{+2.7}} \\
\bottomrule
\end{tabular}
}
\end{table}


==> table/self_ref_results.tex <==
% \begin{table*}[t]
% \centering
% \small
% \setlength{\tabcolsep}{2pt}
% \caption{\textbf{Self-Reference results on Tinyllama-1.1B, all models are trained with OpenWebMath.} 
% We used the Tinyllama-CT as the reference model for SLM.}
% \label{tab:self-ref-1b-owm}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|ccc|cccccc|c}
% \toprule
% \textbf{Model} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} Score \\ Function \end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Uniq.\\ Toks$^*$\end{tabular}}}& \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Train\\ Toks\end{tabular}}} & \textbf{GSM8K} & \textbf{MATH$^\dagger$} & \textbf{SVAMP} & \textbf{ASDiv} & \textbf{MAWPS} & \textbf{MQA} & \textbf{AVG} \\
% \midrule
% Tinyllama-CT (RM) & - & 14B & 15B & 6.3 & 2.6 & 21.7 & 36.7 & 47.7 & 13.9 & 21.5 \\
% % ref loss mask
% Tinyllama-SLM & $\mathcal{L}_{\Delta}$ & 14B & 10.5B & 6.7 & 4.6 & 23.3 & 40.0 & 54.5 & 14.3 & 23.9  \\
% % information entropy
% Tinyllama-SLM & $\mathcal{H}_{\text{RM}}$ & 14B & 10.5B & 7.0 & 4.8 & 23.0 & 39.3 & 50.5 & 13.5 & 23.0 \\
% % add
% Tinyllama-SLM & $\mathcal{L}_{\Delta}\cup\mathcal{H}_{\text{RM}}$ & 14B & 10B & 7.8 & 5.2 & 24.2 & 39.4 & 54.9 & 14.7 & 24.4 \\
% % Tinyllama-SLM & RLM\&IEM & 14B & 10B & 7.8 & 5.2 & 24.2 & 39.4 & 54.9 & 14.7 & 24.4 \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{2pt}
\caption{\textbf{Self-Reference results.} We use OpenWebMath (OWM) to train the reference model.}
\label{tab:self-ref-1b-ppile}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc|cccccc|c}
\toprule
\textbf{Model} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Score \\ Function \end{tabular}}} & \textbf{Data} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Uniq.\\ Toks\end{tabular}}}& \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Train\\ Toks\end{tabular}}} & \textbf{GSM8K} & \textbf{MATH} & \textbf{SVAMP} & \textbf{ASDiv} & \textbf{MAWPS} & \textbf{MQA} & \textbf{AVG} \\
\midrule
Tinyllama-CT (RM) & - & OWM & 14B & 15B & 6.3 & 2.6 & 21.7 & 36.7 & 47.7 & 13.9 & 21.5 \\
Tinyllama-SLM & $\mathcal{L}_{\text{RM}}$ & OWM & 14B & 10.5B & 6.7 & 4.6 & 23.3 & 40.0 & 54.5 & 14.3 & 23.9  \\
Tinyllama-SLM & $\mathcal{H}_{\text{RM}}$ & OWM & 14B & 10.5B & 7.0 & 4.8 & 23.0 & 39.3 & 50.5 & 13.5 & 23.0 \\
% Tinyllama-SLM & $\mathcal{L}_{\Delta}\cup\mathcal{H}_{\text{RM}}$ & OWM & 14B & 10B & 7.8 & 5.2 & 24.2 & 39.4 & 54.9 & 14.7 & 24.4 \\
Tinyllama-SLM & $\mathcal{L}_{\text{RM}}\cap\mathcal{H}_{\text{RM}}$ & OWM & 14B & 9B & \hl{7.1} & \hl{5.0} & \hl{23.5} & \hl{41.2} & \hl{53.8} & \hl{18.0} & \hl{24.8} \\
\midrule
Tinyllama-CT & - & PPile & 55B & 52B & 8.0 & 6.6 & 23.8 & 41.0 & 54.7 & 14.2 & 24.7   \\
Tinyllama-SLM & $\mathcal{L}_{\text{RM}}\cap\mathcal{H}_{\text{RM}}$ & PPile & 55B & 36B & 8.6 & 8.4 & 24.4 & 43.6 & 57.9 & 16.1 & 26.5 \\
\bottomrule
\end{tabular}
}
\end{table*}




==> table/small_ref_results.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{2pt}
\caption{\textbf{Weak-to-Strong generalization result on math benchmark.}
}
\label{tab:small-ref-result}
\resizebox{\linewidth}{!}{
\begin{tabular}{lc|ccccccccc|c}
\toprule
\textbf{Model} & \textbf{Train Toks} & \textbf{GSM8K} & \textbf{MATH} & \textbf{SVAMP} & \textbf{ASDiv} & \textbf{MAWPS} & \textbf{TAB}& \textbf{MQA} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}MMLU\\ STEM\end{tabular}}} & \textbf{SAT} & \textbf{AVG} \\
\midrule
Llama-2-7B-CT & 15B & 28.4 & 13.6 & 50.3 & 62.8 & 79.5 & 37.6 & 34.1 & 41.6 & 43.5 & 43.5 \\
Llama-2-7B-CT w/ 1B RM & 10.5B &  29.8 & 16.0 & 55.5 & 63.7 & 80.4 & 37.9 & 34.3 & 38.2 & 43.8 & 44.4 \\
\bottomrule
\end{tabular}
}
\end{table*}


==> table/token_fluctuating_example.tex <==
\begin{table*}[htbp]
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}p{16cm}@{}}
\toprule
\multicolumn{1}{c}{\textbf{\textit{Examples of Tokens that Exhibit Abnormal Behavior during Training}}} \\
\midrule
\textcolor{black}{ as} \textcolor{black}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{\textbackslash }\textcolor{black}{begin}\textcolor{black}{\{}\textcolor{black}{aligned}\textcolor{black}{\}}\textcolor{black}{A} \textcolor{black}{ \textbackslash }\textcolor{black}{in} \textcolor{black}{ \textbackslash }\textcolor{black}{\{\textbackslash }\textcolor{black}{pm} \textcolor{black}{ \textbackslash }\textcolor{black}{begin}\textcolor{black}{\{}\textcolor{black}{bmatrix}\textcolor{black}{\}\textbackslash }\textcolor{black}{cos}\textcolor{black}{\textbackslash }\textcolor{black}{theta} \textcolor{black}{ \&} \textcolor{black}{ -} \textcolor{black}{ \textbackslash }\textcolor[RGB]{255,140,0}{sin}\textcolor{black}{\textbackslash }\textcolor{black}{theta} \textcolor{black}{ \textbackslash \textbackslash } \textcolor{black}{ \textbackslash }\textcolor[RGB]{255,140,0}{sin}\textcolor{black}{\textbackslash }\textcolor[RGB]{255,140,0}{theta} \textcolor{black}{ \&} \textcolor[RGB]{255,140,0}{ \textbackslash }\textcolor[RGB]{255,140,0}{cos}\textcolor[RGB]{255,140,0}{\textbackslash }\textcolor{black}{theta} \textcolor{black}{ \textbackslash \textbackslash } \textcolor{black}{ \textbackslash }\textcolor[RGB]{255,140,0}{end}\textcolor{black}{\{}\textcolor{black}{bmatrix}\textcolor{black}{\},} \textcolor{black}{ \textbackslash }\textcolor{black}{pm} \textcolor{black}{ \textbackslash }\textcolor{black}{begin}\textcolor{black}{\{}\textcolor{black}{bmatrix}\textcolor{black}{\}\textbackslash }\textcolor{black}{cos}\textcolor{black}{\textbackslash }\textcolor{black}{theta} \textcolor{black}{ \&} \textcolor{black}{ \textbackslash }\textcolor[RGB]{255,140,0}{sin}\textcolor{black}{\textbackslash }\textcolor{black}{theta} \textcolor{black}{ \textbackslash \textbackslash } \textcolor{black}{ \textbackslash }\textcolor[RGB]{255,140,0}{sin}\textcolor{black}{\textbackslash }\textcolor{black}{theta} \textcolor{black}{ \&} \textcolor{black}{ -} \textcolor[RGB]{255,140,0}{ \textbackslash }\textcolor{black}{cos}\textcolor{black}{\textbackslash }\textcolor{black}{theta} \textcolor{black}{ \textbackslash \textbackslash } \textcolor{black}{ \textbackslash }\textcolor[RGB]{255,140,0}{end}\textcolor{black}{\{}\textcolor{black}{bmatrix}\textcolor{black}{\},} \textcolor{black}{ \textbackslash }\textcolor{black}{pm} \textcolor{black}{ \textbackslash }\textcolor{black}{begin}\textcolor{black}{\{}\textcolor{black}{bmatrix}\textcolor{black}{\}}\textcolor{black}{i} \textcolor{black}{ \textbackslash }\textcolor{black}{sin}\textcolor{black}{h}\textcolor{black}{\textbackslash }\textcolor[RGB]{255,140,0}{theta} \textcolor{black}{ \&} \textcolor{black}{ -\textbackslash }\textcolor{black}{cos}\textcolor{black}{h}\textcolor[RGB]{255,140,0}{\textbackslash }\textcolor{black}{theta} \textcolor{black}{ \textbackslash \textbackslash } \textcolor[RGB]{255,140,0}{ \textbackslash }\textcolor[RGB]{255,140,0}{cos}\textcolor[RGB]{255,140,0}{h}\textcolor{black}{\textbackslash }\textcolor{black}{theta} \textcolor[RGB]{255,140,0}{ \&} \textcolor[RGB]{255,140,0}{ i} \textcolor{black}{ \textbackslash }\textcolor[RGB]{255,140,0}{sin}\textcolor[RGB]{255,140,0}{h}\textcolor[RGB]{255,140,0}{\textbackslash }\textcolor{black}{theta} \textcolor[RGB]{255,140,0}{ \textbackslash \textbackslash } \textcolor[RGB]{255,140,0}{ \textbackslash }\textcolor[RGB]{255,140,0}{end}\textcolor{black}{\{}\textcolor{black}{bmatrix}\textcolor[RGB]{255,140,0}{\},} \textcolor{black}{ \textbackslash }\textcolor{black}{pm} \textcolor{black}{ \textbackslash }\textcolor{black}{begin}\textcolor{black}{\{}\textcolor{black}{bmatrix}\textcolor{black}{\}}\textcolor{black}{i} \textcolor{black}{ \textbackslash }\textcolor{black}{sin}\textcolor{black}{h}\textcolor{black}{\textbackslash }\textcolor[RGB]{255,140,0}{theta} \textcolor{black}{ \&} \textcolor{black}{ \textbackslash }\textcolor[RGB]{255,140,0}{cos}\textcolor[RGB]{255,140,0}{h}\textcolor{black}{\textbackslash }\textcolor{black}{theta} \textcolor{black}{ \textbackslash \textbackslash } \textcolor{black}{ \textbackslash }\textcolor[RGB]{255,140,0}{cos}\textcolor[RGB]{255,140,0}{h}\textcolor{black}{\textbackslash }\textcolor{black}{theta} \textcolor[RGB]{255,140,0}{ \&} \textcolor{black}{ -} \textcolor{black}{ i} \textcolor{black}{ \textbackslash }\textcolor{black}{sin}\textcolor{black}{h}\textcolor{black}{\textbackslash }\textcolor{black}{theta} \textcolor[RGB]{255,140,0}{ \textbackslash \textbackslash } \textcolor[RGB]{255,140,0}{ \textbackslash }\textcolor[RGB]{255,140,0}{end}\textcolor{black}{\{}\textcolor[RGB]{255,140,0}{bmatrix}\textcolor{black}{\}\textbackslash }\textcolor{black}{\}\textbackslash }\textcolor{black}{end}\textcolor{black}{\{}\textcolor[RGB]{255,140,0}{aligned}\textcolor{black}{\}} \textcolor{black}{ \textbackslash }\textcolor{black}{quad}\textcolor{black}{\textbackslash }\textcolor{black}{quad}\textcolor{black}{\textbackslash }\textcolor[RGB]{255,140,0}{quad}\textcolor{black}{(}\textcolor{black}{2}\textcolor{black}{5}\textcolor{black}{)} \textcolor{black}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{I} \textcolor{black}{ suspect} \textcolor{black}{ this} \textcolor{black}{ class} \textcolor{black}{ of} \textcolor{black}{ transformations} \textcolor{black}{ has} \textcolor{black}{ a} \textcolor{black}{ name} \textcolor{black}{ in} \textcolor{black}{ the} \textcolor{black}{ grand} \textcolor{black}{ group} \textcolor{black}{ classification} \textcolor{black}{ scheme}\textcolor{black}{,} \textcolor{black}{ but} \textcolor{black}{ I} \textcolor{black}{ don}\textcolor{black}{’}\textcolor{black}{t} \textcolor{black}{ know} \textcolor{black}{ what} \textcolor{black}{ it} \textcolor[RGB]{255,140,0}{ is}\textcolor{black}{.} \textcolor{black}{ \#\#\#} \textcolor{black}{ Mathemat}\textcolor{black}{ics} \textcolor{black}{ Class} \textcolor{black}{ XI} \textcolor{black}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{Unit}\textcolor{black}{-}\textcolor{black}{I}\textcolor{black}{:} \textcolor{black}{ S}\textcolor{black}{ets} \textcolor{black}{ and} \textcolor{black}{ Function}\textcolor{black}{s} \textcolor{black}{ \textbackslash n }\textcolor{black}{Ch}\textcolor{black}{apter} \textcolor{black}{ }\textcolor{black}{1}\textcolor{black}{:} \textcolor{black}{ S}\textcolor{black}{ets} \textcolor{black}{ \textbackslash n }\textcolor{black}{Unit}\textcolor[RGB]{255,140,0}{-}\textcolor{black}{II}\textcolor{black}{:} \textcolor{black}{ Al}\textcolor[RGB]{255,140,0}{gebra} \textcolor{black}{ \textbackslash n }\textcolor[RGB]{255,140,0}{Ch}\textcolor{black}{apter} \textcolor{black}{ }\textcolor{black}{5}\textcolor{black}{:} \textcolor{black}{ Bin}\textcolor[RGB]{255,140,0}{omial} \textcolor{black}{ Theorem} \textcolor{black}{ \textbackslash n }\textcolor{black}{Ch}\textcolor[RGB]{255,140,0}{apter} \textcolor[RGB]{255,140,0}{ }\textcolor{black}{6}\textcolor{black}{:} \textcolor{black}{ Se}\textcolor{black}{quence} \textcolor{black}{ and} \textcolor{black}{ Series} \textcolor{black}{ \textbackslash n }\textcolor{black}{Unit}\textcolor{black}{-}\textcolor[RGB]{255,140,0}{III}\textcolor{black}{:} \textcolor{black}{ Co}\textcolor[RGB]{255,140,0}{ordinate} \textcolor{black}{ Ge}\textcolor[RGB]{255,140,0}{ometry} \textcolor[RGB]{255,140,0}{ \textbackslash n }\textcolor[RGB]{255,140,0}{Ch}\textcolor[RGB]{255,140,0}{apter} \textcolor{black}{ }\textcolor{black}{1}\textcolor{black}{:} \textcolor{black}{ Stra}\textcolor{black}{ight} \textcolor{black}{ L}\textcolor{black}{ines} \textcolor[RGB]{255,140,0}{ \textbackslash n }\textcolor[RGB]{255,140,0}{Ch}\textcolor{black}{apter} \textcolor{black}{ }\textcolor{black}{2}\textcolor{black}{:} \textcolor{black}{ Con}\textcolor[RGB]{255,140,0}{ic} \textcolor{black}{ Se}\textcolor[RGB]{255,140,0}{ctions} \textcolor{black}{ \textbackslash n }\textcolor{black}{Unit}\textcolor{black}{-}\textcolor[RGB]{255,140,0}{IV}\textcolor{black}{:} \textcolor{black}{ Calcul}\textcolor[RGB]{255,140,0}{us} \textcolor{black}{ \textbackslash n }\textcolor{black}{Unit}\textcolor[RGB]{255,140,0}{-}\textcolor{black}{V}\textcolor[RGB]{255,140,0}{:} \textcolor{black}{ Mathemat}\textcolor{black}{ical} \textcolor{black}{ Re}\textcolor[RGB]{255,140,0}{ason}\textcolor{black}{ing} \textcolor{black}{ \textbackslash n }\textcolor{black}{Unit}\textcolor[RGB]{255,140,0}{-}\textcolor[RGB]{255,140,0}{VI}\textcolor{black}{:} \textcolor{black}{ Statistics} \textcolor{black}{ and} \textcolor[RGB]{255,140,0}{ Pro}\textcolor{black}{b}\textcolor{black}{ability} \textcolor[RGB]{255,140,0}{ \textbackslash n }\textcolor{black}{Ch}\textcolor[RGB]{255,140,0}{apter} \textcolor{black}{ }\textcolor{black}{1}\textcolor{black}{:} \textcolor{black}{ Statistics} \textcolor{black}{ \textbackslash n }\textcolor[RGB]{255,140,0}{Ch}\textcolor[RGB]{255,140,0}{apter} \textcolor{black}{ }\textcolor{black}{2}\textcolor{black}{:} \textcolor{black}{ Pro}\textcolor{black}{b}\textcolor[RGB]{255,140,0}{ability} \textcolor[RGB]{255,140,0}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{\#} \textcolor{black}{ Graph}\textcolor{black}{s} \textcolor{black}{ of} \textcolor{black}{ Tr}\textcolor[RGB]{255,140,0}{ig}\textcolor[RGB]{255,140,0}{on}\textcolor[RGB]{255,140,0}{ometric} \textcolor{black}{ Function}\textcolor{black}{s} \textcolor{black}{ \textbackslash n } \textcolor[RGB]{255,140,0}{ \textbackslash n }\textcolor{black}{(}\textcolor{black}{i}\textcolor{black}{)} \\
\hline
\textcolor{black}{ Ge}\textcolor[RGB]{255,140,0}{ometry} \textcolor[RGB]{255,140,0}{ in} \textcolor{black}{ any} \textcolor[RGB]{255,140,0}{ field}\textcolor[RGB]{255,140,0}{.} \textcolor{black}{ Qu}\textcolor{black}{eries} \textcolor{black}{ are} \textcolor[RGB]{255,140,0}{ case}\textcolor[RGB]{255,140,0}{-}\textcolor{black}{in}\textcolor{black}{dependent}\textcolor[RGB]{255,140,0}{.} \textcolor{black}{ Fun}\textcolor{black}{ct}\textcolor{black}{*} \textcolor{black}{ Wild}\textcolor[RGB]{255,140,0}{card} \textcolor{black}{ queries} \textcolor[RGB]{255,140,0}{ are} \textcolor{black}{ specified} \textcolor[RGB]{255,140,0}{ by} \textcolor{black}{ *} \textcolor[RGB]{255,140,0}{ (}\textcolor[RGB]{255,140,0}{e}\textcolor{black}{.}\textcolor[RGB]{255,140,0}{g}\textcolor{black}{.} \textcolor{black}{ functions}\textcolor[RGB]{255,140,0}{,} \textcolor{black}{ fun}\textcolor{black}{ctor}\textcolor{black}{ial}\textcolor{black}{,} \textcolor[RGB]{255,140,0}{ etc}\textcolor[RGB]{255,140,0}{.).} \textcolor{black}{ Otherwise} \textcolor{black}{ the} \textcolor{black}{ search} \textcolor[RGB]{255,140,0}{ is} \textcolor{black}{ exact}\textcolor[RGB]{255,140,0}{.} \textcolor{black}{ ''}\textcolor{black}{Top}\textcolor{black}{ological} \textcolor{black}{ group}\textcolor[RGB]{255,140,0}{''} \textcolor{black}{ P}\textcolor{black}{hr}\textcolor[RGB]{255,140,0}{ases} \textcolor{black}{ (}\textcolor{black}{multi}\textcolor[RGB]{255,140,0}{-}\textcolor{black}{words}\textcolor[RGB]{255,140,0}{)} \textcolor{black}{ should} \textcolor{black}{ be} \textcolor{black}{ set} \textcolor{black}{ in} \textcolor{black}{ ''}\textcolor{black}{stra}\textcolor{black}{ight} \textcolor{black}{ quot}\textcolor[RGB]{255,140,0}{ation} \textcolor[RGB]{255,140,0}{ marks}\textcolor[RGB]{255,140,0}{''.} \textcolor{black}{ au}\textcolor[RGB]{255,140,0}{:} \textcolor{black}{ Bour}\textcolor[RGB]{255,140,0}{b} \textcolor[RGB]{255,140,0}{aki} \textcolor{black}{ \&} \textcolor{black}{ ti}\textcolor[RGB]{255,140,0}{:} \textcolor{black}{ Al}\textcolor[RGB]{255,140,0}{gebra} \textcolor{black}{ Search} \textcolor{black}{ for} \textcolor{black}{ author} \textcolor{black}{ and} \textcolor{black}{ title}\textcolor{black}{.} \textcolor{black}{ The} \textcolor{black}{ and}\textcolor{black}{-}\textcolor[RGB]{255,140,0}{operator} \textcolor{black}{ \&} \textcolor[RGB]{255,140,0}{ is} \textcolor{black}{ default} \textcolor[RGB]{255,140,0}{ and} \textcolor{black}{ can} \textcolor{black}{ be} \textcolor{black}{ omitted}\textcolor[RGB]{255,140,0}{.} \textcolor{black}{ Che}\textcolor[RGB]{255,140,0}{b} \textcolor{black}{ys}\textcolor[RGB]{255,140,0}{he}\textcolor{black}{v} \textcolor{black}{ |} \textcolor{black}{ Tsch}\textcolor[RGB]{255,140,0}{eb}\textcolor[RGB]{255,140,0}{y}\textcolor[RGB]{255,140,0}{sche}\textcolor{black}{ff} \textcolor{black}{ The} \textcolor{black}{ or}\textcolor[RGB]{255,140,0}{-}\textcolor{black}{operator} \textcolor[RGB]{255,140,0}{ |} \textcolor{black}{ allows} \textcolor{black}{ to} \textcolor[RGB]{255,140,0}{ search} \textcolor[RGB]{255,140,0}{ for} \textcolor{black}{ Che}\textcolor{black}{b} \textcolor{black}{ys}\textcolor{black}{he}\textcolor{black}{v} \textcolor[RGB]{255,140,0}{ or} \textcolor[RGB]{255,140,0}{ Tsch}\textcolor{black}{eb}\textcolor{black}{y}\textcolor{black}{sche}\textcolor{black}{ff}\textcolor{black}{.} \textcolor{black}{ ''}\textcolor{black}{Qu}\textcolor{black}{asi}\textcolor{black}{*} \textcolor{black}{ map}\textcolor{black}{*''} \textcolor{black}{ py}\textcolor[RGB]{255,140,0}{:} \textcolor{black}{ }\textcolor[RGB]{255,140,0}{1}\textcolor[RGB]{255,140,0}{9}\textcolor{black}{8}\textcolor{black}{9} \textcolor{black}{ The} \textcolor{black}{ resulting} \textcolor{black}{ documents} \textcolor[RGB]{255,140,0}{ have} \textcolor{black}{ publication} \textcolor[RGB]{255,140,0}{ year} \textcolor[RGB]{255,140,0}{ }\textcolor{black}{1}\textcolor{black}{9}\textcolor{black}{8}\textcolor{black}{9}\textcolor[RGB]{255,140,0}{.} \textcolor{black}{ so}\textcolor[RGB]{255,140,0}{:} \textcolor{black}{ Eur}\textcolor{black}{*} \textcolor[RGB]{255,140,0}{ J}\textcolor[RGB]{255,140,0}{*} \textcolor{black}{ Mat}\textcolor[RGB]{255,140,0}{*} \textcolor{black}{ Soc}\textcolor[RGB]{255,140,0}{*} \textcolor{black}{ cc}\textcolor{black}{:} \textcolor[RGB]{255,140,0}{ }\textcolor[RGB]{255,140,0}{1}\textcolor{black}{4} \textcolor{black}{ Search} \textcolor{black}{ for} \textcolor{black}{ publications} \textcolor{black}{ in} \textcolor[RGB]{255,140,0}{ a} \textcolor{black}{ particular} \textcolor{black}{ source} \textcolor{black}{ with} \textcolor[RGB]{255,140,0}{ a} \textcolor{black}{ Mathemat}\textcolor[RGB]{255,140,0}{ics} \textcolor{black}{ Sub}\textcolor{black}{ject} \textcolor{black}{ Classification} \textcolor[RGB]{255,140,0}{ code} \textcolor[RGB]{255,140,0}{ (}\textcolor{black}{cc}\textcolor[RGB]{255,140,0}{)} \textcolor{black}{ in} \textcolor{black}{ }\textcolor[RGB]{255,140,0}{1}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{.} \textcolor{black}{ ''}\textcolor{black}{Part}\textcolor[RGB]{255,140,0}{ial} \textcolor{black}{ diff}\textcolor[RGB]{255,140,0}{*} \textcolor[RGB]{255,140,0}{ eq}\textcolor{black}{*''} \textcolor{black}{ !} \textcolor{black}{ elli}\textcolor[RGB]{255,140,0}{ptic} \textcolor{black}{ The} \textcolor{black}{ not}\textcolor{black}{-}\textcolor{black}{operator} \textcolor[RGB]{255,140,0}{ !} \textcolor{black}{ elimin}\textcolor{black}{ates} \textcolor[RGB]{255,140,0}{ all} \textcolor{black}{ results} \textcolor{black}{ containing} \textcolor{black}{ the} \textcolor{black}{ word} \textcolor{black}{ elli}\textcolor{black}{ptic}\textcolor{black}{.} \textcolor{black}{ dt}\textcolor[RGB]{255,140,0}{:} \textcolor{black}{ b} \textcolor{black}{ \&} \textcolor{black}{ au}\textcolor{black}{:} \textcolor{black}{ Hil}\textcolor[RGB]{255,140,0}{bert} \textcolor{black}{ The} \textcolor{black}{ document} \textcolor[RGB]{255,140,0}{ type} \textcolor{black}{ is} \textcolor{black}{ set} \textcolor[RGB]{255,140,0}{ to} \textcolor{black}{ books}\textcolor{black}{;} \textcolor{black}{ altern}\textcolor{black}{atively}\textcolor{black}{:} \textcolor{black}{ j} \textcolor{black}{ for} \textcolor[RGB]{255,140,0}{ journal} \textcolor{black}{ articles}\textcolor[RGB]{255,140,0}{,} \textcolor{black}{ a} \textcolor{black}{ for} \textcolor{black}{ book} \textcolor[RGB]{255,140,0}{ articles}\textcolor[RGB]{255,140,0}{.} \textcolor{black}{ py}\textcolor{black}{:} \textcolor[RGB]{255,140,0}{ }\textcolor{black}{2}\textcolor[RGB]{255,140,0}{0}\textcolor[RGB]{255,140,0}{0}\textcolor[RGB]{255,140,0}{0}\textcolor[RGB]{255,140,0}{-}\textcolor{black}{2}\textcolor{black}{0}\textcolor[RGB]{255,140,0}{1}\textcolor{black}{5} \textcolor{black}{ cc}\textcolor{black}{:} \textcolor[RGB]{255,140,0}{ (}\textcolor{black}{9}\textcolor{black}{4}\textcolor{black}{A} \textcolor{black}{ |} \textcolor[RGB]{255,140,0}{ }\textcolor{black}{1}\textcolor{black}{1}\textcolor{black}{T}\textcolor{black}{)} \textcolor{black}{ Number} \textcolor{black}{ ranges} \textcolor[RGB]{255,140,0}{ are} \textcolor{black}{ accepted}\textcolor[RGB]{255,140,0}{.} \textcolor{black}{ Term}\textcolor[RGB]{255,140,0}{s} \textcolor{black}{ can} \textcolor[RGB]{255,140,0}{ be} \textcolor{black}{ grouped} \textcolor{black}{ within} \textcolor{black}{ (}\textcolor{black}{parent}\textcolor[RGB]{255,140,0}{hes}\textcolor{black}{es}\textcolor[RGB]{255,140,0}{).} \textcolor{black}{ la}\textcolor[RGB]{255,140,0}{:} \textcolor{black}{ ch}\textcolor{black}{inese} \textcolor{black}{ Find} \textcolor{black}{ documents} \textcolor[RGB]{255,140,0}{ in} \textcolor{black}{ a} \textcolor{black}{ given} \textcolor[RGB]{255,140,0}{ language}\textcolor[RGB]{255,140,0}{.} \textcolor{black}{ ISO} \textcolor[RGB]{255,140,0}{ }\textcolor{black}{6}\textcolor{black}{3}\textcolor[RGB]{255,140,0}{9}\textcolor[RGB]{255,140,0}{-}\textcolor[RGB]{255,140,0}{1} \textcolor{black}{ language} \textcolor[RGB]{255,140,0}{ codes} \textcolor{black}{ can} \textcolor{black}{ also} \textcolor{black}{ be} \textcolor[RGB]{255,140,0}{ used}\textcolor[RGB]{255,140,0}{.}  
\\ \hline
\textcolor{black}{Code}\textcolor{black}{:} \textcolor{black}{ Select} \textcolor[RGB]{255,140,0}{ all} \textcolor{black}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{x} \textcolor{black}{ =} \textcolor[RGB]{255,140,0}{ }\textcolor{black}{6}\textcolor{black}{4}\textcolor{black}{,} \textcolor{black}{ y} \textcolor[RGB]{255,140,0}{ =} \textcolor[RGB]{255,140,0}{ }\textcolor{black}{8}\textcolor{black}{6}\textcolor{black}{,} \textcolor{black}{ rule} \textcolor[RGB]{255,140,0}{ =} \textcolor{black}{ B}\textcolor{black}{3}\textcolor{black}{/}\textcolor{black}{S}\textcolor{black}{2}\textcolor{black}{3} \textcolor{black}{ \textbackslash n }\textcolor{black}{1}\textcolor{black}{3}\textcolor{black}{bo}\textcolor{black}{\$}\textcolor{black}{3}\textcolor{black}{b}\textcolor{black}{ob}\textcolor{black}{o}\textcolor{black}{6}\textcolor{black}{bo}\textcolor{black}{\$}\textcolor{black}{4}\textcolor{black}{b}\textcolor{black}{2}\textcolor{black}{o}\textcolor{black}{6}\textcolor{black}{b}\textcolor{black}{3}\textcolor{black}{o}\textcolor{black}{\$}\textcolor{black}{4}\textcolor{black}{bo}\textcolor{black}{\$}\textcolor{black}{5}\textcolor{black}{4}\textcolor{black}{bo}\textcolor{black}{\$}\textcolor{black}{5}\textcolor{black}{4}\textcolor{black}{b}\textcolor{black}{ob}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{\$}\textcolor{black}{1}\textcolor{black}{3}\textcolor{black}{b}\textcolor{black}{2}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{3}\textcolor{black}{9}\textcolor{black}{b} \textcolor{black}{2}\textcolor[RGB]{255,140,0}{o} \textcolor{black}{\$}\textcolor{black}{1}\textcolor{black}{2}\textcolor{black}{b}\textcolor{black}{2}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{4}\textcolor{black}{4}\textcolor{black}{b}\textcolor{black}{2}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{\$}\textcolor{black}{3}\textcolor{black}{o}\textcolor{black}{1}\textcolor{black}{1}\textcolor{black}{bo}\textcolor{black}{4}\textcolor{black}{3}\textcolor{black}{b} \textcolor{black}{ \textbackslash n }\textcolor{black}{o}\textcolor{black}{3}\textcolor{black}{b}\textcolor{black}{2}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{\$}\textcolor{black}{2}\textcolor{black}{bo}\textcolor{black}{4}\textcolor{black}{9}\textcolor{black}{bo} \textcolor{black}{6}\textcolor{black}{bo}\textcolor{black}{2}\textcolor{black}{bo}\textcolor{black}{\$}\textcolor{black}{bo}\textcolor{black}{5}\textcolor{black}{0}\textcolor{black}{b} \textcolor{black}{2}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{6}\textcolor{black}{b} \textcolor{black}{ob}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{\$}\textcolor{black}{5}\textcolor{black}{1}\textcolor{black}{b}\textcolor{black}{ob} \textcolor[RGB]{255,140,0}{o}\textcolor{black}{7}\textcolor{black}{bo}\textcolor{black}{\$}\textcolor{black}{7}\textcolor{black}{bo}\textcolor{black}{4}\textcolor{black}{9}\textcolor{black}{bo}\textcolor{black}{\$}\textcolor{black}{7} \textcolor{black}{b}\textcolor{black}{3}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{4}\textcolor{black}{7}\textcolor{black}{b}\textcolor{black}{3}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{\$}\textcolor{black}{1}\textcolor{black}{0}\textcolor{black}{bo}\textcolor{black}{5}\textcolor{black}{b}\textcolor{black}{2}\textcolor[RGB]{255,140,0}{o} \textcolor{black}{ \textbackslash n }\textcolor{black}{4}\textcolor{black}{2}\textcolor{black}{bo}\textcolor{black}{\$}\textcolor{black}{9}\textcolor{black}{b}\textcolor{black}{2}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{4}\textcolor{black}{b}\textcolor{black}{2}\textcolor[RGB]{255,140,0}{o} \textcolor{black}{4}\textcolor{black}{2}\textcolor{black}{b} \textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{\$}\textcolor{black}{1}\textcolor{black}{7}\textcolor{black}{bo}\textcolor{black}{7}\textcolor{black}{\$}\textcolor{black}{1}\textcolor{black}{3}\textcolor{black}{bo}\textcolor{black}{\$}\textcolor{black}{3}\textcolor{black}{b} \textcolor[RGB]{255,140,0}{ob}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{6}\textcolor[RGB]{255,140,0}{bo}\textcolor{black}{\$}\textcolor{black}{4}\textcolor[RGB]{255,140,0}{b} \textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{6}\textcolor[RGB]{255,140,0}{b} \textcolor[RGB]{255,140,0}{3}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{\$}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{\$}\textcolor{black}{5}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{\$}\textcolor[RGB]{255,140,0}{5}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{b} \textcolor[RGB]{255,140,0}{ob}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{\$}\textcolor[RGB]{255,140,0}{1}\textcolor[RGB]{255,140,0}{3}\textcolor[RGB]{255,140,0}{b} \textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o} \textcolor{black}{ }\textcolor{black}{3}\textcolor{black}{9}\textcolor[RGB]{255,140,0}{b}\textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{\$}\textcolor[RGB]{255,140,0}{1}\textcolor{black}{2}\textcolor[RGB]{255,140,0}{b}\textcolor{black}{2}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{4}\textcolor{black}{4}\textcolor[RGB]{255,140,0}{b}\textcolor{black}{2}\textcolor{black}{o}\textcolor{black}{\$}\textcolor{black}{3}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{1}\textcolor{black}{1}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{4}\textcolor{black}{3}\textcolor{black}{bo}\textcolor{black}{3}\textcolor{black}{b}\textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{\$}\textcolor{black}{2}\textcolor[RGB]{255,140,0}{bo}\textcolor{black}{4}\textcolor[RGB]{255,140,0}{9}\textcolor[RGB]{255,140,0}{bo}\textcolor{black}{6}\textcolor[RGB]{255,140,0}{bo}\textcolor{black}{2}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{\$}\textcolor[RGB]{255,140,0}{bo}\textcolor{black}{5}\textcolor{black}{0}\textcolor[RGB]{255,140,0}{b} \textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{6}\textcolor[RGB]{255,140,0}{b} \textcolor[RGB]{255,140,0}{ob}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{\$}\textcolor[RGB]{255,140,0}{5}\textcolor{black}{1}\textcolor[RGB]{255,140,0}{b}\textcolor[RGB]{255,140,0}{ob}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{7}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{\$}\textcolor{black}{7}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{9}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{\$}\textcolor[RGB]{255,140,0}{7}\textcolor[RGB]{255,140,0}{b}\textcolor[RGB]{255,140,0}{3}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{7}\textcolor[RGB]{255,140,0}{b}\textcolor[RGB]{255,140,0}{3}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{\$}\textcolor[RGB]{255,140,0}{1}\textcolor{black}{0}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{5}\textcolor[RGB]{255,140,0}{b}\textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{4}\textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{\$}\textcolor[RGB]{255,140,0}{9}\textcolor{black}{bo}\textcolor{black}{5}\textcolor{black}{b}\textcolor{black}{2}\textcolor{black}{o}\textcolor{black}{4}\textcolor[RGB]{255,140,0}{2}\textcolor{black}{bo}\textcolor{black}{\$}\textcolor{black}{9}\textcolor{black}{b}\textcolor{black}{2}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{6}\textcolor{black}{bo}\textcolor{black}{4}\textcolor{black}{1}\textcolor{black}{b}\textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{7}\textcolor{black}{\$}\textcolor{black}{1}\textcolor{black}{3}\textcolor[RGB]{255,140,0}{bo}\textcolor{black}{\$}\textcolor{black}{3}\textcolor{black}{b}\textcolor[RGB]{255,140,0}{ob}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{6}\textcolor[RGB]{255,140,0}{bo}\textcolor{black}{\$}\textcolor[RGB]{255,140,0}{4}\textcolor{black}{b} \textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{6}\textcolor{black}{b}\textcolor[RGB]{255,140,0}{3}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{\$}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{\$}\textcolor{black}{5}\textcolor{black}{4}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{\$}\textcolor{black}{5}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{b}\textcolor[RGB]{255,140,0}{ob}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{\$}\textcolor[RGB]{255,140,0}{1}\textcolor{black}{3}\textcolor[RGB]{255,140,0}{b}\textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{3}\textcolor[RGB]{255,140,0}{9}\textcolor{black}{b}\textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{\$}\textcolor[RGB]{255,140,0}{1}\textcolor{black}{2}\textcolor[RGB]{255,140,0}{b}\textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{b}\textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{\$}\textcolor[RGB]{255,140,0}{3}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{1}\textcolor{black}{1}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{3}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{3}\textcolor[RGB]{255,140,0}{b}\textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{\$}\textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{9}\textcolor[RGB]{255,140,0}{bo} \textcolor{black}{ }\textcolor[RGB]{255,140,0}{6}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{\$}\textcolor[RGB]{255,140,0}{bo}\textcolor{black}{5}\textcolor{black}{0}\textcolor{black}{b}\textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{6}\textcolor[RGB]{255,140,0}{b}\textcolor[RGB]{255,140,0}{ob}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{\$}\textcolor{black}{5}\textcolor[RGB]{255,140,0}{1}\textcolor{black}{b}\textcolor[RGB]{255,140,0}{ob}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{7}\textcolor[RGB]{255,140,0}{bo}\textcolor{black}{\$}\textcolor{black}{7}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{9}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{\$}\textcolor{black}{7}\textcolor[RGB]{255,140,0}{b}\textcolor[RGB]{255,140,0}{3}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{7}\textcolor[RGB]{255,140,0}{b}\textcolor[RGB]{255,140,0}{3}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{\$}\textcolor{black}{1}\textcolor{black}{0}\textcolor[RGB]{255,140,0}{bo}\textcolor{black}{5}\textcolor{black}{b}\textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{bo}\textcolor{black}{\$}\textcolor{black}{7}\textcolor{black}{b}\textcolor{black}{3}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{5}\textcolor{black}{b}\textcolor{black}{2}\textcolor{black}{o} \textcolor{black}{ }\textcolor{black}{4}\textcolor{black}{0}\textcolor{black}{b}\textcolor{black}{3}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{\$}\textcolor{black}{7}\textcolor{black}{bo}\textcolor{black}{9}\textcolor{black}{bo}\textcolor{black}{3}\textcolor{black}{9}\textcolor{black}{bo}\textcolor{black}{7}\textcolor{black}{\$}\textcolor{black}{1}\textcolor{black}{3}\textcolor[RGB]{255,140,0}{bo}\textcolor{black}{\$}\textcolor[RGB]{255,140,0}{3}\textcolor[RGB]{255,140,0}{b} 
 \textcolor[RGB]{255,140,0}{ob}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{6}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{\$}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{b} \textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{6}\textcolor[RGB]{255,140,0}{b} \textcolor[RGB]{255,140,0}{3}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{\$}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{bo}\textcolor{black}{\$}\textcolor{black}{5}\textcolor{black}{4}\textcolor[RGB]{255,140,0}{bo}\textcolor{black}{\$}\textcolor{black}{5}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{b} \textcolor[RGB]{255,140,0}{ob}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{\$}\textcolor[RGB]{255,140,0}{1}\textcolor[RGB]{255,140,0}{3}\textcolor[RGB]{255,140,0}{b} 
 \textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{3}\textcolor[RGB]{255,140,0}{9}\textcolor[RGB]{255,140,0}{b} \textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{\$} \textcolor{black}{ \textbackslash n }\textcolor{black}{1}\textcolor{black}{2}\textcolor{black}{b} \textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{b} \textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{\$}\textcolor{black}{3}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{1}\textcolor{black}{1}\textcolor{black}{bo}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{3}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{3}\textcolor{black}{b} \textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{\$}\textcolor{black}{2}\textcolor{black}{bo}\textcolor{black}{4}\textcolor[RGB]{255,140,0}{9}\textcolor{black}{bo}\textcolor[RGB]{255,140,0}{6}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{bo}\textcolor{black}{\$}\textcolor[RGB]{255,140,0}{bo}\textcolor{black}{5}\textcolor{black}{0}\textcolor{black}{b} \textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{6}\textcolor{black}{b} \textcolor{black}{ob}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{\$}\textcolor{black}{5}\textcolor[RGB]{255,140,0}{1}\textcolor{black}{b} \textcolor[RGB]{255,140,0}{ob}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{7}\textcolor[RGB]{255,140,0}{bo}\textcolor{black}{\$}\textcolor{black}{7}\textcolor{black}{bo}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{9}\textcolor[RGB]{255,140,0}{bo}\textcolor{black}{\$}\textcolor{black}{7}\textcolor[RGB]{255,140,0}{b} \textcolor[RGB]{255,140,0}{3}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{7}\textcolor[RGB]{255,140,0}{b} 
 \textcolor[RGB]{255,140,0}{3}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{\$}\textcolor[RGB]{255,140,0}{1}\textcolor[RGB]{255,140,0}{0}\textcolor{black}{bo}\textcolor[RGB]{255,140,0}{5}\textcolor[RGB]{255,140,0}{b} \textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{o}\textcolor[RGB]{255,140,0}{4}\textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{bo}\textcolor[RGB]{255,140,0}{\$}\textcolor{black}{7}\textcolor{black}{b} \textcolor{black}{2}\textcolor{black}{ob}\textcolor{black}{o}\textcolor{black}{4}\textcolor{black}{b} \textcolor{black}{2}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{4}\textcolor{black}{0}\textcolor{black}{b} 
 \textcolor{black}{2}\textcolor{black}{ob}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{\$}\textcolor{black}{7}\textcolor{black}{b} 
 \textcolor{black}{ob}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{7}\textcolor{black}{bo}\textcolor{black}{3}\textcolor{black}{9}\textcolor{black}{b} \textcolor{black}{ob}\textcolor[RGB]{255,140,0}{o}\textcolor{black}{!} \textcolor{black}{ The} \textcolor{black}{ }\textcolor{black}{1}\textcolor{black}{6}\textcolor{black}{-}\textcolor{black}{bit}\textcolor{black}{ter} \textcolor{black}{ thus} \textcolor{black}{ goes} \textcolor{black}{ down} \textcolor{black}{ to} \textcolor{black}{ }\textcolor{black}{9} \textcolor{black}{ gl}\textcolor[RGB]{255,140,0}{iders}\textcolor{black}{.} \textcolor{black}{ It} \textcolor{black}{ does} \textcolor{black}{ not} \textcolor{black}{ reduce} \textcolor{black}{ any} \textcolor{black}{ further} \textcolor{black}{ }\textcolor{black}{1}\textcolor{black}{7}\textcolor{black}{-}\textcolor{black}{bit}\textcolor{black}{ters}\textcolor{black}{,} \textcolor{black}{ though}\textcolor{black}{.} \textcolor{black}{ Princess} \textcolor{black}{ of} \textcolor{black}{ Science}\textcolor{black}{,} \textcolor{black}{ Par}\textcolor{black}{c}\textcolor{black}{ly} \textcolor{black}{ Tax}\textcolor{black}{el} \textcolor{black}{ Kaz}\textcolor{black}{yan} \textcolor{black}{ Post}\textcolor[RGB]{255,140,0}{s}\textcolor{black}{:} \textcolor{black}{ }\textcolor{black}{8}\textcolor{black}{6}\textcolor{black}{7} \textcolor{black}{ Jo}\textcolor{black}{ined}\textcolor[RGB]{255,140,0}{:} \textcolor{black}{ February} \textcolor{black}{ }\textcolor{black}{6}\textcolor{black}{th}\textcolor{black}{,} \textcolor{black}{ }\textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{0}\textcolor{black}{1}\textcolor{black}{4}\textcolor[RGB]{255,140,0}{,} \textcolor{black}{ }\textcolor{black}{1}\textcolor{black}{1}\textcolor{black}{:}\textcolor{black}{0}\textcolor{black}{2} \textcolor{black}{ pm} \textcolor{black}{ \#\#\#} \textcolor[RGB]{255,140,0}{ Re}\textcolor{black}{:} \textcolor[RGB]{255,140,0}{ }\textcolor[RGB]{255,140,0}{1}\textcolor{black}{7} \textcolor{black}{ in} \textcolor{black}{ }\textcolor{black}{1}\textcolor{black}{7}\textcolor{black}{:} \textcolor[RGB]{255,140,0}{ E}\textcolor[RGB]{255,140,0}{fficient} \textcolor{black}{ }\textcolor{black}{1}\textcolor{black}{7}\textcolor{black}{-}\textcolor{black}{bit} \textcolor{black}{ synth}\textcolor{black}{esis} \textcolor{black}{ project} \textcolor{black}{ Good} \textcolor{black}{ catch}\textcolor{black}{,} \textcolor{black}{ S}\textcolor{black}{ok}\textcolor[RGB]{255,140,0}{we}\textcolor{black}{.} \textcolor{black}{ \#}\textcolor{black}{6}\textcolor{black}{1} \textcolor{black}{ in} \textcolor{black}{ }\textcolor{black}{1}\textcolor{black}{5}\textcolor{black}{G}\textcolor{black}{:}
\\ \hline
\textcolor{black}{ Gr}\textcolor{black}{ound} \textcolor{black}{ Pen}\textcolor[RGB]{255,140,0}{etr}\textcolor[RGB]{255,140,0}{ating} \textcolor[RGB]{255,140,0}{ Rad}\textcolor[RGB]{255,140,0}{ar} \textcolor{black}{ for} \textcolor{black}{ Arch}\textcolor[RGB]{255,140,0}{ae}\textcolor{black}{ology} \textcolor{black}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{Work}\textcolor{black}{shop} \textcolor{black}{ |} \textcolor[RGB]{255,140,0}{ December}\textcolor[RGB]{255,140,0}{ }\textcolor{black}{1} \textcolor[RGB]{255,140,0}{ |} \textcolor{black}{ }\textcolor{black}{1}\textcolor{black}{-}\textcolor{black}{5} \textcolor[RGB]{255,140,0}{ p}\textcolor{black}{.}\textcolor{black}{m}\textcolor{black}{.} \textcolor[RGB]{255,140,0}{ |} \textcolor{black}{ }\textcolor{black}{1}\textcolor{black}{0}\textcolor{black}{1}\textcolor{black}{ }\textcolor{black}{2}\textcolor{black}{2}\textcolor{black}{5}\textcolor{black}{1} \textcolor{black}{ College} \textcolor{black}{ (}\textcolor{black}{Arch}\textcolor[RGB]{255,140,0}{ae}\textcolor{black}{ological} \textcolor{black}{ Research} \textcolor{black}{ Fac}\textcolor{black}{ility}\textcolor{black}{)} \textcolor{black}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{Sc}\textcolor{black}{ott} \textcolor{black}{ By}\textcolor{black}{ram}\textcolor{black}{,} \textcolor{black}{ Research} \textcolor{black}{ Associ}\textcolor[RGB]{255,140,0}{ate}\textcolor[RGB]{255,140,0}{,} \textcolor{black}{ Arch}\textcolor{black}{ae}\textcolor[RGB]{255,140,0}{ological} \textcolor{black}{ Research} \textcolor[RGB]{255,140,0}{ Fac}\textcolor[RGB]{255,140,0}{ility}\textcolor{black}{,} \textcolor{black}{ U}\textcolor[RGB]{255,140,0}{C} \textcolor[RGB]{255,140,0}{ Ber}\textcolor[RGB]{255,140,0}{keley} \textcolor{black}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{Arch}\textcolor{black}{ae}\textcolor{black}{ological} \textcolor{black}{ Research} \textcolor[RGB]{255,140,0}{ Fac}\textcolor{black}{ility} \textcolor{black}{ \textbackslash n } \textcolor[RGB]{255,140,0}{ \textbackslash n }\textcolor{black}{At} \textcolor{black}{ }\textcolor{black}{1}\textcolor{black}{pm} \textcolor{black}{ the} \textcolor{black}{ work}\textcolor{black}{shop} \textcolor{black}{ will} \textcolor{black}{ begin} \textcolor{black}{ at} \textcolor{black}{ the} \textcolor{black}{ U}\textcolor{black}{C} \textcolor{black}{ Fac}\textcolor[RGB]{255,140,0}{ulty} \textcolor{black}{ Club} \textcolor{black}{ la}\textcolor{black}{wn} \textcolor{black}{ where} \textcolor{black}{ sub}\textcolor{black}{sur}\textcolor{black}{face} \textcolor{black}{ features} \textcolor{black}{ are} \textcolor{black}{ being} \textcolor{black}{ mapped}\textcolor{black}{.} \textcolor{black}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{\#\#}\textcolor[RGB]{255,140,0}{\#} \textcolor{black}{ Student} \textcolor{black}{ Pro}\textcolor{black}{b}\textcolor[RGB]{255,140,0}{ability}\textcolor{black}{/}\textcolor{black}{P}\textcolor{black}{DE} \textcolor{black}{ Sem}\textcolor{black}{inar}\textcolor{black}{:} \textcolor{black}{ Lar}\textcolor{black}{ge} \textcolor{black}{ De}\textcolor{black}{viation} \textcolor{black}{ Princi}\textcolor{black}{ple} \textcolor{black}{ for} \textcolor{black}{ random} \textcolor{black}{ graphs} \textcolor{black}{ II} \textcolor{black}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{Sem}\textcolor{black}{inar} \textcolor[RGB]{255,140,0}{ |} \textcolor{black}{ December}\textcolor[RGB]{255,140,0}{ }\textcolor[RGB]{255,140,0}{1} \textcolor[RGB]{255,140,0}{ |} \textcolor{black}{ }\textcolor{black}{2}\textcolor{black}{:}\textcolor{black}{1}\textcolor{black}{0}\textcolor[RGB]{255,140,0}{-}\textcolor{black}{3}\textcolor{black}{:}\textcolor{black}{3}\textcolor[RGB]{255,140,0}{0} \textcolor{black}{ p}\textcolor{black}{.}\textcolor{black}{m}\textcolor[RGB]{255,140,0}{.} \textcolor[RGB]{255,140,0}{ |} \textcolor{black}{ }\textcolor{black}{8}\textcolor{black}{9}\textcolor{black}{1}\textcolor[RGB]{255,140,0}{ }\textcolor{black}{E}\textcolor[RGB]{255,140,0}{v}\textcolor{black}{ans} \textcolor[RGB]{255,140,0}{ Hall} \textcolor{black}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{F}\textcolor{black}{ray}\textcolor{black}{d}\textcolor{black}{oun} \textcolor{black}{ Re}\textcolor{black}{zak}\textcolor{black}{han}\textcolor[RGB]{255,140,0}{lou}\textcolor[RGB]{255,140,0}{,} \textcolor{black}{ U}\textcolor{black}{C} \textcolor{black}{ Ber}\textcolor[RGB]{255,140,0}{keley} \textcolor{black}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{Dep}\textcolor[RGB]{255,140,0}{art}\textcolor[RGB]{255,140,0}{ment} \textcolor[RGB]{255,140,0}{ of} \textcolor{black}{ Mathemat}\textcolor[RGB]{255,140,0}{ics} \textcolor[RGB]{255,140,0}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{\#\#}\textcolor[RGB]{255,140,0}{\#} \textcolor{black}{ B}\textcolor{black}{LC} \textcolor{black}{ F}\textcolor{black}{ell}\textcolor[RGB]{255,140,0}{ows} \textcolor{black}{ Forum} \textcolor{black}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{Pres}\textcolor{black}{entation} \textcolor[RGB]{255,140,0}{ |} \textcolor{black}{ December}\textcolor[RGB]{255,140,0}{ }\textcolor{black}{1} \textcolor{black}{ |} \textcolor{black}{ }\textcolor{black}{3}\textcolor{black}{-}\textcolor{black}{5} \textcolor{black}{ p}\textcolor{black}{.}\textcolor{black}{m}\textcolor[RGB]{255,140,0}{.} \textcolor[RGB]{255,140,0}{ |} \textcolor{black}{ D}\textcolor{black}{win}\textcolor{black}{elle} \textcolor{black}{ Hall}\textcolor{black}{,} \textcolor{black}{ B}\textcolor{black}{-}\textcolor{black}{4} \textcolor{black}{ (}\textcolor{black}{Class}\textcolor[RGB]{255,140,0}{room} \textcolor{black}{ side}\textcolor{black}{)} \textcolor{black}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{F}\textcolor{black}{All} \textcolor{black}{ }\textcolor[RGB]{255,140,0}{2}\textcolor[RGB]{255,140,0}{0}\textcolor[RGB]{255,140,0}{1}\textcolor[RGB]{255,140,0}{7} \textcolor{black}{ B}\textcolor[RGB]{255,140,0}{LC} \textcolor{black}{ F}\textcolor{black}{ell}\textcolor[RGB]{255,140,0}{ows}\textcolor{black}{,} \textcolor{black}{ U}\textcolor{black}{C} \textcolor{black}{ Ber}\textcolor[RGB]{255,140,0}{keley} \textcolor{black}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{Ber}\textcolor[RGB]{255,140,0}{keley} \textcolor{black}{ Language} \textcolor[RGB]{255,140,0}{ Center} \textcolor{black}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{T}\textcolor{black}{each}\textcolor{black}{ing} \textcolor{black}{ French} \textcolor{black}{ List}\textcolor{black}{ening} \textcolor{black}{ Com}\textcolor[RGB]{255,140,0}{pre}\textcolor[RGB]{255,140,0}{h}\textcolor{black}{ension} \textcolor{black}{ and} \textcolor{black}{ Cultural} \textcolor{black}{ A}\textcolor[RGB]{255,140,0}{war}\textcolor[RGB]{255,140,0}{eness} \textcolor{black}{ through} \textcolor{black}{ Regional} \textcolor{black}{ Vari}\textcolor{black}{ation} \textcolor{black}{ \textbackslash n }\textcolor{black}{E}\textcolor{black}{ly}\textcolor{black}{se} \textcolor{black}{ R}\textcolor{black}{itch}\textcolor{black}{ey}\textcolor{black}{,} \textcolor{black}{ G}\textcolor{black}{SR}\textcolor{black}{,} \textcolor{black}{ French} \textcolor{black}{ \textbackslash n }\textcolor{black}{At} \textcolor{black}{ the} \textcolor{black}{ university} \textcolor{black}{ level}\textcolor{black}{,} \textcolor{black}{ French} \textcolor{black}{ language} \textcolor{black}{ instruction} \textcolor{black}{ in} \textcolor{black}{ the} \textcolor{black}{ US} \textcolor{black}{ tradition}\textcolor[RGB]{255,140,0}{ally} \textcolor{black}{ includes} \textcolor{black}{ a} \textcolor{black}{ course} \textcolor{black}{ on} \textcolor{black}{ ph}\textcolor[RGB]{255,140,0}{on}\textcolor{black}{et}\textcolor[RGB]{255,140,0}{ics} \textcolor{black}{ and} \textcolor{black}{ pron}\textcolor[RGB]{255,140,0}{unci}\textcolor[RGB]{255,140,0}{ation}\textcolor{black}{.} \textcolor{black}{ While} \textcolor{black}{ the} \textcolor{black}{ major} \textcolor{black}{ aim} \textcolor{black}{ of} \textcolor{black}{ such} \textcolor{black}{ courses} \textcolor{black}{ is} \textcolor{black}{ to} \textcolor{black}{ improve} \textcolor{black}{ students}\textcolor{black}{’} \textcolor{black}{ speaking} \textcolor{black}{ and} \textcolor{black}{ listening} \textcolor{black}{ compet}\textcolor{black}{ence}\textcolor{black}{,} \textcolor{black}{ they} \textcolor{black}{ also} \textcolor{black}{ emphas}\textcolor{black}{ize} \textcolor{black}{ speaking} \textcolor{black}{ ‘}\textcolor{black}{correct}\textcolor{black}{ly}\textcolor[RGB]{255,140,0}{’} \textcolor{black}{ using}\textcolor{black}{...}\textcolor{black}{  } \textcolor{black}{ More} \textcolor[RGB]{255,140,0}{ >} \textcolor{black}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{\#\#}\textcolor[RGB]{255,140,0}{\#} \textcolor{black}{ M}\textcolor{black}{EN}\textcolor{black}{A} \textcolor{black}{ Sal}\textcolor[RGB]{255,140,0}{on} \textcolor{black}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{Work}\textcolor{black}{shop} \textcolor{black}{ |} \textcolor[RGB]{255,140,0}{ December}\textcolor[RGB]{255,140,0}{ }\textcolor{black}{1} \textcolor{black}{ |} \textcolor{black}{ }\textcolor{black}{3}\textcolor{black}{-}\textcolor{black}{4} \textcolor{black}{ p}\textcolor{black}{.}\textcolor{black}{m}\textcolor{black}{.} \textcolor[RGB]{255,140,0}{ |} \textcolor{black}{ }\textcolor{black}{3}\textcolor{black}{4}\textcolor{black}{0}\textcolor[RGB]{255,140,0}{ }\textcolor{black}{Ste}\textcolor[RGB]{255,140,0}{ph}\textcolor[RGB]{255,140,0}{ens} \textcolor{black}{ Hall} \textcolor{black}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{Every} \textcolor{black}{ Friday} \textcolor{black}{ in} \textcolor{black}{ the} \textcolor{black}{ sem}\textcolor[RGB]{255,140,0}{ester}\textcolor{black}{,} \textcolor{black}{ the} \textcolor{black}{ C}\textcolor[RGB]{255,140,0}{ME}\textcolor[RGB]{255,140,0}{S} \textcolor{black}{ hosts} \textcolor{black}{ an} \textcolor{black}{ inform}\textcolor[RGB]{255,140,0}{al} \textcolor{black}{ week}
\\ \bottomrule
\end{tabular}
}
\caption{\textbf{An example of an abnormal state of token perplexity during pretrainig process.} The tokens highlighted in \textcolor[RGB]{255,140,0}{orange} represent tokens that were significant abnormalities during the pretraining process.}
\label{tab:example_fluctuating_token}
\end{table*}

==> table/token_reweight_strategy.tex <==
\begin{table*}[t]
\centering
\small
% \setlength{\tabcolsep}{2pt}
\caption{Exploration and ablation results of different token reweight strategies. The selected base model is TinyLLaMA, employing the same Reference Model, and each method was trained on 10 billion tokens.}
\label{tab:lossy_ref_result}
\begin{tabular}{l|ccccc|c}
\toprule
\textbf{Model} & \textbf{GSM8K} & \textbf{MATH} & \textbf{SVAMP} & \textbf{ASDiv} & \textbf{MAWPS} & \textbf{AVG} \\
\midrule
Continue Pretrain & 6.4 & 3.6 & 21.0 & 34.4 & 48.2 & 22.7 \\
Mask High Loss & 12.3 & 5.4 & 25.2 & 35.8 & 43.8 & 24.5 \\
Random Mask & 5.8 & 4.4 & 20.8 & 35.7 & 47.5 & 22.8 \\
Reference Mask & 12.1 & 6.2 & 31.3 & 48.2 & 62.6 & 32.1 \\
Lambda Reweight & 12.1 & 5.6 & 29.6 & 43.3 & 53.2 & 28.8 \\
TopK Reweight & 10.1 & 5.4 & 27.5 & 43.1 & 56.5 & 28.5 \\
Rerank Reweight & 12.1 & 5.6 & 29.6 & 43.3 & 53.2 & 28.8 \\
ToT Loss & 12.1 & 5.6 & 29.6 & 43.3 & 53.2 & 28.8 \\
\bottomrule
\end{tabular}
\end{table*}

==> table/token_select_example.tex <==
\begin{table*}[t]
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}p{16cm}@{}}
\toprule
\multicolumn{1}{c}{\textbf{\textit{Token Selected Examples}}}  \\ \midrule

\textcolor[RGB]{30,144,255}{ •} \textcolor{black}{ Process} \textcolor[RGB]{30,144,255}{ the} \textcolor[RGB]{30,144,255}{ student} \textcolor[RGB]{30,144,255}{ answer} \textcolor[RGB]{30,144,255}{ as} \textcolor{black}{ a} \textcolor[RGB]{30,144,255}{ Math} \textcolor{black}{ Object} \textcolor[RGB]{30,144,255}{ Formula}\textcolor[RGB]{30,144,255}{,} \textcolor[RGB]{30,144,255}{ and} \textcolor[RGB]{30,144,255}{ break} \textcolor{black}{ down} \textcolor[RGB]{30,144,255}{ its} \textcolor{black}{ parse} \textcolor{black}{ tree} \textcolor{black}{ by} \textcolor[RGB]{30,144,255}{ its} \textcolor{black}{ top}\textcolor[RGB]{30,144,255}{-}\textcolor{black}{level} \textcolor{black}{ operators}\textcolor[RGB]{30,144,255}{.} \textcolor{black}{ The} \textcolor{black}{ idea} \textcolor{black}{ is} \textcolor[RGB]{30,144,255}{ to} \textcolor{black}{ create} \textcolor[RGB]{30,144,255}{ an} \textcolor[RGB]{30,144,255}{ array} \textcolor[RGB]{30,144,255}{ of} \textcolor{black}{ the} \textcolor{black}{ student}\textcolor[RGB]{30,144,255}{'}\textcolor[RGB]{30,144,255}{s} \textcolor{black}{ primitive} \textcolor[RGB]{30,144,255}{ factors}\textcolor[RGB]{30,144,255}{,} \textcolor[RGB]{30,144,255}{ so} \textcolor{black}{ say} \textcolor{black}{ }\textcolor[RGB]{30,144,255}{3}\textcolor[RGB]{30,144,255}{(}\textcolor[RGB]{30,144,255}{x}\textcolor{black}{+}\textcolor[RGB]{30,144,255}{1}\textcolor[RGB]{30,144,255}{)(}\textcolor[RGB]{30,144,255}{x}\textcolor[RGB]{30,144,255}{+}\textcolor[RGB]{30,144,255}{2}\textcolor[RGB]{30,144,255}{)\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor{black}{ gives} \textcolor{black}{ (}\textcolor[RGB]{30,144,255}{3}\textcolor[RGB]{30,144,255}{,}\textcolor{black}{x}\textcolor[RGB]{30,144,255}{+}\textcolor[RGB]{30,144,255}{1}\textcolor[RGB]{30,144,255}{,}\textcolor[RGB]{30,144,255}{x}\textcolor[RGB]{30,144,255}{+}\textcolor[RGB]{30,144,255}{2}\textcolor[RGB]{30,144,255}{).} \textcolor[RGB]{30,144,255}{ •} \textcolor{black}{ Because} \textcolor[RGB]{30,144,255}{ we} \textcolor{black}{ may} \textcolor{black}{ want} \textcolor{black}{ factor}\textcolor[RGB]{30,144,255}{ing} \textcolor{black}{ over} \textcolor{black}{ Z}\textcolor[RGB]{30,144,255}{,} \textcolor[RGB]{30,144,255}{ checking} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ g}\textcolor[RGB]{30,144,255}{cd} \textcolor[RGB]{30,144,255}{ of} \textcolor[RGB]{30,144,255}{ coefficients} \textcolor{black}{ within} \textcolor[RGB]{30,144,255}{ each} \textcolor{black}{ factor}\textcolor[RGB]{30,144,255}{.} \textcolor{black}{ •} \textcolor[RGB]{30,144,255}{ Pass} \textcolor{black}{ each} \textcolor[RGB]{30,144,255}{ of} \textcolor[RGB]{30,144,255}{ these} \textcolor{black}{ things} \textcolor[RGB]{30,144,255}{ to} \textcolor{black}{ S}\textcolor{black}{AGE} \textcolor{black}{ and} \textcolor{black}{ ask} \textcolor[RGB]{30,144,255}{ if} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ non}\textcolor{black}{constant} \textcolor[RGB]{30,144,255}{ factors} \textcolor[RGB]{30,144,255}{ are} \textcolor{black}{ redu}\textcolor[RGB]{30,144,255}{cible} \textcolor{black}{ over} \textcolor[RGB]{30,144,255}{ Z} \textcolor{black}{ or} \textcolor[RGB]{30,144,255}{ Q}\textcolor[RGB]{30,144,255}{.} \textcolor{black}{ Also} \textcolor[RGB]{30,144,255}{ ask} \textcolor[RGB]{30,144,255}{ if} \textcolor{black}{ they} \textcolor[RGB]{30,144,255}{ are} \textcolor{black}{ mon}\textcolor[RGB]{30,144,255}{ic}\textcolor[RGB]{30,144,255}{.} \textcolor[RGB]{30,144,255}{ These} \textcolor{black}{ things} \textcolor{black}{ at} \textcolor{black}{ least} \textcolor{black}{ we} \textcolor[RGB]{30,144,255}{ learned} \textcolor{black}{ how} \textcolor[RGB]{30,144,255}{ to} \textcolor[RGB]{30,144,255}{ do} \textcolor{black}{ at} \textcolor{black}{ the} \textcolor{black}{ V}\textcolor{black}{ancouver} \textcolor[RGB]{30,144,255}{ code} \textcolor[RGB]{30,144,255}{ camp}\textcolor[RGB]{30,144,255}{.} \textcolor{black}{ The} \textcolor{black}{ end} \textcolor{black}{ goal} \textcolor[RGB]{30,144,255}{ is} \textcolor[RGB]{30,144,255}{ to} \textcolor{black}{ count} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ following} \textcolor[RGB]{30,144,255}{ forms} \textcolor{black}{ as} \textcolor[RGB]{30,144,255}{ correct}\textcolor[RGB]{30,144,255}{,} \textcolor{black}{ possibly} \textcolor{black}{ controlled} \textcolor[RGB]{30,144,255}{ by} \textcolor[RGB]{30,144,255}{ flags}\textcolor[RGB]{30,144,255}{:} \textcolor{black}{ n} \textcolor[RGB]{30,144,255}{ \textbackslash\{\}}\textcolor{black}{prod} \textcolor{black}{ (}\textcolor{black}{factor}\textcolor[RGB]{30,144,255}{)\^{}}\textcolor{black}{power}\textcolor[RGB]{30,144,255}{,} \textcolor[RGB]{30,144,255}{ where} \textcolor{black}{ each} \textcolor[RGB]{30,144,255}{ factor} \textcolor{black}{ is} \textcolor{black}{ ir}\textcolor[RGB]{30,144,255}{reducible} \textcolor{black}{ in} \textcolor[RGB]{30,144,255}{ Z}\textcolor{black}{{[}}\textcolor{black}{X}\textcolor{black}{{]},} \textcolor[RGB]{30,144,255}{ n} \textcolor[RGB]{30,144,255}{ in} \textcolor[RGB]{30,144,255}{ Z} \textcolor{black}{ r} \textcolor{black}{ \textbackslash\{\}}\textcolor[RGB]{30,144,255}{prod} \textcolor[RGB]{30,144,255}{ (}\textcolor[RGB]{30,144,255}{factor}\textcolor[RGB]{30,144,255}{)\^{}}\textcolor[RGB]{30,144,255}{power}\textcolor[RGB]{30,144,255}{,} \textcolor{black}{ where} \textcolor[RGB]{30,144,255}{ each} \textcolor[RGB]{30,144,255}{ factor} \textcolor[RGB]{30,144,255}{ is} \textcolor[RGB]{30,144,255}{ ir}\textcolor[RGB]{30,144,255}{reducible} \textcolor{black}{ and} \textcolor{black}{ mon}\textcolor[RGB]{30,144,255}{ic} \textcolor[RGB]{30,144,255}{ in} \textcolor[RGB]{30,144,255}{ Q}\textcolor{black}{{[}}\textcolor[RGB]{30,144,255}{X}\textcolor[RGB]{30,144,255}{{]},} \textcolor{black}{ r} \textcolor[RGB]{30,144,255}{ in} \textcolor{black}{ Q} \textcolor{black}{ I} \textcolor{black}{ suppose} \textcolor{black}{ on} \textcolor[RGB]{30,144,255}{ the} \textcolor[RGB]{30,144,255}{ last} \textcolor[RGB]{30,144,255}{ one} \textcolor{black}{ the} \textcolor{black}{ mon}\textcolor[RGB]{30,144,255}{ic} \textcolor{black}{ requirement} \textcolor{black}{ could} \textcolor{black}{ be} \textcolor[RGB]{30,144,255}{ dropped} \textcolor[RGB]{30,144,255}{ with} \textcolor[RGB]{30,144,255}{ a} \textcolor{black}{ flag}\textcolor[RGB]{30,144,255}{.} \textcolor{black}{ I} \textcolor[RGB]{30,144,255}{ have} \textcolor[RGB]{30,144,255}{ no} \textcolor{black}{ plans} \textcolor[RGB]{30,144,255}{ to} \textcolor{black}{ check} \textcolor[RGB]{30,144,255}{ that} \textcolor{black}{ the} \textcolor[RGB]{30,144,255}{ form} \textcolor[RGB]{30,144,255}{ is} \textcolor[RGB]{30,144,255}{ fully} \textcolor[RGB]{30,144,255}{ cond}\textcolor[RGB]{30,144,255}{ensed}\textcolor[RGB]{30,144,255}{,} \textcolor{black}{ e}\textcolor[RGB]{30,144,255}{.}\textcolor[RGB]{30,144,255}{g}\textcolor[RGB]{30,144,255}{.} \textcolor{black}{ forcing} \textcolor[RGB]{30,144,255}{ (}\textcolor[RGB]{30,144,255}{x}\textcolor[RGB]{30,144,255}{+}\textcolor[RGB]{30,144,255}{1}\textcolor[RGB]{30,144,255}{)\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ and} \textcolor[RGB]{30,144,255}{ reject}\textcolor[RGB]{30,144,255}{ing} \textcolor[RGB]{30,144,255}{ (}\textcolor[RGB]{30,144,255}{x}\textcolor[RGB]{30,144,255}{+}\textcolor[RGB]{30,144,255}{1}\textcolor{black}{)(}\textcolor[RGB]{30,144,255}{1}\textcolor[RGB]{30,144,255}{+}\textcolor[RGB]{30,144,255}{x}\textcolor[RGB]{30,144,255}{)}
\\ \hline
\textcolor{black}{The} \textcolor{black}{ equation} \textcolor[RGB]{30,144,255}{ of} \textcolor{black}{ the} \textcolor[RGB]{30,144,255}{ path} \textcolor{black}{ travers}\textcolor[RGB]{30,144,255}{ed} \textcolor[RGB]{30,144,255}{ by} \textcolor{black}{ a} \textcolor{black}{ project}\textcolor[RGB]{30,144,255}{ile} \textcolor[RGB]{30,144,255}{ is} \textcolor{black}{ called} \textcolor{black}{ equation} \textcolor[RGB]{30,144,255}{ of} \textcolor[RGB]{30,144,255}{ traject}\textcolor[RGB]{30,144,255}{ory}\textcolor[RGB]{30,144,255}{.} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{Supp}\textcolor[RGB]{30,144,255}{ose}\textcolor[RGB]{30,144,255}{,} \textcolor{black}{ the} \textcolor{black}{ body} \textcolor{black}{ reaches} \textcolor[RGB]{30,144,255}{ the} \textcolor[RGB]{30,144,255}{ point} \textcolor{black}{ P} \textcolor[RGB]{30,144,255}{ after} \textcolor[RGB]{30,144,255}{ time} \textcolor{black}{ (} \textcolor[RGB]{30,144,255}{ t} \textcolor{black}{ )} \textcolor{black}{ .} \textcolor{black}{ \textbackslash n } \textcolor{black}{ \textbackslash n }\textcolor{black}{Horizontal} \textcolor{black}{ motion} \textcolor[RGB]{30,144,255}{ has} \textcolor{black}{ no} \textcolor{black}{ acceleration}\textcolor{black}{.} \textcolor[RGB]{30,144,255}{ Thus}\textcolor[RGB]{30,144,255}{,} \textcolor[RGB]{30,144,255}{ using} \textcolor[RGB]{30,144,255}{ kin}\textcolor[RGB]{30,144,255}{ematic} \textcolor[RGB]{30,144,255}{ equation}\textcolor[RGB]{30,144,255}{,} \textcolor{black}{ horizontal} \textcolor[RGB]{30,144,255}{ distance} \textcolor[RGB]{30,144,255}{ covered} \textcolor[RGB]{30,144,255}{ will} \textcolor[RGB]{30,144,255}{ be} \textcolor{black}{ –} \textcolor{black}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{x} \textcolor{black}{ =} \textcolor{black}{ u} \textcolor{black}{ \textbackslash }\textcolor[RGB]{30,144,255}{cos} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{theta} \textcolor{black}{ t} \textcolor{black}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{Or}\textcolor{black}{,} \textcolor{black}{ \textbackslash }\textcolor{black}{quad} \textcolor{black}{ t} \textcolor[RGB]{30,144,255}{ =} \textcolor[RGB]{30,144,255}{ (} \textcolor{black}{ \textbackslash }\textcolor[RGB]{30,144,255}{frac} \textcolor[RGB]{30,144,255}{ \{} \textcolor{black}{ x} \textcolor{black}{ \}\{} \textcolor[RGB]{30,144,255}{ u} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{cos} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{theta} \textcolor[RGB]{30,144,255}{ \}} \textcolor[RGB]{30,144,255}{ )} \textcolor{black}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor[RGB]{30,144,255}{Vertical} \textcolor[RGB]{30,144,255}{ motion} \textcolor[RGB]{30,144,255}{ has} \textcolor[RGB]{30,144,255}{ constant} \textcolor[RGB]{30,144,255}{ acceleration} \textcolor{black}{ (} \textcolor[RGB]{30,144,255}{ g} \textcolor[RGB]{30,144,255}{ )} \textcolor[RGB]{30,144,255}{ .} \textcolor[RGB]{30,144,255}{ Thus}\textcolor[RGB]{30,144,255}{,} \textcolor[RGB]{30,144,255}{ distance} \textcolor[RGB]{30,144,255}{ covered} \textcolor[RGB]{30,144,255}{ will} \textcolor[RGB]{30,144,255}{ be} \textcolor{black}{ –} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor[RGB]{30,144,255}{y} \textcolor[RGB]{30,144,255}{ =} \textcolor[RGB]{30,144,255}{ (} \textcolor[RGB]{30,144,255}{ u} \textcolor{black}{ \textbackslash }\textcolor[RGB]{30,144,255}{sin} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{theta} \textcolor{black}{ )}\textcolor{black}{ } \textcolor{black}{ t} \textcolor{black}{ -} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor{black}{left} \textcolor[RGB]{30,144,255}{ (} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{frac} \textcolor[RGB]{30,144,255}{ \{}\textcolor{black}{1}\textcolor[RGB]{30,144,255}{\}\{}\textcolor[RGB]{30,144,255}{2}\textcolor[RGB]{30,144,255}{\}} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{right} \textcolor[RGB]{30,144,255}{ )} \textcolor[RGB]{30,144,255}{ g} \textcolor{black}{ t}\textcolor{black}{\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{=} \textcolor{black}{ (} \textcolor[RGB]{30,144,255}{ u} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{sin} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{theta} \textcolor[RGB]{30,144,255}{ )} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{left} \textcolor[RGB]{30,144,255}{ (} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{frac} \textcolor{black}{ \{}\textcolor{black}{x}\textcolor[RGB]{30,144,255}{\}\{}\textcolor[RGB]{30,144,255}{u} \textcolor{black}{ \textbackslash }\textcolor[RGB]{30,144,255}{cos} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{theta}\textcolor[RGB]{30,144,255}{\}} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{right} \textcolor[RGB]{30,144,255}{ )} \textcolor[RGB]{30,144,255}{ -} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{left} \textcolor[RGB]{30,144,255}{ (} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{frac} \textcolor[RGB]{30,144,255}{ \{}\textcolor[RGB]{30,144,255}{1}\textcolor[RGB]{30,144,255}{\}\{}\textcolor[RGB]{30,144,255}{2}\textcolor[RGB]{30,144,255}{\}} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{right} \textcolor[RGB]{30,144,255}{ )} \textcolor[RGB]{30,144,255}{ g} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{left} \textcolor[RGB]{30,144,255}{ (} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{frac} \textcolor[RGB]{30,144,255}{ \{}\textcolor{black}{x}\textcolor[RGB]{30,144,255}{\}\{}\textcolor[RGB]{30,144,255}{u} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{cos} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{theta}\textcolor[RGB]{30,144,255}{\}} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{right} \textcolor{black}{ )}\textcolor[RGB]{30,144,255}{\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{=} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{left} \textcolor[RGB]{30,144,255}{ (} \textcolor{black}{ \textbackslash }\textcolor{black}{tan} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{theta} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{right} \textcolor[RGB]{30,144,255}{ )} \textcolor[RGB]{30,144,255}{ x} \textcolor[RGB]{30,144,255}{ -} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor{black}{left} \textcolor[RGB]{30,144,255}{ (} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{frac} \textcolor[RGB]{30,144,255}{ \{}\textcolor{black}{g}\textcolor[RGB]{30,144,255}{\}\{}\textcolor{black}{2} \textcolor[RGB]{30,144,255}{ u}\textcolor{black}{\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor{black}{cos}\textcolor[RGB]{30,144,255}{\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{theta}\textcolor[RGB]{30,144,255}{\}} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{right} \textcolor[RGB]{30,144,255}{ )} \textcolor{black}{ x}\textcolor[RGB]{30,144,255}{\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{In} \textcolor{black}{ this} \textcolor[RGB]{30,144,255}{ equation}\textcolor{black}{,} \textcolor[RGB]{30,144,255}{ (} \textcolor{black}{ \textbackslash }\textcolor{black}{theta}\textcolor[RGB]{30,144,255}{,} \textcolor{black}{ \textbackslash } \textcolor[RGB]{30,144,255}{ u} \textcolor{black}{ \textbackslash } \textcolor{black}{ \textbackslash }\textcolor{black}{text} \textcolor[RGB]{30,144,255}{ \{}\textcolor[RGB]{30,144,255}{and}\textcolor{black}{\}} \textcolor[RGB]{30,144,255}{ \textbackslash } \textcolor{black}{ g} \textcolor[RGB]{30,144,255}{ )} \textcolor[RGB]{30,144,255}{ are} \textcolor{black}{ constants}\textcolor{black}{.} \textcolor[RGB]{30,144,255}{ Thus}\textcolor[RGB]{30,144,255}{,} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor[RGB]{30,144,255}{1}\textcolor{black}{.} \textcolor[RGB]{30,144,255}{ Term} \textcolor{black}{ \textbackslash }\textcolor{black}{left} \textcolor[RGB]{30,144,255}{ (} \textcolor{black}{ \textbackslash }\textcolor{black}{tan} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{theta} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{right} \textcolor[RGB]{30,144,255}{ )} \textcolor[RGB]{30,144,255}{ is} \textcolor{black}{ a} \textcolor{black}{ constant}\textcolor[RGB]{30,144,255}{,} \textcolor{black}{ let} \textcolor{black}{ it} \textcolor{black}{ is} \textcolor{black}{ (} \textcolor{black}{ p} \textcolor{black}{ )} \textcolor{black}{ \textbackslash n }\textcolor{black}{2}\textcolor[RGB]{30,144,255}{.} \textcolor{black}{ Term} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{left} \textcolor[RGB]{30,144,255}{ {[}} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{left} \textcolor[RGB]{30,144,255}{ (} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{frac} \textcolor[RGB]{30,144,255}{ \{}\textcolor[RGB]{30,144,255}{g}\textcolor[RGB]{30,144,255}{\}\{}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ u}\textcolor[RGB]{30,144,255}{\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{cos}\textcolor[RGB]{30,144,255}{\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{theta}\textcolor[RGB]{30,144,255}{\}} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{right} \textcolor[RGB]{30,144,255}{ )} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor{black}{right} \textcolor[RGB]{30,144,255}{ {]}} \textcolor[RGB]{30,144,255}{ is} \textcolor{black}{ also} \textcolor[RGB]{30,144,255}{ a} \textcolor[RGB]{30,144,255}{ constant}\textcolor[RGB]{30,144,255}{,} \textcolor[RGB]{30,144,255}{ let} \textcolor[RGB]{30,144,255}{ it} \textcolor{black}{ is} \textcolor{black}{ (} \textcolor[RGB]{30,144,255}{ q} \textcolor[RGB]{30,144,255}{ )} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor[RGB]{30,144,255}{So}\textcolor{black}{,} \textcolor{black}{ \textbackslash }\textcolor{black}{quad} \textcolor{black}{ y} \textcolor[RGB]{30,144,255}{ =} \textcolor{black}{ p} \textcolor[RGB]{30,144,255}{ x} \textcolor[RGB]{30,144,255}{ -} \textcolor{black}{ q} \textcolor[RGB]{30,144,255}{ x}\textcolor[RGB]{30,144,255}{\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{There}\textcolor[RGB]{30,144,255}{fore}\textcolor[RGB]{30,144,255}{,} \textcolor[RGB]{30,144,255}{ (} \textcolor{black}{ y} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor{black}{pro}\textcolor[RGB]{30,144,255}{pto} \textcolor[RGB]{30,144,255}{ x}\textcolor[RGB]{30,144,255}{\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor{black}{ )} \textcolor[RGB]{30,144,255}{ ,} \textcolor[RGB]{30,144,255}{ which} \textcolor[RGB]{30,144,255}{ is} \textcolor[RGB]{30,144,255}{ a} \textcolor[RGB]{30,144,255}{ required} \textcolor{black}{ condition} \textcolor{black}{ of} \textcolor{black}{ a} \textcolor{black}{ par}\textcolor{black}{ab}\textcolor[RGB]{30,144,255}{ola}\textcolor[RGB]{30,144,255}{.} 
\\ \hline 
\textcolor[RGB]{30,144,255}{The} \textcolor[RGB]{30,144,255}{ traject}\textcolor[RGB]{30,144,255}{ory} \textcolor[RGB]{30,144,255}{ of} \textcolor[RGB]{30,144,255}{ the} \textcolor[RGB]{30,144,255}{ project}\textcolor[RGB]{30,144,255}{ile} \textcolor{black}{ is} \textcolor[RGB]{30,144,255}{ a} \textcolor[RGB]{30,144,255}{ par}\textcolor[RGB]{30,144,255}{ab}\textcolor[RGB]{30,144,255}{ola}\textcolor{black}{.} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{\#\#}\textcolor{black}{\#} \textcolor{black}{ Time} \textcolor{black}{ of} \textcolor[RGB]{30,144,255}{ Max}\textcolor[RGB]{30,144,255}{imum} \textcolor{black}{ height} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{As} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ body} \textcolor[RGB]{30,144,255}{ is} \textcolor[RGB]{30,144,255}{ project}\textcolor[RGB]{30,144,255}{ed} \textcolor{black}{ it} \textcolor{black}{ goes} \textcolor{black}{ up}\textcolor[RGB]{30,144,255}{.} \textcolor[RGB]{30,144,255}{ Vert}\textcolor[RGB]{30,144,255}{ical} \textcolor{black}{ component} \textcolor[RGB]{30,144,255}{ of} \textcolor[RGB]{30,144,255}{ velocity} \textcolor{black}{ (} \textcolor[RGB]{30,144,255}{ u} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{sin} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{theta} \textcolor[RGB]{30,144,255}{ )} \textcolor{black}{ gradually} \textcolor{black}{ dimin}\textcolor[RGB]{30,144,255}{ishes} \textcolor{black}{ and} \textcolor{black}{ becomes} \textcolor[RGB]{30,144,255}{ zero} \textcolor[RGB]{30,144,255}{ at} \textcolor[RGB]{30,144,255}{ the} \textcolor[RGB]{30,144,255}{ maximum} \textcolor[RGB]{30,144,255}{ height} \textcolor{black}{ of} \textcolor{black}{ flight}\textcolor[RGB]{30,144,255}{.} \textcolor{black}{ After} \textcolor[RGB]{30,144,255}{ that}\textcolor[RGB]{30,144,255}{,} \textcolor{black}{ body} \textcolor{black}{ starts} \textcolor{black}{ moving} \textcolor[RGB]{30,144,255}{ down}\textcolor[RGB]{30,144,255}{wards}\textcolor[RGB]{30,144,255}{.} \textcolor{black}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{Let}\textcolor[RGB]{30,144,255}{,} \textcolor{black}{ (} \textcolor{black}{ t}\textcolor{black}{\_}\textcolor{black}{m} \textcolor{black}{ )} \textcolor[RGB]{30,144,255}{ is} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ time} \textcolor[RGB]{30,144,255}{ to} \textcolor[RGB]{30,144,255}{ reach} \textcolor[RGB]{30,144,255}{ at} \textcolor[RGB]{30,144,255}{ maximum} \textcolor[RGB]{30,144,255}{ height} \textcolor{black}{ (} \textcolor[RGB]{30,144,255}{ h}\textcolor{black}{\_}\textcolor[RGB]{30,144,255}{m} \textcolor{black}{ )} \textcolor{black}{ of} \textcolor{black}{ flight}\textcolor[RGB]{30,144,255}{.} \textcolor{black}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{There}\textcolor[RGB]{30,144,255}{fore}\textcolor[RGB]{30,144,255}{,} \textcolor[RGB]{30,144,255}{ from} \textcolor{black}{ kin}\textcolor[RGB]{30,144,255}{ematic} \textcolor{black}{ equation}\textcolor[RGB]{30,144,255}{,} \textcolor{black}{ we} \textcolor[RGB]{30,144,255}{ have} \textcolor{black}{ –} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor[RGB]{30,144,255}{0} \textcolor[RGB]{30,144,255}{ =} \textcolor{black}{ u} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{sin} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{theta} \textcolor{black}{ -} \textcolor{black}{ g} \textcolor[RGB]{30,144,255}{ t}\textcolor[RGB]{30,144,255}{\_}\textcolor[RGB]{30,144,255}{m} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{Or}\textcolor[RGB]{30,144,255}{,}\textcolor{black}{ } \textcolor{black}{ \textbackslash }\textcolor{black}{quad} \textcolor[RGB]{30,144,255}{ t}\textcolor[RGB]{30,144,255}{\_}\textcolor[RGB]{30,144,255}{m} \textcolor[RGB]{30,144,255}{ =} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor{black}{left} \textcolor{black}{ (} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{frac} \textcolor[RGB]{30,144,255}{ \{}\textcolor{black}{u} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{sin} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{theta}\textcolor[RGB]{30,144,255}{\}\{}\textcolor{black}{g}\textcolor[RGB]{30,144,255}{\}} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{right} \textcolor[RGB]{30,144,255}{ )} \textcolor{black}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{\#\#}\textcolor[RGB]{30,144,255}{\#} \textcolor{black}{ Time} \textcolor{black}{ of} \textcolor{black}{ Fl}\textcolor[RGB]{30,144,255}{ight} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor[RGB]{30,144,255}{Total} \textcolor{black}{ time} \textcolor[RGB]{30,144,255}{ taken} \textcolor{black}{ by} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ project}\textcolor[RGB]{30,144,255}{ile} \textcolor{black}{ between} \textcolor{black}{ the} \textcolor{black}{ instant} \textcolor[RGB]{30,144,255}{ it} \textcolor[RGB]{30,144,255}{ is} \textcolor{black}{ project}\textcolor[RGB]{30,144,255}{ed} \textcolor{black}{ and} \textcolor{black}{ till} \textcolor[RGB]{30,144,255}{ it} \textcolor{black}{ reaches} \textcolor[RGB]{30,144,255}{ at} \textcolor{black}{ a} \textcolor[RGB]{30,144,255}{ point} \textcolor{black}{ in} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ horizontal} \textcolor[RGB]{30,144,255}{ plane} \textcolor[RGB]{30,144,255}{ of} \textcolor[RGB]{30,144,255}{ its} \textcolor{black}{ projection} \textcolor{black}{ is} \textcolor{black}{ called} \textcolor{black}{ Time} \textcolor[RGB]{30,144,255}{ of} \textcolor{black}{ flight}\textcolor{black}{.} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{Let}\textcolor[RGB]{30,144,255}{,} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ body} \textcolor{black}{ reaches} \textcolor[RGB]{30,144,255}{ at} \textcolor{black}{ point} \textcolor[RGB]{30,144,255}{ B} \textcolor{black}{ on} \textcolor{black}{ ground} \textcolor[RGB]{30,144,255}{ after} \textcolor{black}{ time} \textcolor{black}{ (} \textcolor[RGB]{30,144,255}{ T}\textcolor{black}{\_}\textcolor[RGB]{30,144,255}{f} \textcolor[RGB]{30,144,255}{ )} \textcolor{black}{ of} \textcolor{black}{ projection}\textcolor[RGB]{30,144,255}{.} \textcolor[RGB]{30,144,255}{ Then} \textcolor{black}{ –} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{Net} \textcolor{black}{ vertical} \textcolor{black}{ disp}\textcolor[RGB]{30,144,255}{lacement} \textcolor{black}{ covered} \textcolor{black}{ during} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ time} \textcolor[RGB]{30,144,255}{ of} \textcolor[RGB]{30,144,255}{ flight} \textcolor[RGB]{30,144,255}{ is} \textcolor{black}{ zero}\textcolor{black}{.} \textcolor{black}{ Using} \textcolor{black}{ kin}\textcolor[RGB]{30,144,255}{ematic} \textcolor{black}{ equation} \textcolor{black}{ of} \textcolor{black}{ motion}\textcolor[RGB]{30,144,255}{,} \textcolor[RGB]{30,144,255}{ we} \textcolor[RGB]{30,144,255}{ get} \textcolor{black}{ –} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{0} \textcolor[RGB]{30,144,255}{ =} \textcolor{black}{ (} \textcolor{black}{ u} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{sin} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{theta} \textcolor{black}{ )} \textcolor[RGB]{30,144,255}{ T}\textcolor[RGB]{30,144,255}{\_}\textcolor[RGB]{30,144,255}{f} \textcolor[RGB]{30,144,255}{ -} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{left} \textcolor[RGB]{30,144,255}{ (} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{frac} \textcolor[RGB]{30,144,255}{ \{}\textcolor[RGB]{30,144,255}{1}\textcolor[RGB]{30,144,255}{\}\{}\textcolor[RGB]{30,144,255}{2}\textcolor[RGB]{30,144,255}{\}} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{right} \textcolor{black}{ )} \textcolor[RGB]{30,144,255}{ g} \textcolor{black}{ \textbackslash } \textcolor{black}{ (} \textcolor[RGB]{30,144,255}{ T}\textcolor[RGB]{30,144,255}{\_}\textcolor[RGB]{30,144,255}{f} \textcolor{black}{ )}\textcolor[RGB]{30,144,255}{\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor[RGB]{30,144,255}{Or}\textcolor[RGB]{30,144,255}{,} \textcolor{black}{ \textbackslash }\textcolor[RGB]{30,144,255}{quad} \textcolor{black}{ T}\textcolor[RGB]{30,144,255}{\_}\textcolor[RGB]{30,144,255}{f} \textcolor[RGB]{30,144,255}{ =} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor{black}{left} \textcolor[RGB]{30,144,255}{ (} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{frac} \textcolor[RGB]{30,144,255}{ \{}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ u} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{sin} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{theta}\textcolor[RGB]{30,144,255}{\}\{}\textcolor[RGB]{30,144,255}{g}\textcolor[RGB]{30,144,255}{\}} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{right} \textcolor{black}{ )} \textcolor[RGB]{30,144,255}{ =} \textcolor{black}{ }\textcolor[RGB]{30,144,255}{2} \textcolor{black}{ \textbackslash }\textcolor{black}{left} \textcolor[RGB]{30,144,255}{ (} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{frac} \textcolor[RGB]{30,144,255}{ \{}\textcolor[RGB]{30,144,255}{u} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{sin} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{theta}\textcolor[RGB]{30,144,255}{\}\{}\textcolor[RGB]{30,144,255}{g}\textcolor[RGB]{30,144,255}{\}} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{right} \textcolor[RGB]{30,144,255}{ )} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{=} \textcolor{black}{ }\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ t}\textcolor[RGB]{30,144,255}{\_}\textcolor[RGB]{30,144,255}{m} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor[RGB]{30,144,255}{Th}\textcolor[RGB]{30,144,255}{us}\textcolor[RGB]{30,144,255}{,} \textcolor{black}{ \textbackslash }\textcolor{black}{quad} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor{black}{text} \textcolor[RGB]{30,144,255}{ \{}\textcolor[RGB]{30,144,255}{Total} \textcolor[RGB]{30,144,255}{ time} \textcolor{black}{ of} \textcolor[RGB]{30,144,255}{ flight}\textcolor{black}{\}} \textcolor[RGB]{30,144,255}{ =} \textcolor{black}{ \textbackslash }\textcolor{black}{text} \textcolor[RGB]{30,144,255}{ \{}\textcolor[RGB]{30,144,255}{Time} \textcolor{black}{ of} \textcolor[RGB]{30,144,255}{ as}\textcolor[RGB]{30,144,255}{cent}\textcolor{black}{\}} \textcolor[RGB]{30,144,255}{ +} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{text} \textcolor[RGB]{30,144,255}{ \{}\textcolor[RGB]{30,144,255}{Time} \textcolor[RGB]{30,144,255}{ of} \textcolor{black}{ descent}\textcolor[RGB]{30,144,255}{\}} \textcolor{black}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor[RGB]{30,144,255}{=} \textcolor{black}{ }\textcolor{black}{2} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor{black}{times} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor{black}{text} \textcolor[RGB]{30,144,255}{ \{}\textcolor[RGB]{30,144,255}{Time} \textcolor{black}{ of} \textcolor[RGB]{30,144,255}{ maximum} \textcolor[RGB]{30,144,255}{ height}\textcolor{black}{.\}} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{\#\#}\textcolor{black}{\#} \textcolor{black}{ Max}\textcolor[RGB]{30,144,255}{imum} \textcolor[RGB]{30,144,255}{ height} \textcolor{black}{ of} \textcolor[RGB]{30,144,255}{ Fl}\textcolor[RGB]{30,144,255}{ight} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor[RGB]{30,144,255}{It} \textcolor[RGB]{30,144,255}{ is} \textcolor{black}{ the} \textcolor[RGB]{30,144,255}{ maximum} \textcolor[RGB]{30,144,255}{ height} \textcolor[RGB]{30,144,255}{ reached} \textcolor[RGB]{30,144,255}{ by} \textcolor[RGB]{30,144,255}{ a} \textcolor[RGB]{30,144,255}{ project}\textcolor[RGB]{30,144,255}{ile}\textcolor{black}{.} \textcolor{black}{ It} \textcolor{black}{ is} \textcolor{black}{ denoted} \textcolor[RGB]{30,144,255}{ by} \textcolor[RGB]{30,144,255}{ (} \textcolor[RGB]{30,144,255}{ h}\textcolor[RGB]{30,144,255}{\_}\textcolor{black}{m} \textcolor[RGB]{30,144,255}{ )} \textcolor{black}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{At} \textcolor[RGB]{30,144,255}{ the} \textcolor[RGB]{30,144,255}{ highest} \textcolor[RGB]{30,144,255}{ point} \textcolor[RGB]{30,144,255}{ of} \textcolor{black}{ flight}\textcolor{black}{,} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ vertical} \textcolor{black}{ component} \textcolor[RGB]{30,144,255}{ of} \textcolor[RGB]{30,144,255}{ velocity} \textcolor[RGB]{30,144,255}{ becomes} \textcolor[RGB]{30,144,255}{ zero}\textcolor[RGB]{30,144,255}{.} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{From} \textcolor{black}{ kin}\textcolor[RGB]{30,144,255}{ematic} \textcolor[RGB]{30,144,255}{ equation} \textcolor{black}{ of} \textcolor[RGB]{30,144,255}{ motion}\textcolor[RGB]{30,144,255}{,} \textcolor{black}{ we} \textcolor{black}{ have} \textcolor{black}{ –} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor[RGB]{30,144,255}{v}\textcolor{black}{\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ =} \textcolor[RGB]{30,144,255}{ u}\textcolor[RGB]{30,144,255}{\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ +} \textcolor{black}{ }\textcolor[RGB]{30,144,255}{2} \textcolor{black}{ a} \textcolor{black}{ s} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor[RGB]{30,144,255}{There}\textcolor[RGB]{30,144,255}{fore}\textcolor[RGB]{30,144,255}{,} \textcolor{black}{ \textbackslash }\textcolor{black}{quad} \textcolor[RGB]{30,144,255}{ }\textcolor[RGB]{30,144,255}{0}\textcolor{black}{\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor{black}{ -} \textcolor{black}{ (} \textcolor[RGB]{30,144,255}{ u} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{sin} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{theta} \textcolor[RGB]{30,144,255}{ )}\textcolor{black}{\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ =} \textcolor{black}{ }\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ (} \textcolor{black}{ -} \textcolor{black}{ g} \textcolor{black}{ )} \textcolor{black}{ h}\textcolor[RGB]{30,144,255}{\_}\textcolor[RGB]{30,144,255}{m} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{Or}\textcolor[RGB]{30,144,255}{,} \textcolor{black}{ \textbackslash }\textcolor[RGB]{30,144,255}{quad} \textcolor{black}{ h}\textcolor[RGB]{30,144,255}{\_}\textcolor[RGB]{30,144,255}{m} \textcolor[RGB]{30,144,255}{ =} \textcolor{black}{ \textbackslash }\textcolor{black}{left} \textcolor[RGB]{30,144,255}{ (} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{frac} \textcolor[RGB]{30,144,255}{ \{}\textcolor{black}{u}\textcolor[RGB]{30,144,255}{\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor{black}{ \textbackslash }\textcolor[RGB]{30,144,255}{sin}\textcolor[RGB]{30,144,255}{\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{theta}\textcolor[RGB]{30,144,255}{\}\{}\textcolor{black}{2} \textcolor[RGB]{30,144,255}{ g}\textcolor[RGB]{30,144,255}{\}} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{right} \textcolor[RGB]{30,144,255}{ )} 
\\ \hline
\textcolor{black}{We} \textcolor[RGB]{30,144,255}{ identify} \textcolor{black}{ two} \textcolor[RGB]{30,144,255}{ equations} \textcolor[RGB]{30,144,255}{ having} \textcolor[RGB]{30,144,255}{ the} \textcolor[RGB]{30,144,255}{ same} \textcolor[RGB]{30,144,255}{ solution} \textcolor{black}{ with} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ equivalence} \textcolor{black}{ relation}\textcolor{black}{:} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor[RGB]{30,144,255}{\$(}\textcolor[RGB]{30,144,255}{a}\textcolor[RGB]{30,144,255}{,}\textcolor[RGB]{30,144,255}{b}\textcolor{black}{)} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{sim} \textcolor[RGB]{30,144,255}{ (}\textcolor[RGB]{30,144,255}{c}\textcolor[RGB]{30,144,255}{,}\textcolor[RGB]{30,144,255}{d}\textcolor{black}{)} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor{black}{mbox}\textcolor[RGB]{30,144,255}{\{} \textcolor[RGB]{30,144,255}{ if} \textcolor{black}{ and} \textcolor[RGB]{30,144,255}{ only} \textcolor[RGB]{30,144,255}{ if} \textcolor[RGB]{30,144,255}{ \}} \textcolor[RGB]{30,144,255}{ ad} \textcolor[RGB]{30,144,255}{ =} \textcolor[RGB]{30,144,255}{ b}\textcolor[RGB]{30,144,255}{c}\textcolor[RGB]{30,144,255}{\$} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{To} \textcolor{black}{ show} \textcolor[RGB]{30,144,255}{ that} \textcolor{black}{ this} \textcolor[RGB]{30,144,255}{ is} \textcolor{black}{ an} \textcolor{black}{ equivalence} \textcolor{black}{ relation}\textcolor[RGB]{30,144,255}{:} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{1}\textcolor[RGB]{30,144,255}{.} \textcolor[RGB]{30,144,255}{ Ref}\textcolor[RGB]{30,144,255}{lex}\textcolor[RGB]{30,144,255}{ivity}\textcolor[RGB]{30,144,255}{:} \textcolor{black}{ \$\$}\textcolor{black}{(}\textcolor[RGB]{30,144,255}{a}\textcolor[RGB]{30,144,255}{,}\textcolor[RGB]{30,144,255}{b}\textcolor[RGB]{30,144,255}{)} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{sim} \textcolor[RGB]{30,144,255}{ (}\textcolor{black}{a}\textcolor[RGB]{30,144,255}{,}\textcolor[RGB]{30,144,255}{b}\textcolor[RGB]{30,144,255}{)\$\$} \textcolor{black}{ if} \textcolor[RGB]{30,144,255}{ and} \textcolor[RGB]{30,144,255}{ only} \textcolor[RGB]{30,144,255}{ if} \textcolor[RGB]{30,144,255}{ \$\$}\textcolor{black}{ab} \textcolor[RGB]{30,144,255}{ =} \textcolor[RGB]{30,144,255}{ ba}\textcolor[RGB]{30,144,255}{\$\$} \textcolor{black}{ which} \textcolor{black}{ is} \textcolor{black}{ true}\textcolor[RGB]{30,144,255}{.} \textcolor{black}{ Hence} \textcolor[RGB]{30,144,255}{ it} \textcolor{black}{ is} \textcolor{black}{ ref}\textcolor[RGB]{30,144,255}{lex}\textcolor[RGB]{30,144,255}{ive}\textcolor[RGB]{30,144,255}{.} \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor[RGB]{30,144,255}{2}\textcolor[RGB]{30,144,255}{.} \textcolor[RGB]{30,144,255}{ Sym}\textcolor[RGB]{30,144,255}{met}\textcolor[RGB]{30,144,255}{ry}\textcolor[RGB]{30,144,255}{:} \textcolor[RGB]{30,144,255}{ \$\$}\textcolor[RGB]{30,144,255}{(}\textcolor[RGB]{30,144,255}{a}\textcolor[RGB]{30,144,255}{,}\textcolor[RGB]{30,144,255}{b}\textcolor[RGB]{30,144,255}{)} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{sim} \textcolor[RGB]{30,144,255}{ (}\textcolor{black}{c}\textcolor[RGB]{30,144,255}{,}\textcolor[RGB]{30,144,255}{d}\textcolor[RGB]{30,144,255}{)\$\$} \textcolor[RGB]{30,144,255}{ if} \textcolor[RGB]{30,144,255}{ and} \textcolor[RGB]{30,144,255}{ only} \textcolor[RGB]{30,144,255}{ if} \textcolor[RGB]{30,144,255}{ \$\$}\textcolor{black}{ad} \textcolor[RGB]{30,144,255}{ =} \textcolor[RGB]{30,144,255}{ b}\textcolor[RGB]{30,144,255}{c}\textcolor[RGB]{30,144,255}{\$\$} \textcolor{black}{ if} \textcolor[RGB]{30,144,255}{ and} \textcolor[RGB]{30,144,255}{ only} \textcolor[RGB]{30,144,255}{ if} \textcolor{black}{ \$\$}\textcolor{black}{bc} \textcolor[RGB]{30,144,255}{ =} \textcolor[RGB]{30,144,255}{ ad}\textcolor{black}{\$\$} \textcolor{black}{ if} \textcolor[RGB]{30,144,255}{ and} \textcolor[RGB]{30,144,255}{ only} \textcolor[RGB]{30,144,255}{ if} \textcolor{black}{ \$\$}\textcolor[RGB]{30,144,255}{(}\textcolor{black}{c}\textcolor[RGB]{30,144,255}{,}\textcolor[RGB]{30,144,255}{d}\textcolor{black}{)} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{sim} \textcolor[RGB]{30,144,255}{ (}\textcolor[RGB]{30,144,255}{a}\textcolor[RGB]{30,144,255}{,}\textcolor[RGB]{30,144,255}{b}\textcolor[RGB]{30,144,255}{)\$}\textcolor[RGB]{30,144,255}{\$.} \textcolor{black}{ Hence} \textcolor[RGB]{30,144,255}{ it} \textcolor[RGB]{30,144,255}{ is} \textcolor[RGB]{30,144,255}{ symmetric}\textcolor[RGB]{30,144,255}{.} \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor[RGB]{30,144,255}{3}\textcolor[RGB]{30,144,255}{.} \textcolor{black}{ Trans}\textcolor[RGB]{30,144,255}{itivity}\textcolor[RGB]{30,144,255}{:} \textcolor[RGB]{30,144,255}{ \$\$}\textcolor[RGB]{30,144,255}{(}\textcolor[RGB]{30,144,255}{a}\textcolor[RGB]{30,144,255}{,}\textcolor[RGB]{30,144,255}{b}\textcolor[RGB]{30,144,255}{)} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{sim} \textcolor[RGB]{30,144,255}{ (}\textcolor[RGB]{30,144,255}{c}\textcolor[RGB]{30,144,255}{,}\textcolor[RGB]{30,144,255}{d}\textcolor[RGB]{30,144,255}{)\$\$} \textcolor{black}{ and} \textcolor[RGB]{30,144,255}{ \$\$}\textcolor[RGB]{30,144,255}{(}\textcolor{black}{c}\textcolor[RGB]{30,144,255}{,}\textcolor{black}{d}\textcolor[RGB]{30,144,255}{)} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{sim} \textcolor[RGB]{30,144,255}{ (}\textcolor[RGB]{30,144,255}{e}\textcolor[RGB]{30,144,255}{,}\textcolor[RGB]{30,144,255}{f}\textcolor[RGB]{30,144,255}{)\$\$} \textcolor[RGB]{30,144,255}{ if} \textcolor[RGB]{30,144,255}{ and} \textcolor[RGB]{30,144,255}{ only} \textcolor[RGB]{30,144,255}{ if} \textcolor[RGB]{30,144,255}{ \$\$}\textcolor{black}{ad} \textcolor[RGB]{30,144,255}{ =} \textcolor{black}{ b}\textcolor[RGB]{30,144,255}{c}\textcolor[RGB]{30,144,255}{\$\$} \textcolor[RGB]{30,144,255}{ and} \textcolor[RGB]{30,144,255}{ \$\$}\textcolor[RGB]{30,144,255}{cf} \textcolor[RGB]{30,144,255}{ =} \textcolor{black}{ de}\textcolor[RGB]{30,144,255}{\$}\textcolor[RGB]{30,144,255}{\$.} \textcolor{black}{ Mult}\textcolor[RGB]{30,144,255}{ip}\textcolor[RGB]{30,144,255}{lying} \textcolor{black}{ these} \textcolor{black}{ equations} \textcolor[RGB]{30,144,255}{ together}\textcolor{black}{,} \textcolor{black}{ we} \textcolor[RGB]{30,144,255}{ get} \textcolor{black}{ \$\$}\textcolor{black}{ad}\textcolor[RGB]{30,144,255}{cf} \textcolor{black}{ =} \textcolor[RGB]{30,144,255}{ b}\textcolor{black}{c}\textcolor{black}{de}\textcolor[RGB]{30,144,255}{\$}\textcolor[RGB]{30,144,255}{\$.} \textcolor[RGB]{30,144,255}{ We} \textcolor[RGB]{30,144,255}{ can} \textcolor{black}{ cancel} \textcolor{black}{ \$\$}\textcolor[RGB]{30,144,255}{d}\textcolor[RGB]{30,144,255}{\$\$} \textcolor{black}{ and} \textcolor[RGB]{30,144,255}{ \$\$}\textcolor{black}{c}\textcolor[RGB]{30,144,255}{\$\$} \textcolor[RGB]{30,144,255}{ from} \textcolor[RGB]{30,144,255}{ both} \textcolor[RGB]{30,144,255}{ sides} \textcolor{black}{ to} \textcolor{black}{ get} \textcolor[RGB]{30,144,255}{ \$\$}\textcolor[RGB]{30,144,255}{af} \textcolor[RGB]{30,144,255}{ =} \textcolor[RGB]{30,144,255}{ be}\textcolor[RGB]{30,144,255}{\$}\textcolor[RGB]{30,144,255}{\$.} \textcolor{black}{ Hence} \textcolor[RGB]{30,144,255}{ \$\$}\textcolor[RGB]{30,144,255}{(}\textcolor[RGB]{30,144,255}{a}\textcolor[RGB]{30,144,255}{,}\textcolor[RGB]{30,144,255}{b}\textcolor[RGB]{30,144,255}{)} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{sim} \textcolor[RGB]{30,144,255}{ (}\textcolor[RGB]{30,144,255}{e}\textcolor[RGB]{30,144,255}{,}\textcolor[RGB]{30,144,255}{f}\textcolor[RGB]{30,144,255}{)\$}\textcolor[RGB]{30,144,255}{\$.} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{H}\textcolor[RGB]{30,144,255}{ence}\textcolor[RGB]{30,144,255}{,} \textcolor{black}{ we} \textcolor[RGB]{30,144,255}{ have} \textcolor{black}{ successfully} \textcolor{black}{ formed} \textcolor{black}{ the} \textcolor{black}{ set} \textcolor[RGB]{30,144,255}{ of} \textcolor{black}{ rational} \textcolor[RGB]{30,144,255}{ numbers} \textcolor[RGB]{30,144,255}{ when} \textcolor{black}{ we} \textcolor{black}{ factor} \textcolor[RGB]{30,144,255}{ out} \textcolor{black}{ the} \textcolor{black}{ equivalence} \textcolor[RGB]{30,144,255}{ classes}\textcolor{black}{!} \textcolor{black}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{\$\textbackslash }\textcolor[RGB]{30,144,255}{mathbb}\textcolor[RGB]{30,144,255}{\{}\textcolor{black}{Q}\textcolor[RGB]{30,144,255}{\}} \textcolor{black}{ =} \textcolor{black}{ \textbackslash }\textcolor{black}{frac}\textcolor[RGB]{30,144,255}{\{\textbackslash }\textcolor{black}{mathbb}\textcolor[RGB]{30,144,255}{\{}\textcolor[RGB]{30,144,255}{Z}\textcolor[RGB]{30,144,255}{\}} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{times} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{mathbb}\textcolor[RGB]{30,144,255}{\{}\textcolor[RGB]{30,144,255}{Z}\textcolor[RGB]{30,144,255}{\}\textbackslash }\textcolor[RGB]{30,144,255}{back}\textcolor[RGB]{30,144,255}{slash}\textcolor{black}{\textbackslash \{}\textcolor[RGB]{30,144,255}{0}\textcolor[RGB]{30,144,255}{\textbackslash }\textcolor[RGB]{30,144,255}{\}\}\{\textbackslash }\textcolor[RGB]{30,144,255}{sim}\textcolor[RGB]{30,144,255}{\}\$} \textcolor{black}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{Let}\textcolor{black}{’}\textcolor[RGB]{30,144,255}{s} \textcolor{black}{ now} \textcolor{black}{ take} \textcolor[RGB]{30,144,255}{ a} \textcolor{black}{ look} \textcolor[RGB]{30,144,255}{ at} \textcolor[RGB]{30,144,255}{ what} \textcolor{black}{ members} \textcolor[RGB]{30,144,255}{ of} \textcolor{black}{ \$\$\textbackslash }\textcolor[RGB]{30,144,255}{mathbb}\textcolor[RGB]{30,144,255}{\{}\textcolor[RGB]{30,144,255}{Q}\textcolor{black}{\}\$\$} \textcolor[RGB]{30,144,255}{ look} \textcolor[RGB]{30,144,255}{ like}\textcolor{black}{,} \textcolor[RGB]{30,144,255}{ say} \textcolor{black}{ for} \textcolor[RGB]{30,144,255}{ the} \textcolor[RGB]{30,144,255}{ equation} \textcolor[RGB]{30,144,255}{ \$\$}\textcolor[RGB]{30,144,255}{2}\textcolor[RGB]{30,144,255}{x} \textcolor[RGB]{30,144,255}{ =} \textcolor[RGB]{30,144,255}{ }\textcolor[RGB]{30,144,255}{3}\textcolor[RGB]{30,144,255}{\$}\textcolor[RGB]{30,144,255}{\$.} \textcolor[RGB]{30,144,255}{ This} \textcolor[RGB]{30,144,255}{ equation} \textcolor[RGB]{30,144,255}{ is} \textcolor{black}{ represented} \textcolor{black}{ by} \textcolor[RGB]{30,144,255}{ the} \textcolor[RGB]{30,144,255}{ ordered} \textcolor[RGB]{30,144,255}{ pair}
\\ \hline
\textcolor[RGB]{30,144,255}{If} \textcolor{black}{ the} \textcolor[RGB]{30,144,255}{ light} \textcolor{black}{ moves} \textcolor{black}{ in} \textcolor[RGB]{30,144,255}{ a} \textcolor[RGB]{30,144,255}{ purely} \textcolor{black}{ radial} \textcolor[RGB]{30,144,255}{ direction}\textcolor[RGB]{30,144,255}{,} \textcolor[RGB]{30,144,255}{ we} \textcolor[RGB]{30,144,255}{ can} \textcolor[RGB]{30,144,255}{ describe} \textcolor{black}{ its} \textcolor{black}{ path} \textcolor{black}{ by} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ coordinate} \textcolor{black}{ functions} \textcolor{black}{ \$\$}\textcolor[RGB]{30,144,255}{t}\textcolor{black}{(\textbackslash }\textcolor{black}{lambda}\textcolor{black}{)\$\$} \textcolor[RGB]{30,144,255}{ and} \textcolor[RGB]{30,144,255}{ \$\$}\textcolor{black}{r}\textcolor[RGB]{30,144,255}{(\textbackslash }\textcolor[RGB]{30,144,255}{lambda}\textcolor{black}{)\$}\textcolor{black}{\$.} \textcolor[RGB]{30,144,255}{ The} \textcolor{black}{ equation} \textcolor[RGB]{30,144,255}{ of} \textcolor{black}{ motion} \textcolor{black}{ \$\$}\textcolor{black}{ds}\textcolor{black}{\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor{black}{ =}\textcolor[RGB]{30,144,255}{0}\textcolor[RGB]{30,144,255}{\$\$} \textcolor{black}{ then} \textcolor{black}{ takes} \textcolor[RGB]{30,144,255}{ the} \textcolor[RGB]{30,144,255}{ form} \textcolor[RGB]{30,144,255}{ \$\$}\textcolor{black}{g}\textcolor[RGB]{30,144,255}{\_\{}\textcolor{black}{tt}\textcolor{black}{\}} \textcolor{black}{ \textbackslash }\textcolor{black}{left}\textcolor{black}{(\textbackslash }\textcolor{black}{frac}\textcolor[RGB]{30,144,255}{\{}\textcolor{black}{dt}\textcolor[RGB]{30,144,255}{\}\{}\textcolor[RGB]{30,144,255}{d}\textcolor[RGB]{30,144,255}{\textbackslash }\textcolor[RGB]{30,144,255}{lambda}\textcolor[RGB]{30,144,255}{\}\textbackslash }\textcolor[RGB]{30,144,255}{right}\textcolor[RGB]{30,144,255}{)\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor{black}{ +} \textcolor{black}{ g}\textcolor[RGB]{30,144,255}{\_\{}\textcolor[RGB]{30,144,255}{rr}\textcolor[RGB]{30,144,255}{\}} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{left}\textcolor[RGB]{30,144,255}{(\textbackslash }\textcolor[RGB]{30,144,255}{frac}\textcolor[RGB]{30,144,255}{\{}\textcolor[RGB]{30,144,255}{dr}\textcolor[RGB]{30,144,255}{\}\{}\textcolor[RGB]{30,144,255}{d}\textcolor[RGB]{30,144,255}{\textbackslash }\textcolor[RGB]{30,144,255}{lambda}\textcolor[RGB]{30,144,255}{\}\textbackslash }\textcolor[RGB]{30,144,255}{right}\textcolor[RGB]{30,144,255}{)\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ =} \textcolor[RGB]{30,144,255}{ }\textcolor[RGB]{30,144,255}{0}\textcolor{black}{,}\textcolor[RGB]{30,144,255}{\$\$} \textcolor{black}{ which} \textcolor{black}{ we} \textcolor[RGB]{30,144,255}{ can} \textcolor{black}{ rewrite} \textcolor[RGB]{30,144,255}{ as} \textcolor[RGB]{30,144,255}{ \$\$\textbackslash }\textcolor[RGB]{30,144,255}{left}\textcolor[RGB]{30,144,255}{(\textbackslash }\textcolor[RGB]{30,144,255}{frac}\textcolor[RGB]{30,144,255}{\{}\textcolor{black}{dt}\textcolor[RGB]{30,144,255}{\}\{}\textcolor{black}{dr}\textcolor[RGB]{30,144,255}{\}\textbackslash }\textcolor[RGB]{30,144,255}{right}\textcolor[RGB]{30,144,255}{)\^{}}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ =} \textcolor{black}{ -\textbackslash }\textcolor{black}{frac}\textcolor[RGB]{30,144,255}{\{}\textcolor{black}{g}\textcolor[RGB]{30,144,255}{\_\{}\textcolor[RGB]{30,144,255}{rr}\textcolor[RGB]{30,144,255}{\}\}\{}\textcolor[RGB]{30,144,255}{g}\textcolor[RGB]{30,144,255}{\_\{}\textcolor[RGB]{30,144,255}{tt}\textcolor[RGB]{30,144,255}{\}\}}\textcolor{black}{.\$\$} \textcolor{black}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{The} \textcolor[RGB]{30,144,255}{ length} \textcolor[RGB]{30,144,255}{ of} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ rod} \textcolor{black}{ is} \textcolor[RGB]{30,144,255}{ then} \textcolor{black}{ \$\$}\textcolor[RGB]{30,144,255}{L} \textcolor[RGB]{30,144,255}{ =} \textcolor{black}{ c} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{int}\textcolor[RGB]{30,144,255}{\_\{}\textcolor[RGB]{30,144,255}{r}\textcolor[RGB]{30,144,255}{\_}\textcolor{black}{1}\textcolor[RGB]{30,144,255}{\}\^{}\{}\textcolor[RGB]{30,144,255}{r}\textcolor[RGB]{30,144,255}{\_}\textcolor[RGB]{30,144,255}{2}\textcolor[RGB]{30,144,255}{\}} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{frac}\textcolor[RGB]{30,144,255}{\{}\textcolor{black}{dt}\textcolor[RGB]{30,144,255}{\}\{}\textcolor[RGB]{30,144,255}{dr}\textcolor[RGB]{30,144,255}{\}} \textcolor{black}{ \textbackslash }\textcolor[RGB]{30,144,255}{text}\textcolor[RGB]{30,144,255}{\{} \textcolor{black}{ d}\textcolor{black}{\}}\textcolor[RGB]{30,144,255}{r} \textcolor[RGB]{30,144,255}{ =} \textcolor[RGB]{30,144,255}{ c} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor{black}{int}\textcolor[RGB]{30,144,255}{\_\{}\textcolor[RGB]{30,144,255}{r}\textcolor[RGB]{30,144,255}{\_}\textcolor[RGB]{30,144,255}{1}\textcolor[RGB]{30,144,255}{\}\^{}\{}\textcolor[RGB]{30,144,255}{r}\textcolor[RGB]{30,144,255}{\_}\textcolor[RGB]{30,144,255}{2}\textcolor[RGB]{30,144,255}{\}} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{sqrt}\textcolor{black}{\{}\textcolor{black}{-\textbackslash }\textcolor[RGB]{30,144,255}{frac}\textcolor[RGB]{30,144,255}{\{}\textcolor[RGB]{30,144,255}{g}\textcolor[RGB]{30,144,255}{\_\{}\textcolor[RGB]{30,144,255}{rr}\textcolor[RGB]{30,144,255}{\}\}\{}\textcolor[RGB]{30,144,255}{g}\textcolor[RGB]{30,144,255}{\_\{}\textcolor[RGB]{30,144,255}{tt}\textcolor[RGB]{30,144,255}{\}\}\}} \textcolor[RGB]{30,144,255}{ \textbackslash }\textcolor[RGB]{30,144,255}{text}\textcolor[RGB]{30,144,255}{\{} \textcolor[RGB]{30,144,255}{ d}\textcolor[RGB]{30,144,255}{\}}\textcolor[RGB]{30,144,255}{r}\textcolor{black}{,}\textcolor[RGB]{30,144,255}{\$\$} \textcolor[RGB]{30,144,255}{ where} \textcolor[RGB]{30,144,255}{ I} \textcolor{black}{ have} \textcolor{black}{ taken} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ positive} \textcolor{black}{ square} \textcolor[RGB]{30,144,255}{ root} \textcolor[RGB]{30,144,255}{ because} \textcolor{black}{ \$\$}\textcolor[RGB]{30,144,255}{r}\textcolor{black}{\_}\textcolor[RGB]{30,144,255}{2} \textcolor[RGB]{30,144,255}{ >} \textcolor[RGB]{30,144,255}{ r}\textcolor[RGB]{30,144,255}{\_}\textcolor[RGB]{30,144,255}{1}\textcolor[RGB]{30,144,255}{\$}\textcolor[RGB]{30,144,255}{\$.} \textcolor{black}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor{black}{Not}\textcolor[RGB]{30,144,255}{ice} \textcolor[RGB]{30,144,255}{ that} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ length} \textcolor{black}{ is} \textcolor{black}{ independent} \textcolor[RGB]{30,144,255}{ of} \textcolor{black}{ the} \textcolor{black}{ signature} \textcolor[RGB]{30,144,255}{ of} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ metric}\textcolor{black}{,} \textcolor[RGB]{30,144,255}{ so} \textcolor[RGB]{30,144,255}{ whether} \textcolor{black}{ you} \textcolor{black}{ work} \textcolor{black}{ with} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ (-}\textcolor{black}{++}\textcolor{black}{+)} \textcolor[RGB]{30,144,255}{ or} \textcolor{black}{ (+}\textcolor[RGB]{30,144,255}{---}\textcolor[RGB]{30,144,255}{)} \textcolor{black}{ metric} \textcolor{black}{ is} \textcolor{black}{ purely} \textcolor[RGB]{30,144,255}{ conventional} \textcolor{black}{ and} \textcolor{black}{ will} \textcolor[RGB]{30,144,255}{ not} \textcolor[RGB]{30,144,255}{ change} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ physics}\textcolor{black}{.} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor[RGB]{30,144,255}{For} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ Schwar}\textcolor[RGB]{30,144,255}{z}\textcolor[RGB]{30,144,255}{sch}\textcolor[RGB]{30,144,255}{ild} \textcolor{black}{ metric}\textcolor[RGB]{30,144,255}{,} \textcolor[RGB]{30,144,255}{ we} \textcolor[RGB]{30,144,255}{ obtain} \textcolor{black}{ explicitly} \textcolor{black}{ \$\$}\textcolor{black}{L} \textcolor[RGB]{30,144,255}{ =} \textcolor{black}{ r}\textcolor{black}{\_}\textcolor{black}{2} \textcolor{black}{ -} \textcolor[RGB]{30,144,255}{ r}\textcolor[RGB]{30,144,255}{\_}\textcolor[RGB]{30,144,255}{1} \textcolor{black}{ +} \textcolor{black}{ r}\textcolor[RGB]{30,144,255}{\_}\textcolor{black}{s} \textcolor{black}{ \textbackslash }\textcolor{black}{ln}\textcolor{black}{\textbackslash }\textcolor[RGB]{30,144,255}{left}\textcolor[RGB]{30,144,255}{(\textbackslash }\textcolor[RGB]{30,144,255}{frac}\textcolor[RGB]{30,144,255}{\{}\textcolor[RGB]{30,144,255}{r}\textcolor[RGB]{30,144,255}{\_}\textcolor[RGB]{30,144,255}{2} \textcolor{black}{ -} \textcolor[RGB]{30,144,255}{ r}\textcolor[RGB]{30,144,255}{\_}\textcolor{black}{s}\textcolor[RGB]{30,144,255}{\}\{}\textcolor[RGB]{30,144,255}{r}\textcolor[RGB]{30,144,255}{\_}\textcolor[RGB]{30,144,255}{1} \textcolor{black}{ -} \textcolor[RGB]{30,144,255}{ r}\textcolor[RGB]{30,144,255}{\_}\textcolor[RGB]{30,144,255}{s}\textcolor[RGB]{30,144,255}{\}\textbackslash }\textcolor[RGB]{30,144,255}{right}\textcolor{black}{)} \textcolor[RGB]{30,144,255}{ >} \textcolor{black}{ r}\textcolor[RGB]{30,144,255}{\_}\textcolor{black}{2} \textcolor[RGB]{30,144,255}{ -} \textcolor[RGB]{30,144,255}{ r}\textcolor[RGB]{30,144,255}{\_}\textcolor[RGB]{30,144,255}{1}\textcolor[RGB]{30,144,255}{.\$\$} \textcolor[RGB]{30,144,255}{ \textbackslash n } \textcolor[RGB]{30,144,255}{ \textbackslash n }\textcolor[RGB]{30,144,255}{Now} \textcolor{black}{ what} \textcolor{black}{ happens} \textcolor{black}{ if} \textcolor{black}{ you} \textcolor{black}{ mag}\textcolor[RGB]{30,144,255}{ically}\textcolor{black}{,} \textcolor[RGB]{30,144,255}{ instant}\textcolor[RGB]{30,144,255}{ane}\textcolor[RGB]{30,144,255}{ously} \textcolor[RGB]{30,144,255}{ increase} \textcolor[RGB]{30,144,255}{ the} \textcolor[RGB]{30,144,255}{ mass} \textcolor{black}{ of} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ black} \textcolor[RGB]{30,144,255}{ hole}\textcolor[RGB]{30,144,255}{?} \textcolor{black}{ I} \textcolor{black}{ think} \textcolor[RGB]{30,144,255}{ the} \textcolor[RGB]{30,144,255}{ length} \textcolor{black}{ \$\$}\textcolor[RGB]{30,144,255}{L}\textcolor[RGB]{30,144,255}{\$\$} \textcolor[RGB]{30,144,255}{ of} \textcolor[RGB]{30,144,255}{ the} \textcolor[RGB]{30,144,255}{ rod} \textcolor[RGB]{30,144,255}{ stays} \textcolor[RGB]{30,144,255}{ the} \textcolor[RGB]{30,144,255}{ same} \textcolor[RGB]{30,144,255}{ (}\textcolor{black}{I}\textcolor[RGB]{30,144,255}{'}\textcolor[RGB]{30,144,255}{m} \textcolor[RGB]{30,144,255}{ here} \textcolor{black}{ assuming} \textcolor[RGB]{30,144,255}{ that} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ rod} \textcolor{black}{ is} \textcolor{black}{ infinitely} \textcolor{black}{ st}\textcolor[RGB]{30,144,255}{iff}\textcolor[RGB]{30,144,255}{),} \textcolor[RGB]{30,144,255}{ but} \textcolor{black}{ that} \textcolor{black}{ it} \textcolor{black}{ would} \textcolor{black}{ now} \textcolor[RGB]{30,144,255}{ ''}\textcolor{black}{app}\textcolor[RGB]{30,144,255}{ear} \textcolor{black}{ shorter}\textcolor[RGB]{30,144,255}{''} \textcolor{black}{ to} \textcolor[RGB]{30,144,255}{ the} \textcolor{black}{ distant} \textcolor[RGB]{30,144,255}{ observer} \textcolor{black}{ -} \textcolor{black}{ i}\textcolor[RGB]{30,144,255}{.}\textcolor[RGB]{30,144,255}{e}\textcolor{black}{.} \textcolor{black}{ it} \textcolor[RGB]{30,144,255}{ would} \textcolor[RGB]{30,144,255}{ no} \textcolor[RGB]{30,144,255}{ longer} \textcolor[RGB]{30,144,255}{ occup}\textcolor[RGB]{30,144,255}{y} \textcolor[RGB]{30,144,255}{ the} \textcolor[RGB]{30,144,255}{ entire} \textcolor[RGB]{30,144,255}{ space} \textcolor{black}{ between} \textcolor{black}{ \$\$}\textcolor[RGB]{30,144,255}{r}\textcolor[RGB]{30,144,255}{\_}\textcolor[RGB]{30,144,255}{1}\textcolor[RGB]{30,144,255}{\$\$} \textcolor[RGB]{30,144,255}{ and} \textcolor[RGB]{30,144,255}{ \$\$}\textcolor[RGB]{30,144,255}{r}\textcolor[RGB]{30,144,255}{\_}\textcolor[RGB]{30,144,255}{2}\textcolor[RGB]{30,144,255}{\$}\textcolor[RGB]{30,144,255}{\$.}
\\ \bottomrule 
\end{tabular}
}
\caption{\textbf{Specific examples of selecting tokens during the ToT training process of the \model{}.} The tokens marked in \textcolor[RGB]{30,144,255}{blue} represent the actual tokens trained during the ToT training process, while the remaining black tokens are not trained during the ToT training process.}
\label{tab:example_select_tokens}
\end{table*}

==> table/training_danamic_samples.tex <==
\begin{table*}[t]
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}p{16cm}@{}}
\toprule
\multicolumn{1}{c}{\texttt{After Training 20\% Checkpoint}} \\
\midrule
\textcolor{black}{ All}\textcolor{black}{-}\textcolor[RGB]{34,139,34}{pay} \textcolor[RGB]{34,139,34}{ au}\textcolor[RGB]{34,139,34}{ction} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{The} \textcolor{black}{ all}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{pay} \textcolor[RGB]{34,139,34}{ au}\textcolor[RGB]{34,139,34}{ction} \textcolor[RGB]{34,139,34}{ is} \textcolor{black}{ like} \textcolor{black}{ lo}\textcolor{black}{bb}\textcolor[RGB]{34,139,34}{ying}\textcolor{black}{.} \textcolor[RGB]{34,139,34}{ Each} \textcolor{black}{ player} \textcolor[RGB]{34,139,34}{ makes} \textcolor[RGB]{34,139,34}{ a} \textcolor[RGB]{34,139,34}{ bid}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ and} \textcolor{black}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{•} \textcolor[RGB]{34,139,34}{ \$\{}\textcolor{black}{Q} \textcolor{black}{ =} \textcolor{black}{ Q}\textcolor{black}{\_\{\textbackslash }\textcolor[RGB]{34,139,34}{text}\textcolor[RGB]{34,139,34}{\{}\textcolor{black}{high}\textcolor[RGB]{34,139,34}{est}\textcolor[RGB]{34,139,34}{\}\}}\textcolor[RGB]{34,139,34}{\}\$,} \textcolor[RGB]{34,139,34}{ and} \textcolor{black}{ \textbackslash n }\textcolor{black}{•} \textcolor{black}{ \$\{}\textcolor[RGB]{34,139,34}{P}\textcolor{black}{\}\$} \textcolor[RGB]{34,139,34}{ is} \textcolor{black}{ defined} \textcolor{black}{ by} \textcolor{black}{ requiring} \textcolor{black}{ everyone} \textcolor[RGB]{34,139,34}{ to} \textcolor{black}{ pay} \textcolor[RGB]{34,139,34}{ their} \textcolor{black}{ bid}\textcolor[RGB]{34,139,34}{,} \textcolor{black}{ regardless} \textcolor[RGB]{34,139,34}{ of} \textcolor[RGB]{34,139,34}{ whether} \textcolor[RGB]{34,139,34}{ they} \textcolor[RGB]{34,139,34}{ win} \textcolor{black}{ the} \textcolor{black}{ power} \textcolor{black}{ dr}\textcolor[RGB]{34,139,34}{ill} \textcolor[RGB]{34,139,34}{ or} \textcolor[RGB]{34,139,34}{ not}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{This} \textcolor{black}{ is} \textcolor{black}{ clearly} \textcolor{black}{ not} \textcolor[RGB]{34,139,34}{ in}\textcolor[RGB]{34,139,34}{cent}\textcolor[RGB]{34,139,34}{ive} \textcolor{black}{ compatible}\textcolor[RGB]{34,139,34}{.} \textcolor{black}{ In} \textcolor[RGB]{34,139,34}{ fact}\textcolor[RGB]{34,139,34}{,} \textcolor{black}{ the} \textcolor{black}{ Nash} \textcolor{black}{ equilibrium} \textcolor{black}{ is} \textcolor{black}{ as} \textcolor[RGB]{34,139,34}{ follows}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Pro}\textcolor[RGB]{34,139,34}{position} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{4} \textcolor[RGB]{34,139,34}{ (}\textcolor{black}{N}\textcolor[RGB]{34,139,34}{ash} \textcolor{black}{ equilib}\textcolor{black}{ir}\textcolor[RGB]{34,139,34}{um} \textcolor{black}{ of} \textcolor[RGB]{34,139,34}{ the} \textcolor{black}{ all}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{pay} \textcolor[RGB]{34,139,34}{ au}\textcolor[RGB]{34,139,34}{ction}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{Cons}\textcolor[RGB]{34,139,34}{ider} \textcolor[RGB]{34,139,34}{ a} \textcolor{black}{ first}\textcolor[RGB]{34,139,34}{-}\textcolor{black}{price} \textcolor{black}{ au}\textcolor[RGB]{34,139,34}{ction} \textcolor[RGB]{34,139,34}{ where} \textcolor[RGB]{34,139,34}{ Anna} \textcolor[RGB]{34,139,34}{ and} \textcolor{black}{ El}\textcolor[RGB]{34,139,34}{sa} \textcolor{black}{ have} \textcolor{black}{ values} \textcolor{black}{ uniformly} \textcolor[RGB]{34,139,34}{ distributed} \textcolor{black}{ in} \textcolor{black}{ \$\{}\textcolor[RGB]{34,139,34}{{[}}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1}\textcolor{black}{0}\textcolor{black}{0}\textcolor{black}{0}\textcolor[RGB]{34,139,34}{{]}}\textcolor[RGB]{34,139,34}{\}\$.} \textcolor[RGB]{34,139,34}{ Suppose} \textcolor[RGB]{34,139,34}{ both} \textcolor[RGB]{34,139,34}{ Anna} \textcolor[RGB]{34,139,34}{ and} \textcolor[RGB]{34,139,34}{ El}\textcolor[RGB]{34,139,34}{sa} \textcolor[RGB]{34,139,34}{ bid} \textcolor{black}{ \$\{\textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{2}\textcolor{black}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{cdot} \textcolor{black}{ }\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor{black}{(}\textcolor{black}{x}\textcolor{black}{/}\textcolor{black}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{)\^{}}\textcolor[RGB]{34,139,34}{2}\textcolor{black}{\}\$} \textcolor[RGB]{34,139,34}{ if} \textcolor[RGB]{34,139,34}{ they} \textcolor{black}{ have} \textcolor{black}{ value} \textcolor{black}{ \$\{}\textcolor[RGB]{34,139,34}{x}\textcolor{black}{\}\$.} \textcolor{black}{ Then} \textcolor{black}{ this} \textcolor[RGB]{34,139,34}{ is} \textcolor{black}{ a} \textcolor{black}{ Nash} \textcolor[RGB]{34,139,34}{ equilibrium}\textcolor{black}{.} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Proof}\textcolor[RGB]{34,139,34}{:} \textcolor{black}{ Om}\textcolor{black}{itted}\textcolor{black}{,} \textcolor{black}{ but} \textcolor{black}{ a} \textcolor{black}{ fun} \textcolor{black}{ and} \textcolor[RGB]{34,139,34}{ not}\textcolor[RGB]{34,139,34}{-}\textcolor{black}{hard} \textcolor{black}{ exercise} \textcolor{black}{ if} \textcolor[RGB]{34,139,34}{ you} \textcolor[RGB]{34,139,34}{ like} \textcolor{black}{ integr}\textcolor{black}{als}\textcolor{black}{.} \textcolor[RGB]{34,139,34}{ It} \textcolor[RGB]{34,139,34}{ will} \textcolor{black}{ follow} \textcolor[RGB]{34,139,34}{ from} \textcolor{black}{ a} \textcolor{black}{ later} \textcolor{black}{ result}\textcolor{black}{.} \textcolor{black}{ \$\textbackslash }\textcolor[RGB]{34,139,34}{Box}\textcolor[RGB]{34,139,34}{\$} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{Just} \textcolor[RGB]{34,139,34}{ for} \textcolor[RGB]{34,139,34}{ interest}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ let}\textcolor[RGB]{34,139,34}{’}\textcolor[RGB]{34,139,34}{s} \textcolor[RGB]{34,139,34}{ compute} \textcolor[RGB]{34,139,34}{ how} \textcolor[RGB]{34,139,34}{ much} \textcolor[RGB]{34,139,34}{ money} \textcolor{black}{ Hans} \textcolor{black}{ is} \textcolor[RGB]{34,139,34}{ going} \textcolor[RGB]{34,139,34}{ to} \textcolor[RGB]{34,139,34}{ make} \textcolor{black}{ off} \textcolor[RGB]{34,139,34}{ the} \textcolor[RGB]{34,139,34}{ dr}\textcolor[RGB]{34,139,34}{ill} \textcolor[RGB]{34,139,34}{ in} \textcolor[RGB]{34,139,34}{ this} \textcolor[RGB]{34,139,34}{ equilibrium}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{34,139,34}{ This} \textcolor[RGB]{34,139,34}{ time} \textcolor[RGB]{34,139,34}{ he} \textcolor{black}{ amount} \textcolor{black}{ paid} \textcolor[RGB]{34,139,34}{ to} \textcolor[RGB]{34,139,34}{ him} \textcolor[RGB]{34,139,34}{ is} \textcolor[RGB]{34,139,34}{ equal} \textcolor[RGB]{34,139,34}{ to} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{\$\textbackslash }\textcolor[RGB]{34,139,34}{displaystyle} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{mathbf} \textcolor[RGB]{34,139,34}{ E}\textcolor[RGB]{34,139,34}{\_\{}\textcolor[RGB]{34,139,34}{a}\textcolor[RGB]{34,139,34}{,}\textcolor{black}{e}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{left}\textcolor[RGB]{34,139,34}{(} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor{black}{a}\textcolor[RGB]{34,139,34}{\^{}}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{\}\{}\textcolor{black}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}} \textcolor{black}{ +} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{b}\textcolor[RGB]{34,139,34}{\^{}}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{right}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{34,139,34}{ =} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{int}\textcolor[RGB]{34,139,34}{\_\{}\textcolor{black}{0}\textcolor[RGB]{34,139,34}{\}\^{}\{}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{x}\textcolor{black}{\^{}}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{0}\textcolor{black}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}} \textcolor{black}{ \textbackslash ;} \textcolor{black}{ dx} \textcolor[RGB]{34,139,34}{ =} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor{black}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{3}\textcolor{black}{\}.}\textcolor[RGB]{34,139,34}{\$} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{Sur}\textcolor{black}{prise} \textcolor{black}{ —} \textcolor{black}{ same} \textcolor[RGB]{34,139,34}{ value} \textcolor{black}{ again}\textcolor{black}{!} \textcolor{black}{ This} \textcolor{black}{ is} \textcolor[RGB]{34,139,34}{ a} \textcolor{black}{ very} \textcolor{black}{ special} \textcolor{black}{ case} \textcolor[RGB]{34,139,34}{ of} \textcolor[RGB]{34,139,34}{ the} \textcolor{black}{ Re}\textcolor[RGB]{34,139,34}{venue} \textcolor[RGB]{34,139,34}{ Equ}\textcolor{black}{ival}\textcolor[RGB]{34,139,34}{ence} \textcolor[RGB]{34,139,34}{ Theorem} \textcolor{black}{ later}\textcolor{black}{.}
\\ \midrule
\multicolumn{1}{c}{\texttt{After Training 40\% Checkpoint}} \\
\midrule
\textcolor{black}{ All}\textcolor{black}{-}\textcolor[RGB]{34,139,34}{pay} \textcolor[RGB]{34,139,34}{ au}\textcolor[RGB]{34,139,34}{ction} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{The} \textcolor{black}{ all}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{pay} \textcolor[RGB]{34,139,34}{ au}\textcolor[RGB]{34,139,34}{ction} \textcolor[RGB]{34,139,34}{ is} \textcolor{black}{ like} \textcolor{black}{ lo}\textcolor{black}{bb}\textcolor[RGB]{34,139,34}{ying}\textcolor{black}{.} \textcolor{black}{ Each} \textcolor{black}{ player} \textcolor[RGB]{34,139,34}{ makes} \textcolor[RGB]{34,139,34}{ a} \textcolor[RGB]{34,139,34}{ bid}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ and} \textcolor{black}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{•} \textcolor[RGB]{34,139,34}{ \$\{}\textcolor{black}{Q} \textcolor{black}{ =} \textcolor{black}{ Q}\textcolor{black}{\_\{\textbackslash }\textcolor[RGB]{34,139,34}{text}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{high}\textcolor[RGB]{34,139,34}{est}\textcolor[RGB]{34,139,34}{\}\}}\textcolor[RGB]{34,139,34}{\}\$,} \textcolor[RGB]{34,139,34}{ and} \textcolor{black}{ \textbackslash n }\textcolor{black}{•} \textcolor{black}{ \$\{}\textcolor{black}{P}\textcolor{black}{\}\$} \textcolor[RGB]{34,139,34}{ is} \textcolor{black}{ defined} \textcolor{black}{ by} \textcolor{black}{ requiring} \textcolor{black}{ everyone} \textcolor[RGB]{34,139,34}{ to} \textcolor{black}{ pay} \textcolor{black}{ their} \textcolor{black}{ bid}\textcolor[RGB]{34,139,34}{,} \textcolor{black}{ regardless} \textcolor[RGB]{34,139,34}{ of} \textcolor{black}{ whether} \textcolor[RGB]{34,139,34}{ they} \textcolor[RGB]{34,139,34}{ win} \textcolor{black}{ the} \textcolor{black}{ power} \textcolor[RGB]{34,139,34}{ dr}\textcolor[RGB]{34,139,34}{ill} \textcolor[RGB]{34,139,34}{ or} \textcolor[RGB]{34,139,34}{ not}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{This} \textcolor{black}{ is} \textcolor{black}{ clearly} \textcolor[RGB]{34,139,34}{ not} \textcolor[RGB]{34,139,34}{ in}\textcolor[RGB]{34,139,34}{cent}\textcolor[RGB]{34,139,34}{ive} \textcolor{black}{ compatible}\textcolor[RGB]{34,139,34}{.} \textcolor{black}{ In} \textcolor[RGB]{34,139,34}{ fact}\textcolor[RGB]{34,139,34}{,} \textcolor{black}{ the} \textcolor{black}{ Nash} \textcolor[RGB]{34,139,34}{ equilibrium} \textcolor{black}{ is} \textcolor{black}{ as} \textcolor[RGB]{34,139,34}{ follows}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Pro}\textcolor[RGB]{34,139,34}{position} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{4} \textcolor[RGB]{34,139,34}{ (}\textcolor{black}{N}\textcolor[RGB]{34,139,34}{ash} \textcolor{black}{ equilib}\textcolor{black}{ir}\textcolor{black}{um} \textcolor{black}{ of} \textcolor[RGB]{34,139,34}{ the} \textcolor{black}{ all}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{pay} \textcolor[RGB]{34,139,34}{ au}\textcolor[RGB]{34,139,34}{ction}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Cons}\textcolor[RGB]{34,139,34}{ider} \textcolor[RGB]{34,139,34}{ a} \textcolor{black}{ first}\textcolor[RGB]{34,139,34}{-}\textcolor{black}{price} \textcolor{black}{ au}\textcolor[RGB]{34,139,34}{ction} \textcolor[RGB]{34,139,34}{ where} \textcolor[RGB]{34,139,34}{ Anna} \textcolor[RGB]{34,139,34}{ and} \textcolor{black}{ El}\textcolor{black}{sa} \textcolor{black}{ have} \textcolor{black}{ values} \textcolor{black}{ uniformly} \textcolor{black}{ distributed} \textcolor{black}{ in} \textcolor{black}{ \$\{}\textcolor[RGB]{34,139,34}{{[}}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1}\textcolor{black}{0}\textcolor{black}{0}\textcolor{black}{0}\textcolor[RGB]{34,139,34}{{]}}\textcolor[RGB]{34,139,34}{\}\$.} \textcolor[RGB]{34,139,34}{ Suppose} \textcolor[RGB]{34,139,34}{ both} \textcolor[RGB]{34,139,34}{ Anna} \textcolor[RGB]{34,139,34}{ and} \textcolor[RGB]{34,139,34}{ El}\textcolor[RGB]{34,139,34}{sa} \textcolor[RGB]{34,139,34}{ bid} \textcolor{black}{ \$\{\textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{2}\textcolor{black}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{cdot} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor{black}{(}\textcolor[RGB]{34,139,34}{x}\textcolor{black}{/}\textcolor{black}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{)\^{}}\textcolor[RGB]{34,139,34}{2}\textcolor{black}{\}\$} \textcolor[RGB]{34,139,34}{ if} \textcolor[RGB]{34,139,34}{ they} \textcolor{black}{ have} \textcolor{black}{ value} \textcolor{black}{ \$\{}\textcolor[RGB]{34,139,34}{x}\textcolor[RGB]{34,139,34}{\}\$.} \textcolor{black}{ Then} \textcolor{black}{ this} \textcolor[RGB]{34,139,34}{ is} \textcolor{black}{ a} \textcolor{black}{ Nash} \textcolor[RGB]{34,139,34}{ equilibrium}\textcolor{black}{.} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Proof}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ Om}\textcolor{black}{itted}\textcolor{black}{,} \textcolor{black}{ but} \textcolor{black}{ a} \textcolor{black}{ fun} \textcolor{black}{ and} \textcolor{black}{ not}\textcolor[RGB]{34,139,34}{-}\textcolor{black}{hard} \textcolor[RGB]{34,139,34}{ exercise} \textcolor{black}{ if} \textcolor[RGB]{34,139,34}{ you} \textcolor{black}{ like} \textcolor{black}{ integr}\textcolor{black}{als}\textcolor{black}{.} \textcolor[RGB]{34,139,34}{ It} \textcolor[RGB]{34,139,34}{ will} \textcolor{black}{ follow} \textcolor{black}{ from} \textcolor{black}{ a} \textcolor{black}{ later} \textcolor{black}{ result}\textcolor{black}{.} \textcolor{black}{ \$\textbackslash }\textcolor[RGB]{34,139,34}{Box}\textcolor[RGB]{34,139,34}{\$} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Just} \textcolor[RGB]{34,139,34}{ for} \textcolor[RGB]{34,139,34}{ interest}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ let}\textcolor[RGB]{34,139,34}{’}\textcolor[RGB]{34,139,34}{s} \textcolor[RGB]{34,139,34}{ compute} \textcolor[RGB]{34,139,34}{ how} \textcolor[RGB]{34,139,34}{ much} \textcolor[RGB]{34,139,34}{ money} \textcolor{black}{ Hans} \textcolor{black}{ is} \textcolor[RGB]{34,139,34}{ going} \textcolor[RGB]{34,139,34}{ to} \textcolor[RGB]{34,139,34}{ make} \textcolor{black}{ off} \textcolor[RGB]{34,139,34}{ the} \textcolor[RGB]{34,139,34}{ dr}\textcolor[RGB]{34,139,34}{ill} \textcolor[RGB]{34,139,34}{ in} \textcolor[RGB]{34,139,34}{ this} \textcolor[RGB]{34,139,34}{ equilibrium}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{34,139,34}{ This} \textcolor[RGB]{34,139,34}{ time} \textcolor[RGB]{34,139,34}{ he} \textcolor[RGB]{34,139,34}{ amount} \textcolor{black}{ paid} \textcolor[RGB]{34,139,34}{ to} \textcolor[RGB]{34,139,34}{ him} \textcolor[RGB]{34,139,34}{ is} \textcolor[RGB]{34,139,34}{ equal} \textcolor[RGB]{34,139,34}{ to} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{\$\textbackslash }\textcolor[RGB]{34,139,34}{displaystyle} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{mathbf} \textcolor[RGB]{34,139,34}{ E}\textcolor[RGB]{34,139,34}{\_\{}\textcolor[RGB]{34,139,34}{a}\textcolor[RGB]{34,139,34}{,}\textcolor{black}{e}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{left}\textcolor[RGB]{34,139,34}{(} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor{black}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor{black}{a}\textcolor{black}{\^{}}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{\}\{}\textcolor{black}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ +} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{b}\textcolor[RGB]{34,139,34}{\^{}}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{right}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{34,139,34}{ =} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{int}\textcolor[RGB]{34,139,34}{\_\{}\textcolor{black}{0}\textcolor[RGB]{34,139,34}{\}\^{}\{}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}} \textcolor{black}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor{black}{x}\textcolor{black}{\^{}}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{0}\textcolor{black}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}} \textcolor{black}{ \textbackslash ;} \textcolor{black}{ dx} \textcolor[RGB]{34,139,34}{ =} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor{black}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{3}\textcolor[RGB]{34,139,34}{\}.}\textcolor[RGB]{34,139,34}{\$} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{Sur}\textcolor{black}{prise} \textcolor{black}{ —} \textcolor{black}{ same} \textcolor[RGB]{34,139,34}{ value} \textcolor{black}{ again}\textcolor[RGB]{34,139,34}{!} \textcolor{black}{ This} \textcolor{black}{ is} \textcolor[RGB]{34,139,34}{ a} \textcolor{black}{ very} \textcolor{black}{ special} \textcolor{black}{ case} \textcolor[RGB]{34,139,34}{ of} \textcolor[RGB]{34,139,34}{ the} \textcolor{black}{ Re}\textcolor[RGB]{34,139,34}{venue} \textcolor[RGB]{34,139,34}{ Equ}\textcolor{black}{ival}\textcolor[RGB]{34,139,34}{ence} \textcolor[RGB]{34,139,34}{ Theorem} \textcolor{black}{ later}\textcolor[RGB]{34,139,34}{.} \\
\midrule
\multicolumn{1}{c}{\texttt{After Training 60\% Checkpoint}} \\
\midrule
\textcolor{black}{ All}\textcolor{black}{-}\textcolor[RGB]{34,139,34}{pay} \textcolor[RGB]{34,139,34}{ au}\textcolor[RGB]{34,139,34}{ction} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{The} \textcolor{black}{ all}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{pay} \textcolor[RGB]{34,139,34}{ au}\textcolor[RGB]{34,139,34}{ction} \textcolor[RGB]{34,139,34}{ is} \textcolor{black}{ like} \textcolor{black}{ lo}\textcolor{black}{bb}\textcolor[RGB]{34,139,34}{ying}\textcolor{black}{.} \textcolor[RGB]{34,139,34}{ Each} \textcolor{black}{ player} \textcolor[RGB]{34,139,34}{ makes} \textcolor[RGB]{34,139,34}{ a} \textcolor[RGB]{34,139,34}{ bid}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ and} \textcolor{black}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{•} \textcolor[RGB]{34,139,34}{ \$\{}\textcolor[RGB]{34,139,34}{Q} \textcolor{black}{ =} \textcolor{black}{ Q}\textcolor{black}{\_\{\textbackslash }\textcolor[RGB]{34,139,34}{text}\textcolor[RGB]{34,139,34}{\{}\textcolor{black}{high}\textcolor[RGB]{34,139,34}{est}\textcolor[RGB]{34,139,34}{\}\}}\textcolor[RGB]{34,139,34}{\}\$,} \textcolor[RGB]{34,139,34}{ and} \textcolor{black}{ \textbackslash n }\textcolor{black}{•} \textcolor{black}{ \$\{}\textcolor{black}{P}\textcolor{black}{\}\$} \textcolor[RGB]{34,139,34}{ is} \textcolor{black}{ defined} \textcolor{black}{ by} \textcolor{black}{ requiring} \textcolor[RGB]{34,139,34}{ everyone} \textcolor[RGB]{34,139,34}{ to} \textcolor{black}{ pay} \textcolor[RGB]{34,139,34}{ their} \textcolor{black}{ bid}\textcolor[RGB]{34,139,34}{,} \textcolor{black}{ regardless} \textcolor[RGB]{34,139,34}{ of} \textcolor{black}{ whether} \textcolor[RGB]{34,139,34}{ they} \textcolor[RGB]{34,139,34}{ win} \textcolor{black}{ the} \textcolor{black}{ power} \textcolor[RGB]{34,139,34}{ dr}\textcolor[RGB]{34,139,34}{ill} \textcolor[RGB]{34,139,34}{ or} \textcolor[RGB]{34,139,34}{ not}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{This} \textcolor{black}{ is} \textcolor{black}{ clearly} \textcolor{black}{ not} \textcolor[RGB]{34,139,34}{ in}\textcolor[RGB]{34,139,34}{cent}\textcolor[RGB]{34,139,34}{ive} \textcolor{black}{ compatible}\textcolor[RGB]{34,139,34}{.} \textcolor{black}{ In} \textcolor[RGB]{34,139,34}{ fact}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ the} \textcolor{black}{ Nash} \textcolor{black}{ equilibrium} \textcolor{black}{ is} \textcolor{black}{ as} \textcolor[RGB]{34,139,34}{ follows}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Pro}\textcolor[RGB]{34,139,34}{position} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{4} \textcolor[RGB]{34,139,34}{ (}\textcolor{black}{N}\textcolor[RGB]{34,139,34}{ash} \textcolor{black}{ equilib}\textcolor{black}{ir}\textcolor{black}{um} \textcolor{black}{ of} \textcolor[RGB]{34,139,34}{ the} \textcolor{black}{ all}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{pay} \textcolor[RGB]{34,139,34}{ au}\textcolor[RGB]{34,139,34}{ction}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Cons}\textcolor[RGB]{34,139,34}{ider} \textcolor[RGB]{34,139,34}{ a} \textcolor{black}{ first}\textcolor[RGB]{34,139,34}{-}\textcolor{black}{price} \textcolor{black}{ au}\textcolor[RGB]{34,139,34}{ction} \textcolor[RGB]{34,139,34}{ where} \textcolor[RGB]{34,139,34}{ Anna} \textcolor[RGB]{34,139,34}{ and} \textcolor{black}{ El}\textcolor{black}{sa} \textcolor{black}{ have} \textcolor{black}{ values} \textcolor{black}{ uniformly} \textcolor{black}{ distributed} \textcolor{black}{ in} \textcolor{black}{ \$\{}\textcolor[RGB]{34,139,34}{{[}}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1}\textcolor{black}{0}\textcolor{black}{0}\textcolor{black}{0}\textcolor[RGB]{34,139,34}{{]}}\textcolor[RGB]{34,139,34}{\}\$.} \textcolor[RGB]{34,139,34}{ Suppose} \textcolor{black}{ both} \textcolor[RGB]{34,139,34}{ Anna} \textcolor[RGB]{34,139,34}{ and} \textcolor[RGB]{34,139,34}{ El}\textcolor[RGB]{34,139,34}{sa} \textcolor[RGB]{34,139,34}{ bid} \textcolor{black}{ \$\{\textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{2}\textcolor{black}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{cdot} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor{black}{(}\textcolor[RGB]{34,139,34}{x}\textcolor{black}{/}\textcolor{black}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{)\^{}}\textcolor[RGB]{34,139,34}{2}\textcolor{black}{\}\$} \textcolor[RGB]{34,139,34}{ if} \textcolor[RGB]{34,139,34}{ they} \textcolor{black}{ have} \textcolor{black}{ value} \textcolor{black}{ \$\{}\textcolor[RGB]{34,139,34}{x}\textcolor{black}{\}\$.} \textcolor{black}{ Then} \textcolor{black}{ this} \textcolor[RGB]{34,139,34}{ is} \textcolor{black}{ a} \textcolor{black}{ Nash} \textcolor[RGB]{34,139,34}{ equilibrium}\textcolor{black}{.} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Proof}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ Om}\textcolor{black}{itted}\textcolor{black}{,} \textcolor{black}{ but} \textcolor{black}{ a} \textcolor{black}{ fun} \textcolor{black}{ and} \textcolor{black}{ not}\textcolor{black}{-}\textcolor{black}{hard} \textcolor{black}{ exercise} \textcolor{black}{ if} \textcolor[RGB]{34,139,34}{ you} \textcolor{black}{ like} \textcolor{black}{ integr}\textcolor{black}{als}\textcolor{black}{.} \textcolor[RGB]{34,139,34}{ It} \textcolor[RGB]{34,139,34}{ will} \textcolor{black}{ follow} \textcolor[RGB]{34,139,34}{ from} \textcolor{black}{ a} \textcolor{black}{ later} \textcolor{black}{ result}\textcolor{black}{.} \textcolor{black}{ \$\textbackslash }\textcolor[RGB]{34,139,34}{Box}\textcolor[RGB]{34,139,34}{\$} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{Just} \textcolor[RGB]{34,139,34}{ for} \textcolor[RGB]{34,139,34}{ interest}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ let}\textcolor[RGB]{34,139,34}{’}\textcolor[RGB]{34,139,34}{s} \textcolor[RGB]{34,139,34}{ compute} \textcolor[RGB]{34,139,34}{ how} \textcolor[RGB]{34,139,34}{ much} \textcolor[RGB]{34,139,34}{ money} \textcolor{black}{ Hans} \textcolor{black}{ is} \textcolor[RGB]{34,139,34}{ going} \textcolor[RGB]{34,139,34}{ to} \textcolor[RGB]{34,139,34}{ make} \textcolor{black}{ off} \textcolor[RGB]{34,139,34}{ the} \textcolor[RGB]{34,139,34}{ dr}\textcolor[RGB]{34,139,34}{ill} \textcolor[RGB]{34,139,34}{ in} \textcolor[RGB]{34,139,34}{ this} \textcolor[RGB]{34,139,34}{ equilibrium}\textcolor[RGB]{34,139,34}{.} \textcolor{black}{ This} \textcolor[RGB]{34,139,34}{ time} \textcolor[RGB]{34,139,34}{ he} \textcolor{black}{ amount} \textcolor{black}{ paid} \textcolor[RGB]{34,139,34}{ to} \textcolor[RGB]{34,139,34}{ him} \textcolor[RGB]{34,139,34}{ is} \textcolor[RGB]{34,139,34}{ equal} \textcolor[RGB]{34,139,34}{ to} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{\$\textbackslash }\textcolor[RGB]{34,139,34}{displaystyle} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{mathbf} \textcolor[RGB]{34,139,34}{ E}\textcolor[RGB]{34,139,34}{\_\{}\textcolor[RGB]{34,139,34}{a}\textcolor[RGB]{34,139,34}{,}\textcolor{black}{e}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{left}\textcolor[RGB]{34,139,34}{(} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor{black}{a}\textcolor{black}{\^{}}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{\}\{}\textcolor{black}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ +} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{b}\textcolor[RGB]{34,139,34}{\^{}}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{right}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{34,139,34}{ =} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{int}\textcolor[RGB]{34,139,34}{\_\{}\textcolor{black}{0}\textcolor[RGB]{34,139,34}{\}\^{}\{}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}} \textcolor{black}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{x}\textcolor{black}{\^{}}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{\}\{}\textcolor{black}{1}\textcolor[RGB]{34,139,34}{0}\textcolor{black}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}} \textcolor{black}{ \textbackslash ;} \textcolor{black}{ dx} \textcolor[RGB]{34,139,34}{ =} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor{black}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{3}\textcolor{black}{\}.}\textcolor[RGB]{34,139,34}{\$} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{Sur}\textcolor{black}{prise} \textcolor{black}{ —} \textcolor{black}{ same} \textcolor[RGB]{34,139,34}{ value} \textcolor{black}{ again}\textcolor{black}{!} \textcolor[RGB]{34,139,34}{ This} \textcolor{black}{ is} \textcolor[RGB]{34,139,34}{ a} \textcolor{black}{ very} \textcolor{black}{ special} \textcolor{black}{ case} \textcolor[RGB]{34,139,34}{ of} \textcolor[RGB]{34,139,34}{ the} \textcolor{black}{ Re}\textcolor[RGB]{34,139,34}{venue} \textcolor[RGB]{34,139,34}{ Equ}\textcolor{black}{ival}\textcolor[RGB]{34,139,34}{ence} \textcolor[RGB]{34,139,34}{ Theorem} \textcolor{black}{ later}\textcolor{black}{.} \\
\midrule
\multicolumn{1}{c}{\texttt{After Training 80\% Checkpoint}} \\
\midrule
\textcolor{black}{ All}\textcolor{black}{-}\textcolor[RGB]{34,139,34}{pay} \textcolor[RGB]{34,139,34}{ au}\textcolor[RGB]{34,139,34}{ction} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{The} \textcolor{black}{ all}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{pay} \textcolor[RGB]{34,139,34}{ au}\textcolor[RGB]{34,139,34}{ction} \textcolor[RGB]{34,139,34}{ is} \textcolor{black}{ like} \textcolor{black}{ lo}\textcolor{black}{bb}\textcolor[RGB]{34,139,34}{ying}\textcolor{black}{.} \textcolor[RGB]{34,139,34}{ Each} \textcolor{black}{ player} \textcolor[RGB]{34,139,34}{ makes} \textcolor[RGB]{34,139,34}{ a} \textcolor[RGB]{34,139,34}{ bid}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ and} \textcolor{black}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{•} \textcolor[RGB]{34,139,34}{ \$\{}\textcolor{black}{Q} \textcolor{black}{ =} \textcolor{black}{ Q}\textcolor{black}{\_\{\textbackslash }\textcolor[RGB]{34,139,34}{text}\textcolor[RGB]{34,139,34}{\{}\textcolor{black}{high}\textcolor[RGB]{34,139,34}{est}\textcolor[RGB]{34,139,34}{\}\}}\textcolor[RGB]{34,139,34}{\}\$,} \textcolor[RGB]{34,139,34}{ and} \textcolor{black}{ \textbackslash n }\textcolor{black}{•} \textcolor{black}{ \$\{}\textcolor{black}{P}\textcolor{black}{\}\$} \textcolor[RGB]{34,139,34}{ is} \textcolor{black}{ defined} \textcolor{black}{ by} \textcolor{black}{ requiring} \textcolor{black}{ everyone} \textcolor[RGB]{34,139,34}{ to} \textcolor{black}{ pay} \textcolor[RGB]{34,139,34}{ their} \textcolor{black}{ bid}\textcolor[RGB]{34,139,34}{,} \textcolor{black}{ regardless} \textcolor[RGB]{34,139,34}{ of} \textcolor{black}{ whether} \textcolor[RGB]{34,139,34}{ they} \textcolor[RGB]{34,139,34}{ win} \textcolor{black}{ the} \textcolor{black}{ power} \textcolor[RGB]{34,139,34}{ dr}\textcolor[RGB]{34,139,34}{ill} \textcolor[RGB]{34,139,34}{ or} \textcolor[RGB]{34,139,34}{ not}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{This} \textcolor{black}{ is} \textcolor{black}{ clearly} \textcolor{black}{ not} \textcolor[RGB]{34,139,34}{ in}\textcolor[RGB]{34,139,34}{cent}\textcolor[RGB]{34,139,34}{ive} \textcolor{black}{ compatible}\textcolor[RGB]{34,139,34}{.} \textcolor{black}{ In} \textcolor[RGB]{34,139,34}{ fact}\textcolor[RGB]{34,139,34}{,} \textcolor{black}{ the} \textcolor{black}{ Nash} \textcolor{black}{ equilibrium} \textcolor{black}{ is} \textcolor{black}{ as} \textcolor[RGB]{34,139,34}{ follows}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Pro}\textcolor[RGB]{34,139,34}{position} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{4} \textcolor[RGB]{34,139,34}{ (}\textcolor{black}{N}\textcolor[RGB]{34,139,34}{ash} \textcolor{black}{ equilib}\textcolor{black}{ir}\textcolor{black}{um} \textcolor{black}{ of} \textcolor[RGB]{34,139,34}{ the} \textcolor{black}{ all}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{pay} \textcolor[RGB]{34,139,34}{ au}\textcolor[RGB]{34,139,34}{ction}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Cons}\textcolor[RGB]{34,139,34}{ider} \textcolor[RGB]{34,139,34}{ a} \textcolor{black}{ first}\textcolor[RGB]{34,139,34}{-}\textcolor{black}{price} \textcolor{black}{ au}\textcolor[RGB]{34,139,34}{ction} \textcolor[RGB]{34,139,34}{ where} \textcolor[RGB]{34,139,34}{ Anna} \textcolor[RGB]{34,139,34}{ and} \textcolor{black}{ El}\textcolor[RGB]{34,139,34}{sa} \textcolor{black}{ have} \textcolor{black}{ values} \textcolor{black}{ uniformly} \textcolor{black}{ distributed} \textcolor{black}{ in} \textcolor{black}{ \$\{}\textcolor[RGB]{34,139,34}{{[}}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1}\textcolor{black}{0}\textcolor{black}{0}\textcolor{black}{0}\textcolor[RGB]{34,139,34}{{]}}\textcolor[RGB]{34,139,34}{\}\$.} \textcolor[RGB]{34,139,34}{ Suppose} \textcolor[RGB]{34,139,34}{ both} \textcolor[RGB]{34,139,34}{ Anna} \textcolor[RGB]{34,139,34}{ and} \textcolor[RGB]{34,139,34}{ El}\textcolor[RGB]{34,139,34}{sa} \textcolor[RGB]{34,139,34}{ bid} \textcolor{black}{ \$\{\textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{2}\textcolor{black}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{cdot} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor{black}{(}\textcolor[RGB]{34,139,34}{x}\textcolor{black}{/}\textcolor{black}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor{black}{0}\textcolor{black}{)\^{}}\textcolor[RGB]{34,139,34}{2}\textcolor{black}{\}\$} \textcolor[RGB]{34,139,34}{ if} \textcolor[RGB]{34,139,34}{ they} \textcolor{black}{ have} \textcolor{black}{ value} \textcolor{black}{ \$\{}\textcolor[RGB]{34,139,34}{x}\textcolor{black}{\}\$.} \textcolor{black}{ Then} \textcolor{black}{ this} \textcolor[RGB]{34,139,34}{ is} \textcolor{black}{ a} \textcolor{black}{ Nash} \textcolor[RGB]{34,139,34}{ equilibrium}\textcolor{black}{.} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Proof}\textcolor[RGB]{34,139,34}{:} \textcolor{black}{ Om}\textcolor{black}{itted}\textcolor{black}{,} \textcolor{black}{ but} \textcolor{black}{ a} \textcolor{black}{ fun} \textcolor{black}{ and} \textcolor{black}{ not}\textcolor{black}{-}\textcolor{black}{hard} \textcolor[RGB]{34,139,34}{ exercise} \textcolor{black}{ if} \textcolor[RGB]{34,139,34}{ you} \textcolor[RGB]{34,139,34}{ like} \textcolor{black}{ integr}\textcolor{black}{als}\textcolor{black}{.} \textcolor[RGB]{34,139,34}{ It} \textcolor[RGB]{34,139,34}{ will} \textcolor{black}{ follow} \textcolor[RGB]{34,139,34}{ from} \textcolor{black}{ a} \textcolor{black}{ later} \textcolor{black}{ result}\textcolor{black}{.} \textcolor{black}{ \$\textbackslash }\textcolor[RGB]{34,139,34}{Box}\textcolor[RGB]{34,139,34}{\$} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Just} \textcolor[RGB]{34,139,34}{ for} \textcolor[RGB]{34,139,34}{ interest}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ let}\textcolor[RGB]{34,139,34}{’}\textcolor[RGB]{34,139,34}{s} \textcolor[RGB]{34,139,34}{ compute} \textcolor[RGB]{34,139,34}{ how} \textcolor[RGB]{34,139,34}{ much} \textcolor[RGB]{34,139,34}{ money} \textcolor{black}{ Hans} \textcolor{black}{ is} \textcolor[RGB]{34,139,34}{ going} \textcolor[RGB]{34,139,34}{ to} \textcolor[RGB]{34,139,34}{ make} \textcolor{black}{ off} \textcolor[RGB]{34,139,34}{ the} \textcolor[RGB]{34,139,34}{ dr}\textcolor[RGB]{34,139,34}{ill} \textcolor[RGB]{34,139,34}{ in} \textcolor[RGB]{34,139,34}{ this} \textcolor[RGB]{34,139,34}{ equilibrium}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{34,139,34}{ This} \textcolor[RGB]{34,139,34}{ time} \textcolor[RGB]{34,139,34}{ he} \textcolor[RGB]{34,139,34}{ amount} \textcolor{black}{ paid} \textcolor[RGB]{34,139,34}{ to} \textcolor[RGB]{34,139,34}{ him} \textcolor[RGB]{34,139,34}{ is} \textcolor[RGB]{34,139,34}{ equal} \textcolor[RGB]{34,139,34}{ to} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{\$\textbackslash }\textcolor[RGB]{34,139,34}{displaystyle} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{mathbf} \textcolor[RGB]{34,139,34}{ E}\textcolor[RGB]{34,139,34}{\_\{}\textcolor[RGB]{34,139,34}{a}\textcolor[RGB]{34,139,34}{,}\textcolor{black}{e}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{left}\textcolor[RGB]{34,139,34}{(} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor{black}{a}\textcolor{black}{\^{}}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{\}\{}\textcolor{black}{2}\textcolor{black}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ +} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{b}\textcolor[RGB]{34,139,34}{\^{}}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{right}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{34,139,34}{ =} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{int}\textcolor[RGB]{34,139,34}{\_\{}\textcolor{black}{0}\textcolor[RGB]{34,139,34}{\}\^{}\{}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor{black}{x}\textcolor{black}{\^{}}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{0}\textcolor{black}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}} \textcolor{black}{ \textbackslash ;} \textcolor{black}{ dx} \textcolor[RGB]{34,139,34}{ =} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{3}\textcolor{black}{\}.}\textcolor[RGB]{34,139,34}{\$} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{Sur}\textcolor{black}{prise} \textcolor{black}{ —} \textcolor{black}{ same} \textcolor{black}{ value} \textcolor{black}{ again}\textcolor[RGB]{34,139,34}{!} \textcolor[RGB]{34,139,34}{ This} \textcolor{black}{ is} \textcolor[RGB]{34,139,34}{ a} \textcolor{black}{ very} \textcolor{black}{ special} \textcolor{black}{ case} \textcolor[RGB]{34,139,34}{ of} \textcolor[RGB]{34,139,34}{ the} \textcolor{black}{ Re}\textcolor[RGB]{34,139,34}{venue} \textcolor{black}{ Equ}\textcolor{black}{ival}\textcolor[RGB]{34,139,34}{ence} \textcolor[RGB]{34,139,34}{ Theorem} \textcolor{black}{ later}\textcolor{black}{.} \\
\midrule
\multicolumn{1}{c}{\texttt{After Training 100\% Checkpoint}} \\
\midrule
\textcolor{black}{ All}\textcolor{black}{-}\textcolor[RGB]{34,139,34}{pay} \textcolor[RGB]{34,139,34}{ au}\textcolor[RGB]{34,139,34}{ction} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{The} \textcolor{black}{ all}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{pay} \textcolor[RGB]{34,139,34}{ au}\textcolor[RGB]{34,139,34}{ction} \textcolor[RGB]{34,139,34}{ is} \textcolor{black}{ like} \textcolor[RGB]{34,139,34}{ lo}\textcolor{black}{bb}\textcolor[RGB]{34,139,34}{ying}\textcolor{black}{.} \textcolor[RGB]{34,139,34}{ Each} \textcolor{black}{ player} \textcolor[RGB]{34,139,34}{ makes} \textcolor[RGB]{34,139,34}{ a} \textcolor[RGB]{34,139,34}{ bid}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ and} \textcolor{black}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{•} \textcolor[RGB]{34,139,34}{ \$\{}\textcolor{black}{Q} \textcolor{black}{ =} \textcolor{black}{ Q}\textcolor{black}{\_\{\textbackslash }\textcolor{black}{text}\textcolor[RGB]{34,139,34}{\{}\textcolor{black}{high}\textcolor[RGB]{34,139,34}{est}\textcolor[RGB]{34,139,34}{\}\}}\textcolor[RGB]{34,139,34}{\}\$,} \textcolor[RGB]{34,139,34}{ and} \textcolor{black}{ \textbackslash n }\textcolor{black}{•} \textcolor{black}{ \$\{}\textcolor{black}{P}\textcolor{black}{\}\$} \textcolor[RGB]{34,139,34}{ is} \textcolor{black}{ defined} \textcolor{black}{ by} \textcolor{black}{ requiring} \textcolor{black}{ everyone} \textcolor[RGB]{34,139,34}{ to} \textcolor{black}{ pay} \textcolor{black}{ their} \textcolor{black}{ bid}\textcolor[RGB]{34,139,34}{,} \textcolor{black}{ regardless} \textcolor[RGB]{34,139,34}{ of} \textcolor{black}{ whether} \textcolor[RGB]{34,139,34}{ they} \textcolor[RGB]{34,139,34}{ win} \textcolor{black}{ the} \textcolor{black}{ power} \textcolor[RGB]{34,139,34}{ dr}\textcolor[RGB]{34,139,34}{ill} \textcolor[RGB]{34,139,34}{ or} \textcolor[RGB]{34,139,34}{ not}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{This} \textcolor{black}{ is} \textcolor{black}{ clearly} \textcolor{black}{ not} \textcolor[RGB]{34,139,34}{ in}\textcolor[RGB]{34,139,34}{cent}\textcolor[RGB]{34,139,34}{ive} \textcolor{black}{ compatible}\textcolor[RGB]{34,139,34}{.} \textcolor{black}{ In} \textcolor[RGB]{34,139,34}{ fact}\textcolor[RGB]{34,139,34}{,} \textcolor{black}{ the} \textcolor{black}{ Nash} \textcolor{black}{ equilibrium} \textcolor{black}{ is} \textcolor{black}{ as} \textcolor[RGB]{34,139,34}{ follows}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Pro}\textcolor[RGB]{34,139,34}{position} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{4} \textcolor[RGB]{34,139,34}{ (}\textcolor{black}{N}\textcolor[RGB]{34,139,34}{ash} \textcolor{black}{ equilib}\textcolor{black}{ir}\textcolor{black}{um} \textcolor{black}{ of} \textcolor[RGB]{34,139,34}{ the} \textcolor{black}{ all}\textcolor[RGB]{34,139,34}{-}\textcolor[RGB]{34,139,34}{pay} \textcolor[RGB]{34,139,34}{ au}\textcolor[RGB]{34,139,34}{ction}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Cons}\textcolor[RGB]{34,139,34}{ider} \textcolor[RGB]{34,139,34}{ a} \textcolor{black}{ first}\textcolor[RGB]{34,139,34}{-}\textcolor{black}{price} \textcolor{black}{ au}\textcolor[RGB]{34,139,34}{ction} \textcolor[RGB]{34,139,34}{ where} \textcolor[RGB]{34,139,34}{ Anna} \textcolor[RGB]{34,139,34}{ and} \textcolor{black}{ El}\textcolor[RGB]{34,139,34}{sa} \textcolor{black}{ have} \textcolor{black}{ values} \textcolor{black}{ uniformly} \textcolor{black}{ distributed} \textcolor{black}{ in} \textcolor{black}{ \$\{}\textcolor[RGB]{34,139,34}{{[}}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1}\textcolor{black}{0}\textcolor{black}{0}\textcolor{black}{0}\textcolor[RGB]{34,139,34}{{]}}\textcolor[RGB]{34,139,34}{\}\$.} \textcolor[RGB]{34,139,34}{ Suppose} \textcolor[RGB]{34,139,34}{ both} \textcolor[RGB]{34,139,34}{ Anna} \textcolor[RGB]{34,139,34}{ and} \textcolor[RGB]{34,139,34}{ El}\textcolor[RGB]{34,139,34}{sa} \textcolor[RGB]{34,139,34}{ bid} \textcolor{black}{ \$\{\textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{2}\textcolor{black}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{cdot} \textcolor[RGB]{34,139,34}{ }\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor{black}{(}\textcolor[RGB]{34,139,34}{x}\textcolor{black}{/}\textcolor{black}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor{black}{0}\textcolor[RGB]{34,139,34}{)\^{}}\textcolor[RGB]{34,139,34}{2}\textcolor{black}{\}\$} \textcolor[RGB]{34,139,34}{ if} \textcolor[RGB]{34,139,34}{ they} \textcolor{black}{ have} \textcolor{black}{ value} \textcolor{black}{ \$\{}\textcolor[RGB]{34,139,34}{x}\textcolor{black}{\}\$.} \textcolor{black}{ Then} \textcolor{black}{ this} \textcolor[RGB]{34,139,34}{ is} \textcolor{black}{ a} \textcolor{black}{ Nash} \textcolor[RGB]{34,139,34}{ equilibrium}\textcolor{black}{.} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Proof}\textcolor[RGB]{34,139,34}{:} \textcolor[RGB]{34,139,34}{ Om}\textcolor{black}{itted}\textcolor{black}{,} \textcolor{black}{ but} \textcolor{black}{ a} \textcolor{black}{ fun} \textcolor{black}{ and} \textcolor{black}{ not}\textcolor[RGB]{34,139,34}{-}\textcolor{black}{hard} \textcolor{black}{ exercise} \textcolor{black}{ if} \textcolor[RGB]{34,139,34}{ you} \textcolor[RGB]{34,139,34}{ like} \textcolor{black}{ integr}\textcolor{black}{als}\textcolor{black}{.} \textcolor[RGB]{34,139,34}{ It} \textcolor[RGB]{34,139,34}{ will} \textcolor{black}{ follow} \textcolor[RGB]{34,139,34}{ from} \textcolor{black}{ a} \textcolor{black}{ later} \textcolor{black}{ result}\textcolor{black}{.} \textcolor{black}{ \$\textbackslash }\textcolor[RGB]{34,139,34}{Box}\textcolor[RGB]{34,139,34}{\$} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{Just} \textcolor[RGB]{34,139,34}{ for} \textcolor[RGB]{34,139,34}{ interest}\textcolor[RGB]{34,139,34}{,} \textcolor[RGB]{34,139,34}{ let}\textcolor[RGB]{34,139,34}{’}\textcolor[RGB]{34,139,34}{s} \textcolor[RGB]{34,139,34}{ compute} \textcolor[RGB]{34,139,34}{ how} \textcolor[RGB]{34,139,34}{ much} \textcolor[RGB]{34,139,34}{ money} \textcolor{black}{ Hans} \textcolor{black}{ is} \textcolor[RGB]{34,139,34}{ going} \textcolor[RGB]{34,139,34}{ to} \textcolor[RGB]{34,139,34}{ make} \textcolor{black}{ off} \textcolor[RGB]{34,139,34}{ the} \textcolor[RGB]{34,139,34}{ dr}\textcolor[RGB]{34,139,34}{ill} \textcolor[RGB]{34,139,34}{ in} \textcolor[RGB]{34,139,34}{ this} \textcolor[RGB]{34,139,34}{ equilibrium}\textcolor[RGB]{34,139,34}{.} \textcolor[RGB]{34,139,34}{ This} \textcolor[RGB]{34,139,34}{ time} \textcolor[RGB]{34,139,34}{ he} \textcolor[RGB]{34,139,34}{ amount} \textcolor{black}{ paid} \textcolor[RGB]{34,139,34}{ to} \textcolor[RGB]{34,139,34}{ him} \textcolor[RGB]{34,139,34}{ is} \textcolor[RGB]{34,139,34}{ equal} \textcolor[RGB]{34,139,34}{ to} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor[RGB]{34,139,34}{\$\textbackslash }\textcolor[RGB]{34,139,34}{displaystyle} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{mathbf} \textcolor[RGB]{34,139,34}{ E}\textcolor[RGB]{34,139,34}{\_\{}\textcolor[RGB]{34,139,34}{a}\textcolor[RGB]{34,139,34}{,}\textcolor{black}{e}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{left}\textcolor[RGB]{34,139,34}{(} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor{black}{a}\textcolor{black}{\^{}}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{\}\{}\textcolor{black}{2}\textcolor{black}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ +} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{b}\textcolor[RGB]{34,139,34}{\^{}}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{right}\textcolor[RGB]{34,139,34}{)} \textcolor[RGB]{34,139,34}{ =} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{int}\textcolor[RGB]{34,139,34}{\_\{}\textcolor{black}{0}\textcolor[RGB]{34,139,34}{\}\^{}\{}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor{black}{x}\textcolor{black}{\^{}}\textcolor[RGB]{34,139,34}{2}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{0}\textcolor{black}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}} \textcolor{black}{ \textbackslash ;} \textcolor{black}{ dx} \textcolor[RGB]{34,139,34}{ =} \textcolor[RGB]{34,139,34}{ \textbackslash }\textcolor[RGB]{34,139,34}{frac}\textcolor[RGB]{34,139,34}{\{}\textcolor[RGB]{34,139,34}{1}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{0}\textcolor[RGB]{34,139,34}{\}\{}\textcolor[RGB]{34,139,34}{3}\textcolor{black}{\}.}\textcolor[RGB]{34,139,34}{\$} \textcolor[RGB]{34,139,34}{ \textbackslash n } \textcolor[RGB]{34,139,34}{ \textbackslash n }\textcolor{black}{Sur}\textcolor{black}{prise} \textcolor{black}{ —} \textcolor{black}{ same} \textcolor[RGB]{34,139,34}{ value} \textcolor{black}{ again}\textcolor[RGB]{34,139,34}{!} \textcolor[RGB]{34,139,34}{ This} \textcolor{black}{ is} \textcolor[RGB]{34,139,34}{ a} \textcolor{black}{ very} \textcolor{black}{ special} \textcolor{black}{ case} \textcolor[RGB]{34,139,34}{ of} \textcolor[RGB]{34,139,34}{ the} \textcolor{black}{ Re}\textcolor[RGB]{34,139,34}{venue} \textcolor{black}{ Equ}\textcolor{black}{ival}\textcolor[RGB]{34,139,34}{ence} \textcolor[RGB]{34,139,34}{ Theorem} \textcolor{black}{ later}\textcolor{black}{.} 
\\ \bottomrule
\end{tabular}
}
\caption{During the process of training the \model{} using ToT, the selection of tokens for the same piece of text. The tokens marked in \textcolor[RGB]{34,139,34}{green} represent the actual tokens trained during the ToT training process, while the remaining black tokens are not trained during the ToT training process.}
\label{tab:train_dymatic_tokens}
\end{table*}
